Intensity interferometry for ultralight bosonic dark matter detection

Ultralight bosonic dark matter (UBDM) can be described by a classical wave-like field oscillating near the Compton frequency of the bosons. If a measurement scheme for the direct detection of UBDM interactions is sensitive to a signature quadratic in the field, then there is a near-zero-frequency (dc) component of the signal. Thus, a detector with a given finite bandwidth can be used to search for bosons with Compton frequencies many orders of magnitude larger than its bandwidth. This opens the possibility of a detection scheme analogous to Hanbury Brown and Twiss intensity interferometry. Assuming that the UBDM is virialized in the galactic gravitational potential, the random velocities produce slight deviations from the Compton frequency. These result in stochastic fluctuations of the intensity on a time scale determined by the spread in kinetic energies. In order to mitigate ubiquitous local low-frequency noise, a network of sensors can be used to search for the stochastic intensity fluctuations by measuring cross-correlation between the sensors. This method is inherently broadband, since a large range of Compton frequencies will yield near-zero-frequency components within the sensor bandwidth that can be searched for simultaneously. Measurements with existing sensor networks have sufficient sensitivity to search experimentally unexplored parameter space.

==> VersionControl/Comments20230516.tex <==
%\DB{I am not sure if it is clear from the text 1. what exactly is proportional to UBDM intensitity and 2. what UBDM intensity is. Normally, intensity is measured in power per unit time per unit area. Probably not what you mean here...} \DK{I think explicitly defining that we are referring to the square of the field and then putting intensity in quotes gives the flavor of what we mean: we want to explain the title of the paper and make the connection to HBT interferometry, but we don't want to be too technically explicit, since the key information is really in the cited equations. Hopefully this language solves the issues Dima raised.} 
%{\color{cyan}YS: In optics, there exists a definition of the light-field intensity as being equal to the square of the light-field amplitude. We could in principle use a similar terminology for our scalar field here with the understanding of this analogy. It is more usual, however, to relate $\varphi^2$ to the energy density via a proportionality relation.}


%\DB{I used to be a big proponent of this, but now I wonder if such language is accurate. If we have just one boson, the phase should be undefined. It is probably still OK to add all the modes like this, but association with individual bosons seems wrong...} \NLF{I agree; I think that individual particles would also be spatially localized wavepackets (and therefore have multiple frequencies). However, this discussion is out of the scope of this work; maybe we can avoid it somehow?} \DK{I also agree, this has always bothered me. I propose to use the terminology ``an individual plane wave representing a mode of the bosonic field'' -- I view the ``particles'' as excitations of a particular mode of the field.}
%{\color{cyan}YS: I personally don't see a big issue here, but if you prefer, it could be clearer to instead present an expression for the overall wavefunction as a sum over the wavefunctions associated with the individual particles.} \HMR{I think that changing the wording will create more confusion than clarity.  I would keep the term bosons and add a similar footnote to  footnote 3 of Ref.~\cite{foster2018} as Derek suggested.}

%\DB{Somehow, I am reminded of the number-phase uncertainty relation here; maybe we should bring this up for a quick discussion...} \DK{I agree, and this highlights the problem with this terminology, so I would use ``plane wave'' instead of ``boson'' here}

%\DB{One more time... Maybe, I would feel better about individual waves rather than individual bosons} \DK{Agreed, switch to ``plane waves''.} 
%{\color{cyan}YS: The wavefunctions associated with the individual bosons are indeed plane waves in our case. Regarding related discussion below about avoiding the use of the term ``bosons'' and the insinuation of their corpuscular/particle nature, the principle of wave-particle duality allows us to consider bosons as either particles or waves, so I personally don't see a strong reason to avoid using the term ``bosons'' in our discussion.}


%\DB{So where is the promised explanation of why it is good to go to the complex notation?} \NLF{That is the explanation, its immediately above this comment: it leads to a sum of $N$ terms instead of $N^2$ terms; its a big difference for the computer. It is purely a technical issue.} \DK{I think this is fine as is.} \DB{In response, I agree that this is HUGE in terms computations; however, I feel that attributing this to the use of complex notations may be misleading. It must be that using sin and cos and some simple trigonometry, one should be able to arrive at the same results. You agree?} \NLF{I think I now see your point: Yes, I think both expressions are equivalent (redefining the phases $\theta_n$). The trick we want to communicate is NOT going into complex notation; the trick is evaluating the field and "squaring" it INSTEAD of evaluating the expression for the field squared [+ using the chain rule for the gradients]. One is much more computationally expensive. I think we could have just as well evaluated Eq. 7 (cosines) and "squared" that. Is that correct Hector?} \HMR{ I am not sure that I understand but I think you mean that one can go from Eq.12 to Eq.16 (which are equivalent) without the step of introducing complex notation. The advantage is clear Eq.12 is a double sum and Eq.16 is four independent sums (two are hidden in $\varphi_c$ and $\varphi_c^*$. It may be that simple trigonometry can bring you from Eq.12 to Eq.16. However, I did not try and I find that complex notation is a standard mathematical tool to simplify operations. It is not an attribution but a way ( of probably many ) to show that Eq.12 to Eq.16 are the same.

%\DB{waves ?} \DK{Agreed, suggest again to change to ``plane waves''.}
%This is considerably less that the number of particles expected to be interacting with a sensor. \DB{I am no longer sure, this is a relevant quantity to compare to...} \DK{Yes, this is another good point about the confusion related to the mixing of terminology between particles and waves. There is a discussion of this exact point in the Safdi paper \cite{foster2018}, and they end up callin gthem ``particles'' even though that is misleading, but they discuss it in a footnote. I think we should continue to call them ``waves'' but we can adapt that discussion in footnote 3 of Ref.~\cite{foster2018} to our case here. I suggest we do that. Also in Phys Rev. D you can have footnotes on the same page instead of at the end which I like. We could make use of that throughout as necessary, here might be a good opportunity!} [For an example UBDM mass of $10^{-11}$\,eV/$c^2$ (and $\rho\ts{dm} = 0.3$~GeV/cm$^3$) there is a number density of particles of $\sim \! 10^{19}$\,cm$^{-3}$. Also, the de~Broglie wavelength for particles moving with $v_0$, is $\sim \! 10^{10}$\,cm: a sensor will be interacting with a number of particles that cannot be simulated with the methods presented here within a reasonable time.] Instead we chose $N=10^3$ as the number of particles that can be simulated with our available hardware.


%The characteristic coherence time of the field $\varphi$ is~\cite{derevianko2018detecting} 
%\begin{equation}
%    \tau_\varphi \approx \frac{2 \hbar}{ m_\varphi v_0^2}\,,
%    \label{eq:coherence_time}
%\end{equation}
%which is used as a benchmark timescale throughout the text. Note that there is an ambiguity, up to a factor of $2\pi$, in the definitions of $\tau_c$ used in the literature~\cite{Centers2019}. 
%\DB{I would say, the factor of 2 here is a ``pollutant,'' especially, becuase this equation is already introduced (without the 2) at the end of p. 1. My suggestion would be to make the equation on p. 1 into a separate line and use that as the definition of the dorrelation time; I would then lose Eq. (18). We can discuss, if you like.} \DK{I think that we could definitely do it Dima's way, or at least now that the two instances agree it is not as bad. Whatever Nate thinks is fine with me :).} \NLF{I prefer to leave it as is. Redefining this is dangerous at this point. For example, we would also have to change the definition of Eq. 17 or rescale Fig 2, without a strong reason IMO.}
%{\color{cyan}YS: The coherence time is set by the characteristic spread in the particle kinetic energies $mv^2/2$, so the factor of 2 in the numerator of Eq.~(18) does in principle have an important physical basis.}

%The full width at half maximum of the~$\varphi$ spectral lineshape is $\approx \omega_c v_0^2/c^2$, giving a useful estimate of the benchmark coherence time $\tau_\varphi$ of the field~(the result is exact for a Lorentzian lineshape~\cite{gramolin2021spectral} \DB{This confuses the socks off of me... If the lineshape is non-Lorenzian, how can one talk about any exact results? There must be some imprecision in wording here...} \NLF{The general coherence time is defined in Eq. 17, there is no need for things to be Lorentzian. About the wording, I think the paragraphs are arranged in a strange way, maybe because of the appendix migration.- The idea is: 1) the coherence time for a general pair of signals is Eq. 17. 2) The exact $\tau_c$ --for a Lorentzian lineshaped-- scalar ALP is $\tau_\varphi$ Eq. 18. 3) We simulated different ALP field (gradients) and compared their resulting $\tau_c$ with the ideal Lorentzian case, $\tau_\varphi$.} \DK{I think maybe with the factor of 2 now appearing in the original and the cited refs and discussion around Eq. (18) all is maybe OK now.}. \DB{In response, I like the way NFL has laid this out here. Can this be incorporated? No strong feelings, though.} \DK{Cool, sounds good to me!}


%\DB{In experiments like, say WRESL, we take the FT of the data and see a bunch of peaks, which are usually spurious. We can do various experiments to test if the peaks are real. However, here, since we look at near-DC, this is like a big waste bin, where ALL spurious effects will contribute. I imagine, we can add auxiliary sensors (gravimeters, unshielded mags, etc.) to reduce the correlated signal. However, it will not be so trivial to prove that whatever remains is not spurious. This leaves some dissatisfaction... Maybe, the relations in Figs. 1 and 2 can help a bit.} \DK{I do agree that low-frequency signals (the smallest frequency bin) can be challenging to interpret, but I propose no change to the manuscript and leave as is. Good point but not much to say other than let's deal with this in our results paper!} \DB{One the other hand, the point just above about this extra check may be worth capturing in a sentence...} \DK{Sure!}


%\DB{All these assumptions seem questionable...} \DK{I think that what we are really saying here is that there is no preferred direction, but maybe this is not true as there is a ``wind'' in the direction of Cygnus. But over time as the Earth rotates there is some averaging of this. On the other hand, I think all this is accounted for in the simulation, and that seems to agree. So if there is any non-spherically symmetric correlations in the final result, they turn out to be small. Maybe we should note that because of the relative motion of the Earth with respect to the rest frame of the galaxy, these assumptions may not be fully satisfied, but our simulation which accounts for this motion shows there is no significant deviations from the basic conclusions of this derivation (see Fig. 7).} \DB{OK, but there is a nonzero projection of the Earth rotation axis onto the direction towards Signus and that does not average over the year, correct? If so, if the sensitive axis of the sensor has a nonzero projection on the rotation axis, there is no averaging...} \DK{Yes, I agree with that. But maybe there is not much left after the various velocities of rotation and orbit around Sun are accounted for...? Also the spread is about equal to the mean. But definitely I agree this should be mentioned.}

==> VersionControl/maintext_20230407.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Missing Reviewer A comment
%It would also be helpful to the general reader to justify the cosmological motivations for the fluctuations on this scale in a practical way, i.e. addressing at what stage of the universe these fluctuations arise (when are the cosmic fields "frozen in") and if they are possibly affected by inflation, etc.


% Introduce the dark matter problem
A wide variety of evidence suggests the existence of dark matter, an invisible substance that constitutes a large fraction of the matter in the Universe \cite{Fen10,spergel2015dark,graham2015experimental}. Despite decades of research, its microscopic nature remains unknown. A promising hypothesis is that dark matter predominantly consists of ultralight bosons, particles with masses $m_\varphi \ll 1~{\textrm{eV}}/c^2$, such as axions~\cite{Pre83,Abb83,Din83}, axion-like particles (ALPs)~\cite{Gra15,co2020predictions}, or hidden photons~\cite{holdom1986two,cvetivc1996implications,Okun1982}. Ultralight bosons can couple to Standard Model (SM) particles through a variety of ``portals'' \cite{graham2016dark,safronova2018search}, which have been used to search for ultralight bosonic dark matter (UBDM) --- see, for example, Refs.\,\cite{Asz01,Asz10,budker2014proposal,Sik14,chaudhuri2015radio,geraci2016sensitivity,abel2017search,wu2019search,garcon2019constraints,phipps2020exclusion,manley2020searching,crescini2020axion,braine2020extended,backes2021quantum,antypas2021probing,roussy2021experimental,Ayb21CASPErE,gramolin2021search}.

% Advantage of intensity measurement
Numerous experiments looking for UBDM are based on resonant systems, which require accurate tuning to the unknown Compton frequency, $\omega_c = m_\varphi c^2 / \hbar$, in order to be sensitive to UBDM. Therefore, a time-consuming scan of tunable parameters must be performed to search a wide range of masses. However, if a search is based on the measurement of the \emph{intensity} of the UBDM, part of the signal is down-converted to near-zero frequency~\cite{stadnik2015can,hees2018violation}, regardless of the particular Compton frequency of the UBDM. 

% Explain the stochastic fluctuations
% Edited by Derek
In the commonly considered simplest version of the standard halo model (SHM) for dark matter~\cite{Zyla:2020zbs,evans2019refinement,drukier1986detecting}, the net UBDM field results from the superposition of numerous virialized bosons \cite{derevianko2018detecting}. Such a model assumes minimal self-interactions \cite{Bohua2014} and ignores non-virialized dark matter streams \cite{diemand2008clumps} and small-scale composite dark matter structures such as boson stars \cite{eby2016boson} or topological defects \cite{Pos13}.  The velocity dispersion of the dark matter particles in the neighborhood of our solar system is $v_0 \sim 10^{-3}c$. Consequently, the oscillation frequencies associated with the virialized bosons are Doppler-shifted. This generates a fractional shift from $\omega_c$ and a spread of frequencies of $\sim v_0^2/\prn{2c^2} \sim 5 \times 10^{-7}$. Because of the random distribution of frequencies of the UBDM, the amplitude of the net UBDM field stochastically fluctuates, as discussed in detail in Refs.~\cite{Centers2019,foster2018,hui2021wave,schive2014cosmic,turner1990periodic,o2017axion,lisanti2021stochastic,gramolin2021spectral}. We emphasize that this is an essential feature of the UBDM field in the SHM.  The characteristic time scale, $\tau_\phi \sim m_\phi v_0^2 / \hbar$, and length scale, $\lambda_\phi \sim \hbar / \prn{m_\phi v_0}$, of the fluctuations depends on the mass, $m_\phi$, and velocity dispersion, $v_0$, of the bosons~\cite{derevianko2018detecting}. In comparison to a direct measurement of the UBDM field, a measurement of the UBDM field intensity produces a frequency down-conversion of the UBDM signal to near-dc. The spectral linewidth of this near-dc signal is $\sim \! \! 10^6$~times smaller than $\omega_c$. Looking for this near-dc feature allows sensors with a limited bandwidth to probe UBDM with masses $\sim \! \! 10^6$~times larger than searching for direct field oscillations at $\omega_c$.

% quadratic Lagrangian for clocks
The frequency down-conversion discussed above occurs naturally when considering quadratic portals where the interaction with SM particles is proportional to the square of the UBDM field\,\cite{stadnik2015can,hees2018violation,Pos13,Der14,Oli08,Sta15,dailey2021quantum}. A spin-0 field $\varphi(\bs{r},t)$ can interact with SM fermions and electromagnetic fields according to the phenomenological quadratic scalar Lagrangian\,\cite{stadnik2015can}
\begin{align}
    \mc{L}_s = \hbar c \prn{\pm \frac{m_f c^2}{\Lambda_f^2} \bar{\psi}_f\psi_f \pm \frac{1}{4 \Lambda_\gamma^2} F_{\mu\nu}^2} \varphi^2(\bs{r},t)~,
    \label{eq:scalar-Lagrangian}
\end{align}
where $\Lambda_f$ and $\Lambda_\gamma$ parametrize the couplings to fermions and photons, respectively, where the $\pm$ indicates the sign of the coupling, $m_f$ is the fermion mass, $\psi_f$ is the fermion field, and $F_{\mu\nu}$ is the Faraday tensor.

% Effect of the interaction for clocks
The effects of the interactions described by Eq.\,\eqref{eq:scalar-Lagrangian} can be understood in terms of redefinitions of the effective fermion masses and the fine-structure constant $\alpha$\,\cite{stadnik2015can,Der14}:
\begin{align}
    m_f^{({\rm{eff}})} (\bs{r},t) & = m_f \prn{ 1 \mp \frac{\hbar c}{\Lambda_f^2} \varphi^2(\bs{r},t) }~, \label{eq:scalar-mass-variation} \\
    \alpha^{({\rm{eff}})} (\bs{r},t) & = \alpha \prn{ 1 \pm \frac{\hbar c}{\Lambda_\gamma^2} \varphi^2(\bs{r},t) }~. \label{eq:scalar-alpha-variation}
\end{align}
Variations of $m_f^{({\rm{eff}})}$ and $\alpha^{({\rm{eff}})}$ can be measured with atomic clocks or interferometers~\cite{Der14,wcislo2016experimental,roberts2017search,roberts2020search,dailey2021quantum,nagano2019axion,aiello2021constraints,badurina2020aion,Stadnik2016,Grote2019,Vermeulen2021,Sta15}, or generally by direct comparison of systems with different dependence on these fundamental constants~\cite{Antypas2019Oct,Antypas2020Apr,antypas2021probing,Oswald2021Nov,Tretiak2022Jan}.

% Quadratic interaction with magnetometers
Additionally, a generalized spin-0 pseudoscalar (ALP) field can possess linear and/or quadratic interactions with the axial-vector current of a SM
fermion~\cite{Pos13}, $\bar{\psi}_f \gamma^\mu\gamma_\ts{5} \psi_f$,
\begin{align}
 \mc{L}_\ts{lin} = \pm\frac{1}{f_l} \bar{\psi}_f \gamma^\mu\gamma_\ts{5} \psi_f \partial_\mu \varphi(\bs{r},t)~,
 \label{eq:pseudoscalar-Lagrangian_lin}
 \\
 \mc{L}_\ts{quad} = \pm\frac{1}{f_q^2} \bar{\psi}_f \gamma^\mu\gamma_\ts{5} \psi_f \partial_\mu \varphi^2(\bs{r},t)~,
\label{eq:pseudoscalar-Lagrangian}
\end{align}
%\begin{align}
%    \mc{L}_\varphi = \pm\frac{1}{f_q^2} \underbrace{\bar{\psi}_f \gamma^\mu\gamma_\ts{5} \psi_f}_{{\substack{\text{fermion axial} \\ \text{vector current}}}} \partial_\mu \varphi^2(\bs{r},t)~,
%    \label{eq:pseudoscalar-Lagrangian}
%\end{align}
where $f_l$ and $f_q$ parameterize the linear and quadratic couplings to fermion spins,  $\gamma^\mu$ and $\gamma_\ts{5}$ are Dirac matrices. The quantum chromodynamics (QCD) axion \cite{Kim79,Shi80,Zhi80,Din81,Sik83} associated with the Peccei-Quinn solution to the strong CP-problem \cite{peccei1977cp} generally possesses the linear coupling described by Eq.~\eqref{eq:pseudoscalar-Lagrangian_lin} (see, e.g., Ref.~\cite{Gra13}). Alternatively, in effective field theories with ALPs not associated with the QCD sector, the linear coupling term may be strongly suppressed or absent \cite{Oli08}, in which case the leading-order interaction with the axial-vector current may be the quadratic coupling of Eq.~\eqref{eq:pseudoscalar-Lagrangian} \cite{Pos13}.
Note that, like Eq.~\eqref{eq:pseudoscalar-Lagrangian_lin}, the description of the quadratic interaction in Eq.~\eqref{eq:pseudoscalar-Lagrangian} is manifestly Lorentz covariant, since replacing $\varphi$ by $\varphi^2$ preserves the overall number-type Lorentz structure because $\varphi$ is a spinless field.
Effective field theories featuring an ALP-spin interaction dominated by the quadratic term have much weaker constraints on the associated coupling constant $f_q$ from astrophysics \cite{Oli08,Pos13}. Of note is the fact that while the linear interaction of Eq.~\eqref{eq:pseudoscalar-Lagrangian_lin} is CP-conserving, the quadratic interaction in Eq.~\eqref{eq:pseudoscalar-Lagrangian} is CP-violating, and thus could potentially play a role in baryogenesis \cite{bernreuther2002cp}. While models with interactions $\propto \varphi^2$ were originally developed phenomenologically (see Ref.~\cite{Oli08} and references therein), string theory is an example of a fundamental theory generating quadratic interactions \cite{hinterbichler2011towards} such as those described by Eqs.~\eqref{eq:scalar-Lagrangian} and \eqref{eq:pseudoscalar-Lagrangian}, and theoretical work in this area is ongoing. Since our proposed search method relies on signals quadratic in the ALP field, in the rest of this work we focus our attention on the quadratic coupling.

As with the linear interaction~\cite{Sta14,JacksonKimball2023}, in the nonrelativistic limit, Eq.\,\eqref{eq:pseudoscalar-Lagrangian} yields the interaction Hamiltonian \cite{Pos13,dailey2021quantum} 
\begin{align}
    \mc{H}_\varphi = \mp\frac{2\hbar^2c^2}{f_q^2} \bs{S} \cdot \bs{\nabla} \varphi^2(\bs{r},t)~.
    \label{eq:quadratic-Hamiltonian}
\end{align}
Equation~\eqref{eq:quadratic-Hamiltonian} features a structure similar to that of the Zeeman Hamiltonian, $\mc{H}_Z= \gamma \bs{S} \cdot \bs{B}$, where $\gamma$ is the gyromagnetic ratio and $\bs{B}$ is a magnetic field (with the above noted difference that $\mc{H}_Z$ is CP-even while $H_\varphi$ is CP-odd). Therefore $\bs{\nabla} \varphi^2(\bs{r},t)$ couples to a fermion spin $\bs{S}$ in a manner similar to a magnetic field~\cite{Pos13}, playing the role of a ``pseudo-magnetic'' field. Thus, such pseudoscalar fields can be searched for in the spin dynamics of electrons or nuclei. While a variety of sensors could be used, here we focus on atomic (nuclear) magnetometers since these are intrinsically sensitive to Zeeman shifts~\cite{Pus13,afach2018characterization,kimball2018searching,masia-roig_analysis_2020,afach2021search,Jiang2021Dec}.

% Networks to detect the stochastic fluctuations
The effects described by Eqs.\,\eqref{eq:scalar-mass-variation},~\eqref{eq:scalar-alpha-variation},~and~\eqref{eq:quadratic-Hamiltonian} are proportional to the UBDM intensity and exhibit \mbox{near-dc} stochastic amplitude fluctuations. Although measuring low-frequency signals is technically challenging due to multiple sources of low-frequency noise, an array of independent, geographically distributed sensors will tend to have uncorrelated noise. In contrast, the slowly-changing UBDM intensity will lead to a common-mode fluctuating signal present in all detectors within a coherence length of one another, which will appear in correlations between the sensors. We advocate for the use of networks of sensors to search for these stochastic fluctuations. There are existing and proposed dark matter searches sensitive to these interactions using networks consisting of a variety of sensor types such as atomic clocks~\cite{Der14,wcislo2016experimental,roberts2017search,roberts2020search,dailey2021quantum,collaboration2021frequency}, atomic magnetometers~\cite{Pos13,Pus13,afach2018characterization,kimball2018searching,masia-roig_analysis_2020,afach2021search,fedderke2021earth,fedderke2021search,arza2021earth}, gravimeters~\cite{hu2020network,mcnally2020constraining,horowitz2020gravimeter}, laser interferometers~\cite{hall2018laser,nagano2019axion,aiello2021constraints,Stadnik2016,Grote2019,Vermeulen2021,Sta15}, and atom interferometers \cite{badurina2020aion}. The methodology described below is analogous to Hanbury Brown and Twiss intensity interferometry\,\cite{brown1956question}, and can be used to dramatically expand the range of UBDM Compton frequencies that particular sensors can probe~\cite{InterferometryNote}\nocite{derevianko2018detecting,foster2021}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section*{Stochastic properties of the ultralight bosonic dark matter field}
\label{sec:field-properties}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Introduce our treatment of the UBDM field

\medskip

\noindent \emph{Stochastic properties of the UBDM field.~---~}The properties of the UBDM field can be derived using the framework described in Refs.\,\cite{Centers2019,derevianko2018detecting,foster2018,hui2021wave,schive2014cosmic,turner1990periodic,o2017axion,lisanti2021stochastic,gramolin2021spectral}. In brief, assuming that UBDM does not interact with itself, each individual particle can be treated as an independent wave. In this scenario, the UBDM field is well described by a superposition of these individual waves.

% Field produced by one boson
If the local dark-matter energy density $\rho\ts{dm}$ results from $N$ ultralight bosons of mass $m_\varphi$, the field contribution of an individual boson $n$ is
\begin{align}
    \varphi_n(\bs{r},t) \approx \frac{\varphi_0}{\sqrt{N}} \cos\prn{ \omega_n t - \bs{k}_n \cdot \bs{r} + \theta_n }~,
    \label{eq:single-boson-field}
\end{align}
where the boson field amplitude is given by~\cite{Gra13}
\begin{align}
    \varphi_0 = \frac{\hbar}{m_\varphi c} \sqrt{ 2 \rho\ts{dm} },
    \label{eq:single-ALP-field-amp}
\end{align}
such that the average energy density in the UBDM field comprises the totality of the local dark matter. Here, $\bs{k}_n = m_\varphi \bs{v}_n /  \hbar$ is the wave vector corresponding to $\bs{v}_n$, the velocity of the $n^\text{th}$ boson in the laboratory frame, while $\theta_n$ is a phase associated with each boson, that is randomly distributed between $0$ and $2\pi$. The oscillation frequency of the individual UBDM particles, $\omega_{n}$, is determined mostly by their Compton frequency, $\omega_{c}$. However, the relativistic Doppler effect introduces small deviations from $\omega_{c}$, so that
\begin{align}
    \omega_n = \omega_c \prn{ 1 + \frac{\bs{v}_n^2}{2c^2} },
\end{align}
for $v_n \ll c$. Therefore, the distribution of $\omega_n$ (and $\bs{k}_n$) is determined by the velocity distribution of the particles as observed in the laboratory frame. According to the standard halo model,~$\bs{v}_n$ follows a displaced Maxwell-Boltzmann distribution.
%given by
%\begin{equation}
%f_{\text{lab}}(\bs{v}) \approx \frac{1}{\pi^{3/2} v_0^3} \exp{\left(-\frac{(\bs{v-\bs{v}_{\text{lab}}})^2}{v_0^2}\right)}, \label{eq:f_lab_velocity}
%\end{equation}
%where the velocity of the lab frame is~$\bs{v}_{\text{lab}} = |\bs{v}_{\text{lab}}| \bs{\hat{z}}$, and we have ignored the escape velocity cut-off. In our simulations, we take the isotropic velocity dispersion of the local UBDM to be determined by the characteristic virial velocity $v_0\approx 220~\text{km}/\text{s}$, and $\bs{v}_{\text{lab}}$ to be dominated by the motion of the Sun in the galactic frame, $|\bs{v}_{\text{lab}}| \approx 233~\text{km}/\text{s}$.


% Motivate the interest on |\varphi|^2 and \bs{\nabla} |\varphi|^2
The total UBDM field $\varphi(\bs{r},t)$ is given by the superposition of the wavefunctions of $N$ individual bosons as described by Eq.\,\eqref{eq:single-boson-field}. Sufficiently strong self-interactions could affect the coherence properties of the net UBDM field. However, since these interactions are expected to be relatively weak~\cite{hui2021wave,Bohua2014}, they are commonly neglected in studies of direct detection searches~\cite{foster2021,derevianko2018detecting,lisanti2021stochastic}, as in this work.  Here, our interest lies in quadratic interactions with the field, proportional to $\varphi^2(\bs{r},t)$ or $\bs{\nabla} \varphi^2(\bs{r},t)$. These quantities have two terms: one near-dc component and one fast oscillating component at $\approx 2\omega_c$. We consider sensors with a limited bandwidth $\Delta \omega \ll \omega_c$, such that the fast oscillating terms can be ignored. Therefore, only the near-dc component (denoted by the subscript~$s$) of $\varphi^2$ and $\bs{\nabla} \varphi^2$ is considered. Analytic expressions for these quantities are presented in Appendix~\ref{app:calculation}.
%Using this approximation, the near-dc component (denoted by the subscript~$s$) of $\varphi^2$ and $\bs{\nabla} \varphi^2$ can be written as
%\begin{align}
%    \varphi_s^2(\bs{r},t) &= \frac{\varphi_0^2}{2N} \sum_{n,m=1}^N \cos \prn{\omega_{nm} t -\bs{k}_{nm} \cdot \bs{r}  +\theta_{nm}},\label{eq:field-squared}\\
%    \bs{\nabla} \varphi_s^2(\bs{r},t) &=  \frac{\varphi_0^2}{2N} \sum_{n,m=1}^N   \bs{k}_{nm} \sin \prn{\omega_{nm} t -\bs{k}_{nm} \cdot \bs{r} +\theta_{nm}}, \label{eq:gradient-field-sqr} 
%\end{align}
%where $\omega_{nm}= \omega_{n} - \omega_{m}$, $\bs{k}_{nm} = \bs{k}_{n} - \bs{k}_{m}$, and $\theta_{nm}=\theta_{n} - \theta_{m}$. 
%Since the sensors are assumed to be within the same coherence patch (such that $\Delta\bs{k} \cdot \Delta\bs{r} \approx 0$, where $\Delta \bs{k}$ is the characteristic spread of values in $\bs{k}_{nm}$ and $\Delta \bs{r}$ is the difference in the position vectors for the pair of sensors at $\boldsymbol{r}_n$ and $\boldsymbol{r}_m$), the $\bs{r}$ dependence can be neglected and we can evaluate the expressions at $\bs{r}=0$ in the following calculations~\cite{TruckNote}\nocite{grotti2018geodesy,takamoto2020test}.

% Introduce the degree of first-order coherence and coherence time

The signal measured with each sensor would have a small UBDM-related component $\kappa\, \xi(t)$, where $\kappa$ accounts for the coupling of the sensor to the UBDM field, and $\xi(t)$ is either $\varphi^2_s$ (scalar interaction) or $\hat{\bs{m}} \cdot \bs{\nabla} \varphi^2_s$ (pseudoscalar gradient interaction, where $\hat{\bs{m}}$ represents the sensitive direction of the sensor). The correlations between measurable signals produced in different sensors by a UBDM field can be quantified using the degree of first-order coherence $g^{(1)}(\tau)$ for different delay times $\tau$,
\begin{equation}
    g^{(1)}(\tau) = \frac{\langle \xi(t) \xi(t+\tau) \rangle_t}{\langle \xi^2 \rangle_t}~,
    \label{eq:first-order-coherence-definition}
\end{equation}
where $\abrk{\cdots}_t$ denotes the time average. The value of $g^{(1)}(\tau)$ is a measure of the degree of correlation between $\xi(t)$ and $\xi(t+\tau)$. The coherence time $\tau_c$ is calculated from the properties of $g^{(1)}(\tau)$ as described in Appendix~\ref{app:similarity}. 

%The characteristic coherence time of the field $\varphi$ is 
%\begin{equation}
%    \tau_\varphi \approx \frac{2 \hbar}{ m_\varphi v_0^2},
%    \label{eq:coherence_time}
%\end{equation}
%which is used as a benchmark timescale throughout the text.

%To illustrate the stochastic properties of $\bs{\nabla} \varphi_s^2(0,t)$ %and $\varphi_s^2(0,t)$, their time evolution was simulated (details in %Appendix~\ref{app:calculation}). Plots of $g^{(1)}(\tau)$ for %$\varphi_s^2(t)$ and for projections of $\bs{\nabla} \varphi_s^2(t)$ onto %parallel and perpendicular directions with respect to $\bs{v}\ts{lab}$ can %be seen in Fig.\,\ref{fig:g1}. Additionally, for the simplified case where %$|\bs{v}_{\text{lab}|} \gg v_0$, an analytical expression for %$g^{(1)}(\tau)$ can be found in Appendix~\ref{app:analytic}. Note that, as %seen in Fig.\,\ref{fig:g1} and discussed in detail in %Appendix~\ref{app:similarity}, the coherence time $\tau_c$ of $\bs{\nabla} %\varphi_s^2(0,t)$ and $\varphi_s^2(0,t)$ is approximately half of that for %the field $\varphi_s$. 
%
%\begin{figure}[ht]
%\center
%\includegraphics[width=\columnwidth,trim={0 5mm 0 3mm},clip]{Coherence.pdf}
%\caption{\small{ Degree of first-order coherence as a function of delay %time $\tau$ for $\varphi_s^2$ and different projections of the gradient %$\bs{\nabla} \varphi_s^2$ relative to $\bs{v}_\ts{lab}$. Each curve is the %result of 100~averages simulating $10^3$ particles, where the mean was %subtracted (details in Appendix~\ref{app:calculation}). The approximate %values of the coherence times are given in colors matching their respective %plot traces.}}
%\label{fig:g1}
%\end{figure}

%Propose the search method
A possible method to look for UBDM is to use multi-sensor intensity interferometry to measure the cross-correlation between time-series data from different sensors.
When using pairs of geographically distributed sensors, a correlated global background field will produce a nonzero cross-correlation $g^{(1)}_{AB}(\tau)$ between sensors $A$ and $B$ proportional to $g^{(1)}(\tau)$, as discussed in Appendix~\ref{app:search}. Note that uncorrelated noise in the sensors will reduce the expected value of $g^{(1)}_{AB}(0)$ in the presence of a UBDM signal, making it smaller than the maximum value of one (see Appendix~\ref{app:search}). 
In the case of the gradient coupling, a relative misalignment of the sensors' sensitive axes also leads to a reduction in the value of $g^{(1)}_{AB}(0)$ (see Appendix~\ref{app:AngleDep}). 
In order to distinguish a correlated signal from uncorrelated noise,  $g^{(1)}_{AB}(0)$ can be compared with $g^{(1)}_{AB}(\tau \gg \tau_\varphi)$, where $\tau_\varphi$ is the coherence time of the UBDM field (Appendix~\ref{app:similarity}). 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\section{Accessible ultralight bosonic dark matter parameter space}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%In this section, we show that existing networks of clocks and magnetometers have sufficient sensitivity to probe unexplored parameter space describing UBDM by searching for correlated stochastic fluctuations as described above.

\medskip

\noindent \emph{Accessible UBDM parameter space.~---~}Existing sensor networks have sufficient sensitivity to probe experimentally unexplored parameter space describing UBDM by searching for correlated stochastic fluctuations using intensity interferometry.

%----------------------------------------------------------------
\begin{figure}[t]
\center
\includegraphics[width=\columnwidth]{IntensityInterferometrySensGNOME.pdf}
\caption{\small{Estimated parameter space describing ALP dark matter that can be probed by GNOME (dashed line, purple shaded region) and Advanced GNOME (dotted line, light blue shaded region) measuring for $\approx 100$~days using $N_m = 10$ magnetometers. GNOME and Advanced GNOME are sensitive to the interaction of the ALP field with proton spins described by Eq.\,\eqref{eq:quadratic-Hamiltonian}; $f_q$ parameterizes the ALP-nucleon coupling strength. The vertical dashed red line marks the Compton frequency and mass for which the ALP coherence length equals the Earth's diameter. The vertical dashed blue line marks the Compton frequency and mass for which $\tau_c \approx 24~{\rm hours}$. The dark red shaded region shows constraints from the Noble and Alkali Spin Detectors for Ultra-light Coherent darK matter (NASDUCK) experiment \cite{bloch2022new}. The dark green shaded area represents astrophysical bounds on spin-dependent ALP interactions with nucleons \cite{Oli08,chang2018supernova}. Note, however, that there are theoretical scenarios where these astrophysical bounds can be circumvented \cite{derocco2020exploring}.}}
\label{Fig:sensitivity-GNOME}
\end{figure}
%Note that there are also experimental constraints for lower $m_\varphi$ and $f_q$ from the Cosmic Axion Spin Precession Experiment (CASPEr) \cite{wu2019search,garcon2019constraints} as well as constraints competitive with the projected GNOME sensitivity obtained from reinterpretation \cite{bloch2020axion} of comagnetometer data used for other tests of fundamental physics \cite{kornack2005test,vasilakis2011precision,Bro10}.

%Estimated parameter space describing ALP dark matter that can be probed by GNOME (dashed line, purple shaded region) and Advanced GNOME (dotted line, light blue shaded region) in $\approx 100$~days of searching for correlated stochastic fluctuations using $N_m = 10$ magnetometers. GNOME and Advanced GNOME are sensitive to the interaction of the ALP field with proton spins described by Eq.\,\eqref{eq:quadratic-Hamiltonian}; $f_q$ parameterizes the ALP-nucleon coupling strength. The vertical dashed red line marks the Compton frequency and mass for which the ALP coherence length equals the Earth's diameter, $\lambda\ts{coh} \approx 2R_E$, corresponding to a characteristic coherence time scale for fluctuations of $\bs{\nabla} \varphi^2_s$ of $\tau_c \approx 30~{\rm s}$. The vertical dashed blue line marks the Compton frequency and mass for which $\tau_c \approx 24~{\rm hours}$; for $m_\varphi$ much smaller than this value, the pseudo-magnetic field is quasi-static in the Galactic rest frame and thus the signals are frequency upconverted in the sensor network due to Earth's rotation. The dark red shaded region shows constraints from the Noble and Alkali Spin Detectors for Ultra-light Coherent darK matter (NASDUCK) experiment \cite{bloch2022new}. The dark green shaded area represents astrophysical bounds on spin-dependent ALP interactions with nucleons \cite{Oli08,chang2018supernova}. Note, however, that there are theoretical scenarios where these astrophysical bounds can be circumvented \cite{derocco2020exploring}, and thus laboratory searches are complementary to astrophysical observations. 
%----------------------------------------------------------------

%----------------------------------------------------------------
\begin{figure}[t]
\center
\includegraphics[width=\columnwidth]{StochasticFluctuationsSensClock.pdf}
\caption{\small{Estimated parameter space describing UBDM fields that can be probed by an optical clock network such as those described in Refs.\,\cite{collaboration2021frequency,lisdat2016clock} (dotted line, light purple shaded region) in $\approx 100$~days of searching for correlated stochastic fluctuations using $N_c = 10$ clocks, not accounting for (anti)screening from back-action \cite{hees2018violation,stadnik2020new}, which can play a significant role near Earth's surface above the long-dashed blue line as indicated by the blue arrow. Clocks are sensitive to the interactions described by Eq.\,\eqref{eq:scalar-Lagrangian}; $\Lambda_\gamma$ parameterizes the strength of the coupling of the ultralight bosons to photons. The vertical dashed red line marks the Compton frequency and mass for which the ultralight boson's coherence length equals the Earth's diameter. The dark green shaded area represents astrophysical bounds on such quadratic scalar interactions between ultralight bosons and photons from stellar cooling and observations of supernova 1987a \cite{Oli08,chang2018supernova}; the light green shaded region represents bounds from Big Bang nucleosynthesis (BBN) \cite{stadnik2015can}.}}
\label{Fig:sensitivity-clocks}
\end{figure}
%----------------------------------------------------------------

Atomic magnetometers can search for ALP fields by detecting Zeeman shifts caused by the interaction described in Eq.\,\eqref{eq:quadratic-Hamiltonian}. In analogy with the Zeeman Hamiltonian, the gradient of the square of the ALP field acts as a ``pseudo-magnetic field'' $\bs{\mc{B}}_q$ given by
\begin{align}
    \bs{\mc{B}}_q \approx \mp\frac{2 \hbar^2 c^2}{g_F\mu_B f_q^2} \bs{\nabla} \varphi^2(\bs{r},t)~,
    \label{eq:pseudo-magnetic-field}
\end{align}
where $g_F$ is the Land\'e factor, $\mu_B$ is the Bohr magneton (or, for nuclear-spin-based magnetometers, the nuclear magneton). The projection of the near-dc component of $\bs{\mc{B}}_q$ along the sensitive axis of a magnetometer defined by the unit vector $\hat{\bs{m}}$ can be estimated in a manner similar to that discussed in, for example, Ref.\,\cite{gramolin2021spectral}, by evaluating the sum in Eq.\,\eqref{eq:gradient-field-sqr}, yielding a characteristic magnitude (with an average value of zero) of %\DK{I think that we should include a factor of $1/\sqrt{3}$ below for the average over the random direction of the gradient. This is derived in Appendix~\ref{app:AngleDep}, see Eq.~\eqref{eq:angledep}. Then that cancels a factor of 2 that used to appear in the numerator. So I got rid of the 2. I don't think we need to explain it, do we?}
\begin{align}
    \hat{\bs{m}} \cdot \bs{\mc{B}}_q \sim \frac{\hbar^3 \rho\ts{dm} v_0}{g_F \mu_B m_\varphi f_q^2}~.
    \label{eq:ALP-intensity-gradient}
\end{align}
In the derivation of the above equation we assumed that frequency and wave-vector are uncorrelated. The accuracy of this approximation is discussed in Appendix~\ref{app:similarity}. Nonetheless, Eq.\,\eqref{eq:ALP-intensity-gradient} is suitable for a rough estimate of the sensitivity of a magnetometer network to such UBDM, given that $|\bs{v}\ts{lab}| \approx v_0$.
%In the derivation of the above equation we assumed that the average spread %of values of $\hat{\bs{m}}\cdot\bs{k}_{nm}$ is $\approx m_\varphi %v_0/\hbar$. This estimate implicitly assumes that $\omega_{nm}$ and %$\bs{k}_{nm}$ are uncorrelated, and thus the accuracy of this approximation %varies with $\bs{v}\ts{lab}$ as discussed in Appendix~\ref{app:similarity}. %Nonetheless, Eq.\,\eqref{eq:ALP-intensity-gradient} is suitable for a rough %estimate of the sensitivity of a magnetometer network to such UBDM, given %that $|\bs{v}\ts{lab}| \approx v_0$.


%In order to estimate the sensitivity of a magnetometer network, for simplicity we assume $N_m$ identical sensors having the same directional sensitivity and dominated by Gaussian noise with the same variance (of course, this is not the typical case for real networks, these feature different directional sensitivities -- see Appendix~\ref{app:AngleDep} -- and are affected by $1/f$ noise).
%In the cases of interest, the coherence length of the UBDM is much larger than the spacing between the sensors, so the UBDM signal will be identical in all sensors. 
%To understand the scaling of the sensitivity with $N_m$, $\tau_\varphi$, and total acquisition time $T$, suppose that we divide the network into two distinct groups each with $N_m/2$ sensors and average the data in each group. 
%Furthermore, suppose that the time-series data are binned in $\tau_\varphi$-long segments and time-averaged in each bin. 
%Based on this approach, in the absence of a correlated UBDM signal, each group of sensors will exhibit a bin-to-bin variance in the measured magnetic field of approximately $\delta B / \sqrt{\tau_\varphi N_m/2} \sim \delta B / \sqrt{\tau_\varphi N_m}$, where $\delta B$ is the sensitivity of a single magnetometer in units of magnetic field strength times the square root of time. For a total acquisition time $T$, there will be $N_b = T/\tau_\varphi$ bins.
%The expected residual from noise in the cross-correlation between the two groups provides an estimate of the network resolution, which in turn gives the minimum detectable pseudo-magnetic field squared 
%\begin{align}
%    \abrk{ \mc{B}_q({\rm{min}})^2 }_t \approx \frac{\delta B^2}{N_m \tau_\varphi}\frac{1}{\sqrt{N_b}} \approx \frac{\delta B^2}{N_m \sqrt{\tau_\varphi T}}~.
%    \label{eq:min-field}
%\end{align}
%An in-depth discussion of the $T$ and $N_m$ scaling for a similar case can be found in Ref.~\cite{derevianko2018detecting}.

The sensitivity of a sensor network depending on the number of sensors ($N_m$), the UBDM field coherence time ($\tau_\varphi$), and total acquisition time ($T$) is discussed in Appendix~\ref{app:search}. Combining Eqs.~\eqref{eq:ALP-intensity-gradient} and \eqref{eq:min-field}, an estimate for the UBDM coupling constant to which a magnetometer network would be sensitive is given by
\begin{align}
    f_q^2 \lesssim \frac{\hbar^3 \rho\ts{dm} v_0 }{g_F\mu_B m_\varphi \delta B} \prn{\tau_\varphi T}^{1/4} \sqrt{N_m}~.
    \label{eq:f_q-sens-mags}
\end{align}
Figure~\ref{Fig:sensitivity-GNOME} shows sensitivity estimates for the Global Network of Optical Magnetometers for Exotic physics searches (GNOME) based on alkali vapor magnetometers with $\delta B \approx 100~{\rm fT/\sqrt{Hz}}$ and the Advanced GNOME network based on noble gas comagnetometers with $\delta B \approx 1~{\rm fT/\sqrt{Hz}}$, assuming $T=100$~days and $N_m = 10$. Note that for $\tau_c \gg 24$\,hours, the signal amplitude is partially modulated at the frequency of Earth's rotation since the signals are $\propto \bs{\hat{m}}\cdot\bs{\mc{B}}_q$ and $\hat{\bs{m}}$ rotates with the Earth while $\bs{\mc{B}}_q$ does not, which can in principle enable the detection of UBDM with coherence times much longer than a day. Notable is the extent to which GNOME and Advanced GNOME can probe UBDM with Compton frequencies far beyond the nominal sensor bandwidths.

Optical atomic clocks are an example of a sensor that can search for scalar fields through the apparent variation of fundamental constants as described in Eqs.\,\eqref{eq:scalar-mass-variation} and \eqref{eq:scalar-alpha-variation}, due to, for example, the variation of the fine-structure constant $\alpha$ and relativistic effects (see Ref.\,\cite{safronova2018search} and references therein). For example, the fractional frequency variation in an atomic clock due to variation of the fine-structure constant $\alpha$ is given by
\begin{align}
    \frac{\delta \nu(t)}{\nu} = \kappa_\alpha \frac{\delta \alpha(t)}{\alpha}~,
    \label{eq:frac-freq-variation-alpha-1}
\end{align}
where $\nu$ is the clock frequency and $\kappa_\alpha$ is a dimensionless sensitivity coefficient that depends on the type of clock: $\kappa_\alpha \approx 2$ for most current optical atomic clocks, but note that there are exceptions, such as the proposed clock with $\kappa_\alpha \approx -15$ described in Ref.~\cite{Safronova2018Apr}, and the possibility of future clocks based on highly charged ions \cite{kozlov2018highly} or a Th nuclear transition \cite{peik2021nuclear} that could have orders of magnitude larger values of $\kappa_\alpha$. 

It is important to note that the sensitivity of intensity interferometry can be significantly impacted by back-action of the surrounding matter density on the scalar field as pointed out in Refs.\,\cite{stadnik2020new,hees2018violation} and also discussed in Refs.\,\cite{Oli08,hinterbichler2010screening,jaffe2017testing}. The accessible range of parameter space for current optical clocks near the surface of the Earth is well within the regime where such back-action effects are significant (above the long-dashed blue line in Fig.\,\ref{Fig:sensitivity-clocks}, see Appendix~\ref{app:back-action}). However, for the range of boson masses and coupling constants considered in the present work, it turns out for a space-based network of sensors \cite{Schkolnik2022Apr} the screening effects can be largely neglected \cite{stadnik2020new}, and so for simplicity we consider such a space-based network in our sensitivity estimates.

Assuming the effect described by Eq.\,\eqref{eq:scalar-alpha-variation} and a scalar field that makes up the entirety of the dark matter density, the amplitude of the fractional frequency variation is given by
\begin{align}
    \frac{\delta \nu}{\nu} \approx \kappa_\alpha \frac{2 \hbar^3 \rho\ts{dm}}{\Lambda_\gamma^2 m_\varphi^2 c}~.
    \label{eq:frac-freq-variation-alpha-2}
\end{align}
Optical clock networks, with $N_c$ independent clocks, can achieve a fractional frequency uncertainty~\cite{collaboration2021frequency,lisdat2016clock}
\begin{align}
    \frac{\delta \nu}{\nu} \approx \frac{3 \times 10^{-16}}{(\tau_\varphi T)^{1/4}\sqrt{N_c}}~,
    \label{eq:frac-freq-variation-clock-sens}
\end{align}
which translates to the sensitivity to the quadratic scalar coupling constant shown in Fig.\,\ref{Fig:sensitivity-clocks}. Appendix~\ref{app:SensiticityDifference} offers a heuristic argument for the significant  sensitivity difference between atomic clock and magnetometer networks to the respective coupling parameters $\Lambda_\gamma$ and $f_q$.

%Ultimately, the sensitivity of sensor networks used to search for correlated signals from UBDM may be limited by systematic effects due to prosaic natural phenomena. 
%Known natural phenomena that could generate noise with long-range correlations include, for example, time-dependent electromagnetic fields associated with cavity resonances of the conducting Earth-ionosphere cavity \cite{fedderke2021earth} (such as the Schumann resonances \cite{schumann1952strahlungslosen}) and vibrational noise due to free oscillations of the Earth excited by large earthquakes \cite{hu2020network} (such as the ``breathing'' mode of the Earth at $\approx 800~{\rm \mu Hz}$ \cite{dziewonski1981preliminary,rosat2007geographical}). 
%In the event of a non-null result, auxiliary measurements with other instruments may be able to rule out such systematic effects. 
%For example, GNOME uses unshielded magnetometers to monitor the magnetic environment near the shielded dark matter sensors to veto signals from anomalously large local magnetic field excursions \cite{afach2018characterization}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Conclusion}

\medskip

\noindent\emph{Conclusion.~---~}In summary, we propose a new method to search for UBDM by using intensity interferometry with sensor networks. We show that when the sensors measure signals quadratic in the UBDM field, there is a near-dc component of the signal that enables finite-bandwidth sensors to search for UBDM with Compton frequencies many orders of magnitude larger than possible if a traditional search for signals oscillating at the Compton frequency is carried out. Here we have focused on quadratic UBDM interactions and sensors with a linear response; however, the results are also valid for linear interactions and sensors that respond quadratically to the field (square-law detectors). The method of intensity interferometry is intrinsically broadband, with the potential to search for UBDM with particle masses ranging over many orders of magnitude without having to probe individual narrow frequency bands. UBDM searches with intensity interferometry using existing sensor networks can probe unexplored parameter space.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\section*{Acknowledgements}
\vspace{12pt}
The authors are sincerely grateful to Grzegorz Lukasiewicz, Jason Stalnaker, Ibrahim Sulai, Maxim Pospelov, Arran Phipps, Ben Buchler, Ron Folman, and Menachem Givon for enlightening discussions. The authors also thank Tatum Wilson, Rayshaun Preston, Christopher Verga, and Mario Duenas for early work on simulations. This work was supported by the U.S. National Science Foundation under grant PHYS-2110388, by the Cluster of Excellence ``Precision Physics, Fundamental Interactions, and Structure of Matter'' (PRISMA+ EXC 2118/1) funded by the German Research Foundation (DFG) within the German Excellence Strategy (Project ID 39083149), by the German Federal Ministry of Education and Research (BMBF) within the Quantumtechnologien program (Grant No. 13N15064), by the European Research Council (ERC) under the European Union Horizon 2020 research and innovation program (project Dark-OST, grant agreement No 695405), and by the DFG Project ID 423116110.
The authors at Boston University acknowledge support from the Simons Foundation Grant No. 641332, the National Science Foundation CAREER Award No. PHY-2145162, the John Templeton Foundation Grant No. 60049570, and the U.S. Department of Energy, Office of High Energy Physics program under the QuantISED program, FWP 100495. The work of YVS was supported by the Australian Research Council under the Discovery Early Career Researcher Award DE210101593. The work of SP was supported by the National Science Centre of Poland within the grant No. 2020/39/B/ST2/01524.



==> VersionControl/maintext_long.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Introduce the dark matter problem
A wide variety of evidence suggests the existence of dark matter, an invisible substance that constitutes a large fraction of the matter in the Universe \cite{Fen10,spergel2015dark,graham2015experimental}. Despite decades of research, its microscopic nature remains unknown. A promising hypothesis is that dark matter predominantly consists of ultralight bosons, particles with masses $m_\varphi \ll 1~{\textrm{eV}}/c^2$, such as axions~\cite{Pre83,Abb83,Din83}, axion-like particles (ALPs)~\cite{Gra15,co2020predictions}, or hidden photons~\cite{holdom1986two,cvetivc1996implications,Okun1982}. Ultralight bosons can couple to Standard Model (SM) particles through a variety of ``portals'' \cite{graham2016dark,safronova2018search}, which have been used to search for ultralight bosonic dark matter (UBDM) --- see, for example, Refs.\,\cite{Asz01,Asz10,budker2014proposal,Sik14,chaudhuri2015radio,geraci2016sensitivity,abel2017search,wu2019search,garcon2019constraints,phipps2020exclusion,manley2020searching,crescini2020axion,braine2020extended,backes2021quantum,antypas2021probing,roussy2021experimental,Ayb21CASPErE,gramolin2021search}.

% Advantage of intensity measurement
Numerous experiments looking for UBDM are based on resonant systems, which require an accurate tuning to the unknown Compton frequency, $\omega_c = m_\varphi c^2 / \hbar$, in order to be sensitive to UBDM. Therefore, a time-consuming scan of tunable parameters must be performed to search a wide range of masses. However, if a search is based on the measurement of the \emph{intensity} of the UBDM, part of the signal is down-converted to near-zero frequency~\cite{stadnik2015can,hees2018violation}, regardless of the particular Compton frequency of the UBDM. Furthermore, assuming the standard halo model~\cite{Zyla:2020zbs,evans2019refinement,drukier1986detecting}, there are stochastic fluctuations of this near-dc component~\cite{Centers2019,derevianko2018detecting,foster2018,hui2021wave,schive2014cosmic,turner1990periodic,o2017axion,lisanti2021stochastic,gramolin2021spectral}. The linewidth of this spectral near-dc feature is comparable to the spectral linewidth of the UBDM field, $\approx \! \! 10^6$~times smaller than $\omega_c$. Looking for this near-dc feature allows sensors with a limited bandwidth to probe UBDM with masses $\approx \! \! 10^6$~times larger than searching for direct field oscillations at $\omega_c$.%(as in existing and planned experiments reviewed in, for example, Refs.\,\cite{safronova2018search,graham2015experimental,irastorza2018new}).%\footnote{Note that although Refs.\,\cite{derevianko2018detecting,foster2021dark} consider UBDM interferometry using sensor networks, they do not consider the intensity interferometry as we do here.}

%This method is limited by the fact that large Compton frequencies produce a broad dc feature, which eventually causes an attenuation of the signal due to the finite bandwidth of the detectors.

% quadratic Lagrangian for clocks
The frequency down-conversion discussed above occurs naturally when considering quadratic portals where the interaction with SM particles is proportional to the square of the UBDM field\,\cite{stadnik2015can,hees2018violation,Pos13,Der14,Oli08,Sta15,dailey2021quantum}. A spin-0 field $\varphi(\bs{r},t)$ can interact with SM fermions and electromagnetic fields according to the phenomenological quadratic scalar Lagrangian
\begin{align}
    \mc{L}_s = \hbar c \prn{\pm \frac{m_f c^2}{\Lambda_f^2} \bar{\psi}_f\psi_f \pm \frac{1}{4 \Lambda_\gamma^2} F_{\mu\nu}^2} \varphi^2(\bs{r},t)~,
    \label{eq:scalar-Lagrangian}
\end{align}
where $\Lambda_f$ and $\Lambda_\gamma$ parametrize the couplings to fermions and photons, respectively, where the $\pm$ indicates the sign of the coupling, $m_f$ is the fermion mass, $\psi_f$ is the fermion field, and $F_{\mu\nu}$ is the Faraday tensor.

% Effect of the interaction for clocks
The effects of the interactions described by Eq.\,\eqref{eq:scalar-Lagrangian} can be understood in terms of redefinitions of the effective fermion masses and the fine-structure constant $\alpha$\,\cite{stadnik2015can,Der14}:
\begin{align}
    m_f^{({\rm{eff}})} (\bs{r},t) & = m_f \prn{ 1 \mp \frac{\hbar c}{\Lambda_f^2} \varphi^2(\bs{r},t) }~, \label{eq:scalar-mass-variation} \\
    \alpha^{({\rm{eff}})} (\bs{r},t) & = \alpha \prn{ 1 \pm \frac{\hbar c}{\Lambda_\gamma^2} \varphi^2(\bs{r},t) }~. \label{eq:scalar-alpha-variation}
\end{align}
Variations of $m_f^{({\rm{eff}})}$ and $\alpha^{({\rm{eff}})}$ can be measured with atomic clocks or interferometers~\cite{Der14,wcislo2016experimental,roberts2017search,roberts2020search,dailey2021quantum,nagano2019axion,aiello2021constraints,badurina2020aion,Stadnik2016,Grote2019,Vermeulen2021,Sta15}, or generally by direct comparison of systems with different dependence on these fundamental constants~\cite{Antypas2019Oct,Antypas2020Apr,antypas2021probing,Oswald2021Nov,Tretiak2022Jan}.

% Quadratic interaction with magnetometers
Additionally, a UBDM field with pseudoscalar interactions (such as an axion or ALP field) can interact with SM fermions via the phenomenological interaction Lagrangian~\cite{dailey2021quantum}
\begin{align}
    \mc{L}_\varphi = \pm\frac{1}{f_q^2} \underbrace{\bar{\psi}_f \gamma^\mu\gamma_\ts{5} \psi_f}_{{\substack{\text{fermion axial} \\ \text{vector current}}}} \partial_\mu \varphi^2(\bs{r},t)~,
    \label{eq:pseudoscalar-Lagrangian}
\end{align}
where $f_q$ parameterizes the coupling to fermion spins,  $\gamma^\mu$ and $\gamma_\ts{5}$ are the Dirac matrices. %(note that $\bar{\psi}_f \gamma^\mu\gamma_\ts{5} \psi_f$ is the fermion axial vector current).
In the nonrelativistic limit, Eq.\,\eqref{eq:pseudoscalar-Lagrangian} yields the interaction Hamiltonian
\begin{align}
    \mc{H}_\varphi = \mp\frac{2\hbar^2c^2}{f_q^2} \bs{S} \cdot \bs{\nabla} \varphi^2(\bs{r},t)~,
    \label{eq:quadratic-Hamiltonian}
\end{align}
which shows that the gradient of the square of the pseudoscalar field couples to a fermion spin $\bs{S}$ similarly to a magnetic field. Here $\bs{\nabla} \varphi^2(\bs{r},t)$ plays the role of a pseudo-magnetic field. Thus, such pseudoscalar fields can be searched for in the spin dynamics of electrons or nuclei. While a variety of sensors could be used, here we focus on atomic (nuclear) magnetometers since these are intrinsically sensitive to Zeeman shifts~\cite{Pos13,Pus13,afach2018characterization,kimball2018searching,masia-roig_analysis_2020,afach2021search,Jiang2021Dec}.

% Networks to detect the stochastic fluctuations
The effects described by Eqs.\,\eqref{eq:scalar-mass-variation},~\eqref{eq:scalar-alpha-variation},~and~\eqref{eq:quadratic-Hamiltonian} are proportional to the UBDM intensity and exhibit \mbox{near-dc} stochastic amplitude fluctuations. Although measuring low-frequency signals is technically challenging due to multiple sources of low-frequency noise, an array of independent, geographically distributed sensors will tend to have uncorrelated noise. In contrast, the slowly-changing UBDM intensity will lead to a common-mode fluctuating signal present in all detectors within a coherence length of one another, which will appear in correlations between the sensors. We advocate for the use of networks of sensors to search for these stochastic fluctuations. There are existing and proposed dark matter searches sensitive to these interactions using networks consisting of a variety of sensor types such as atomic clocks~\cite{Der14,wcislo2016experimental,roberts2017search,roberts2020search,dailey2021quantum,collaboration2021frequency}, atomic magnetometers~\cite{Pos13,Pus13,afach2018characterization,kimball2018searching,masia-roig_analysis_2020,afach2021search,fedderke2021earth,fedderke2021search,arza2021earth}, gravimeters~\cite{hu2020network,mcnally2020constraining,horowitz2020gravimeter}, laser interferometers~\cite{hall2018laser,nagano2019axion,aiello2021constraints,Stadnik2016,Grote2019,Vermeulen2021,Sta15}, and atom interferometers \cite{badurina2020aion}. The methodology described below is analogous to Hanbury Brown and Twiss intensity interferometry\,\cite{brown1956question}, and can be used to dramatically expand the range of UBDM Compton frequencies that particular sensors can probe~\cite{InterferometryNote}\nocite{derevianko2018detecting,foster2021dark}.

% Suggest the use of moving trucks
%If there are UBDM-related cross-correlations discovered, further analysis can narrow the range of possible boson masses. (For example, by measuring the coherence time and length, for which portable sensors could be employed as in Refs.\,\cite{grotti2018geodesy,takamoto2020test}.)


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section*{Stochastic properties of the ultralight bosonic dark matter field}
\label{sec:field-properties}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Introduce our treatment of the UBDM field

\medskip

\noindent \emph{Stochastic properties of the UBDM field.~---~}The properties of the UBDM field can be derived using the framework described in Refs.\,\cite{Centers2019,derevianko2018detecting,foster2018,hui2021wave,schive2014cosmic,turner1990periodic,o2017axion,lisanti2021stochastic,gramolin2021spectral}. In brief, assuming that UBDM does not interact with itself, each individual particle can be treated as an independent wave. In this scenario, the UBDM field is well described by a superposition of these individual waves.

% Field produced by one boson
If the local dark-matter energy density $\rho\ts{dm}$ results from $N$ ultralight bosons of mass $m_\varphi$, the field contribution of an individual boson $n$ is
\begin{align}
    \varphi_n(\bs{r},t) \approx \frac{\varphi_0}{\sqrt{N}} \cos\prn{ \omega_n t - \bs{k}_n \cdot \bs{r} + \theta_n }~,
    \label{eq:single-boson-field}
\end{align}
where the boson field amplitude is given by~\cite{Gra13}
\begin{align}
    \varphi_0 = \frac{\hbar}{m_\varphi c} \sqrt{ 2 \rho\ts{dm} },
    \label{eq:single-ALP-field-amp}
\end{align}
such that the average energy density in the UBDM field comprises the totality of the local dark matter. Here, $\bs{k}_n = m_\varphi \bs{v}_n /  \hbar$ is the wave vector corresponding to $\bs{v}_n$, the velocity of the $n^\text{th}$ boson in the laboratory frame, while $\theta_n$ is a phase associated with each boson, that is distributed between $0$ and $2\pi$. The oscillation frequency of the individual UBDM particles, $\omega_{n}$, is determined mostly by their Compton frequency, $\omega_{c}$. However, the second-order Doppler effect introduces small deviations from $\omega_{c}$, so that
\begin{align}
    \omega_n = \omega_c \prn{ 1 + \frac{\bs{v}_n^2}{2c^2} }.
\end{align}
Therefore, the distribution of $\omega_n$ (and $\bs{k}_n$) is determined by the velocity distribution of the particles as observed in the laboratory frame, which, according to the standard halo model, follows a displaced Maxwell-Boltzmann distribution given by
\begin{equation}
f_{\text{lab}}(\bs{v}) \approx \frac{1}{\pi^{3/2} v_0^3} \exp{\left(-\frac{(\bs{v-\bs{v}_{\text{lab}}})^2}{v_0^2}\right)}, \label{eq:f_lab_velocity}
\end{equation}
where the velocity of the lab frame is~$\bs{v}_{\text{lab}} = |\bs{v}_{\text{lab}}| \bs{\hat{z}}$, and we have ignored the escape velocity cut-off. In our simulations, we take the isotropic velocity dispersion of the local UBDM to be determined by the characteristic virial velocity $v_0\approx 220~\text{km}/\text{s}$, and $\bs{v}_{\text{lab}}$ to be dominated by the motion of the Sun in the galactic frame, $|\bs{v}_{\text{lab}}| \approx 233~\text{km}/\text{s}$.

% Total UBDM field (removed as suggested by Dima and Sasha G. in order to space space. Replaced by a sentence in next paragraph)
%The total UBDM field is given by the superposition %of the $N$ individual bosons,
%\begin{align}
%    \varphi(\bs{r},t) = \frac{a_0}{\sqrt{N}} \sum_{n=1}^N  \cos\prn{ \omega_n t - \bs{k}_n \cdot \bs{r} +\phi_n }.
%    \label{eq:ALPsum}
%\end{align}


% Motivate the interest on |\varphi|^2 and \bs{\nabla} |\varphi|^2
The total UBDM field $\varphi(\bs{r},t)$ is given by the superposition of the wavefunctions of $N$ individual bosons as described by Eq.\,\eqref{eq:single-boson-field}. Here, our interest lies in quadratic interactions with the field, proportional to $\varphi^2(\bs{r},t)$ or $\bs{\nabla} \varphi^2(\bs{r},t)$. These quantities have two terms: one near-dc component and one fast oscillating component at $\approx 2\omega_c$. We consider sensors with a limited bandwidth $\Delta \omega \ll \omega_c$, such that the fast oscillating terms can be ignored. Using this approximation the near-dc component (denoted by the subscript~$s$) of $\varphi^2$ and $\bs{\nabla} \varphi^2$ can be written as
\begin{align}
    \varphi_s^2(\bs{r},t) &= \frac{\varphi_0^2}{2N} \sum_{n,m=1}^N \cos \prn{\omega_{nm} t -\bs{k}_{nm} \cdot \bs{r}  +\theta_{nm}},\label{eq:field-squared}\\
    \bs{\nabla} \varphi_s^2(\bs{r},t) &=  \frac{\varphi_0^2}{2N} \sum_{n,m=1}^N   \bs{k}_{nm} \sin \prn{\omega_{nm} t -\bs{k}_{nm} \cdot \bs{r} +\theta_{nm}}, \label{eq:gradient-field-sqr} 
\end{align}
where $\omega_{nm}= \omega_{n} - \omega_{m}$, $\bs{k}_{nm} = \bs{k}_{n} - \bs{k}_{m}$, and $\theta_{nm}=\theta_{n} - \theta_{m}$. 
Since the sensors are assumed to be within the same coherence patch (such that $\Delta\bs{k} \cdot \Delta\bs{r} \approx 0$, where $\Delta \bs{k}$ is the characteristic spread of values in $\bs{k}_{nm}$ and $\Delta \bs{r}$ is the difference of the position vectors for both sensors), the $\bs{r}$ dependence can be neglected and we can evaluate the expressions at $\bs{r}=0$ in the following calculations~\cite{TruckNote}\nocite{grotti2018geodesy,takamoto2020test}.%\footnote{Note that the spatial dependence for coherence lengths smaller than the Earth's diameter could also be exploited to look for UBDM, for which portable sensors could be employed as in Refs.\,\cite{grotti2018geodesy,takamoto2020test}.}

% Introduce the degree of first-order coherence and coherence time

The signal measured with each sensor would have a small UBDM-related component $\kappa\, \xi(t)$, where $\kappa$ accounts for the coupling of the sensor to the UBDM field, and $\xi(t)$ is either $\varphi^2_s$ (scalar interaction) or $\hat{\bs{m}} \cdot \bs{\nabla} \varphi^2_s$ (pseudoscalar gradient interaction, where $\hat{\bs{m}}$ represents the sensitive direction of the sensor). The correlations between measurable signals produced in different sensors by a UBDM field can be quantified using the degree of first-order coherence $g^{(1)}(\tau)$ for different delay times $\tau$,
\begin{equation}
    g^{(1)}(\tau) = \frac{\langle \xi(t) \xi(t+\tau) \rangle_t}{\langle \xi^2 \rangle_t}~,
    \label{eq:first-order-coherence-definition}
\end{equation}
where $\abrk{\cdots}_t$ denotes the time average. The value of $g^{(1)}(\tau)$ is a measure of the degree of correlation between $\xi(t)$ and $\xi(t+\tau)$. 
%\DK{My first proposal is to move all the details about the coherence time to Appendix B, I think 194 Number of math displayed: 20 it is somewhat less essential to the overall narrative. I think this trims about 550 words including the figure.}
The characteristic coherence time of the field $\varphi$ is 
\begin{equation}
    \tau_\varphi \approx \frac{2 \hbar}{ m_\varphi v_0^2},
    \label{eq:coherence_time}
\end{equation}
which is used as a benchmark timescale throughout the text.
 
 
%\DKDel{Additionally, we will define the coherence time as the power-equivalent width of $g^{(1)}(\tau)$~\cite{loudon2000the,saleh2019fundamentals},}
%\DKDel{\begin{equation}
%    \tau_c = \int_{-\infty}^{+\infty} |g^{(1)}(\tau)|^2 d\tau,
%    \label{eq:coherence_time_def}
%\end{equation}
%which gives a characteristic time scale for the decay of $g^{(1)}(\tau)$. The full width at half maximum of the~$\varphi$ lineshape is $\approx \omega_c v_0^2/c^2$, giving a useful estimation of the coherence time of the field~(the result is exact for a Lorentzian lineshape~\cite{gramolin2021spectral}),}

%\DKDel{\begin{equation}
%    \tau_\varphi \approx \frac{2 \hbar}{ m_\varphi v_0^2},
%    \label{eq:coherence_time}
%\end{equation}
%which will be used as a benchmark timescale throughout the text. Note that there is an ambiguity, up to a factor of $2\pi$, in the definitions of $\tau_c$ used in the literature~\cite{Centers2019}. Because the actual lineshape describing $\varphi$ is expected to be non-Lorentzian \cite{gramolin2021spectral}, $\tau_\varphi$ slightly differs from the coherence time of the field $\varphi$ derived from the simulations. For the considered $\bs{v}_\ts{lab}$, simulations show a coherence time $\approx 1.12(1) \tau_\varphi$.}

To illustrate the stochastic properties of $\bs{\nabla} \varphi^2(0,t)$ and $\varphi^2(0,t)$, their time evolution was simulated (details in Appendix~\ref{app:calculation}). Plots of $g^{(1)}(\tau)$ for $\varphi^2(t)$ and for projections of $\bs{\nabla} \varphi^2(t)$ onto parallel and perpendicular directions with respect to $\bs{v}\ts{lab}$ can be seen in Fig.\,\ref{fig:g1}. Note that, as seen in Fig.\,\ref{fig:g1} and discussed in detail in Appendix~\ref{app:similarity}, the coherence time $\tau_c$ of $\bs{\nabla} \varphi^2(0,t)$ and $\varphi^2(0,t)$ is approximately half of that for the field $\varphi$. %\DKDel{Note that these quantities experience stochastic fluctuations occurring at similar time scales.}
\begin{figure}[ht]
\center
\includegraphics[width=\columnwidth,trim={0 5mm 0 3mm},clip]{Coherence.pdf}
\caption{\small{ Degree of first-order coherence as a function of delay time $\tau$ for $\varphi_s^2$ and different projections of the gradient $\bs{\nabla} \varphi_s^2$ relative to $\bs{v}_\ts{lab}$. Each curve is the result of 100~averages simulating $10^3$ particles, where the mean was subtracted (details in Appendix~\ref{app:calculation}). The approximate values of the coherence times are given in colors matching their respective plot traces.}}
\label{fig:g1}
\end{figure}

% Coherence time of $\varphi^2_s(0,t)$ and gradient
%\DKDel{The coherence time for $\varphi^2_s$ is approximately half of that for the field $\varphi$. This is a result of the field $\varphi^2_s$ being a sum over terms depending on the difference of frequencies $\omega_{nm}$, as opposed to $\varphi$, which only contains terms depending on $\omega_n$. The probability distribution of $\omega_{nm}$ can be calculated as the convolution of the distribution of $\omega_n$ with itself. This results in a distribution for $\omega_{nm}$ that is broader. Consequently, the coherence time is shorter since $g^{(1)}(\tau)$ is given by the Fourier transform of the power spectral density of $\varphi^2_s$ (proportional to the $\omega_{nm}$ distribution), according to the Wiener–Khinchin theorem. The gradient coupling features even shorter coherence times due to the $\bs{k}_{nm}$ factor weighting the contribution of the oscillating terms. Larger $\omega_{nm}$ tends to correspond to larger $\bs{k}_{nm}$: this effectively broadens the power spectral density of $\bs{\nabla} \varphi^2_s$, leading to a shorter coherence time. This is also the reason why parallel and perpendicular components of the gradient have different coherence times~(see~Appendix~\ref{app:similarity}).}

%\DKDel{A formal derivation of $g^{(1)}(\tau)$ for $\varphi^2_s$ and $\bs{\nabla} \varphi^2_s$ in the simplified case where $|\bs{v}_{\text{lab}|} \gg v_0$ can be found in Appendix~\ref{app:analytic}.}

% Relate coherence time of the fields to mass
%\DKDel{The coherence time is also related to the mass of the UBDM particle as can be seen in Eq.\,\eqref{eq:coherence_time}. The relationship between the UBDM mass and the coherence time exhibited by $\varphi^2_s$ and $\bs{\nabla} \varphi^2_s$ is shown in Fig.\,\ref{Fig:massdep}. The coherence times for $\varphi^2_s$ and $\bs{\nabla} \varphi^2_s$ are proportional to the coherence time of $\varphi$, $\tau_\varphi$ as defined in Eq.\,\eqref{eq:coherence_time}. In the case of detection, this could be used to estimate the mass of the UBDM particles. Further discussion on the scaling of the coherence times can be found in Appendix~\ref{app:similarity}.}
%\begin{figure}[ht]
%\center
%\includegraphics[width=\columnwidth,trim={0 5mm 0 3mm},clip]{MassVStc.pdf}
%\caption{\small{Mass dependence of the characteristic delay time at which $g^{(1)}(\tau)=0.5$ for $\varphi_s^2$ and projections of $\bs{\nabla} \varphi_s^2$. Each point is the result of 100~averages simulating $10^3$ particles (details in Appendix~\ref{app:calculation}).}}
%\label{Fig:massdep}
%\end{figure}


%Propose the search method
A possible method to look for UBDM by exploiting these stochastic properties is to use intensity interferometry with multiple sensors to measure the cross-correlation between the time-series data from different sensors.
When using pairs of independent and geographically distributed sensors, a correlated global background field will produce a nonzero cross-correlation $g^{(1)}_{AB}(\tau)$ between sensors $A$ and $B$ proportional to $g^{(1)}(\tau)$, as discussed in Appendix~\ref{app:search}. Note that uncorrelated noise in the sensors will reduce the expected value of $g^{(1)}_{AB}(0)$ in the presence of a UBDM signal, making it smaller than the maximum value of one (see Appendix~\ref{app:search}). 
In the case of the gradient coupling, a relative misalignment of the sensors' sensitive axes also leads to a reduction in the value of $g^{(1)}_{AB}(0)$ (see Appendix~\ref{app:AngleDep}). 
In order to distinguish a correlated signal from uncorrelated noise,  $g^{(1)}_{AB}(0)$ can be compared with $g^{(1)}_{AB}(\tau \gg \tau_\varphi)$. 
%\DK{Cutting the following sentences saves about 70 words, and I don't think they say anything too significant that cant be inferred.} \DKDel{Additionally, the uncertainty in the measurement can be reduced by averaging over many coherence times. Therefore this approach to analysis requires measurement times $T \gg \tau_\varphi$, in practice setting a lower limit on the accessible mass range. However, for low frequencies, the UBDM signal can be directly detected without the need of the frequency down-conversion used here. Furthermore, for a network of many sensors, pairwise measurements can be used to check for consistency.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\section{Accessible ultralight bosonic dark matter parameter space}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%In this section, we show that existing networks of clocks and magnetometers have sufficient sensitivity to probe unexplored parameter space describing UBDM by searching for correlated stochastic fluctuations as described above.

\medskip

\noindent \emph{Accessible UBDM parameter space.~---~}Existing sensor networks have sufficient sensitivity to probe experimentally unexplored parameter space describing UBDM by searching for correlated stochastic fluctuations using intensity interferometry.

%----------------------------------------------------------------
\begin{figure}[t]
\center
\includegraphics[width=\columnwidth]{IntensityInterferometrySensGNOME.pdf}
\caption{\small{Estimated parameter space describing ALP dark matter that can be probed by GNOME (dashed line, purple shaded region) and Advanced GNOME (dotted line, light blue shaded region) in $\approx 100$~days of searching for correlated stochastic fluctuations using $N_m = 10$ magnetometers. GNOME and Advanced GNOME are sensitive to the interaction of the ALP field with proton spins described by Eq.\,\eqref{eq:quadratic-Hamiltonian}; $f_q$ parameterizes the ALP-fermion coupling strength. The vertical dashed red line marks the Compton frequency and mass for which the ALP coherence length equals the Earth's diameter, $\lambda\ts{coh} \approx 2R_E$, corresponding to a characteristic coherence time scale for fluctuations of $\bs{\nabla} \varphi^2_s$ of $\tau_c \approx 30~{\rm s}$. The vertical dashed blue line marks the Compton frequency and mass for which $\tau_c \approx 24~{\rm hours}$; for $m_\varphi$ much smaller than this value, the pseudo-magnetic field is quasi-static in the galactic rest frame and thus the signals are frequency upconverted in the sensor network due to Earth's rotation. The dark red shaded region shows constraints from the Noble and Alkali Spin Detectors for Ultra-light Coherent darK matter (NASDUCK) experiment \cite{bloch2022new}. Note that there are also experimental constraints for lower $m_\varphi$ and $f_q$ from the Cosmic Axion Spin Precession Experiment (CASPEr) \cite{wu2019search,garcon2019constraints} as well as constraints competitive with the projected GNOME sensitivity obtained from reinterpretation \cite{bloch2020axion} of comagnetometer data used for other tests of fundamental physics \cite{kornack2005test,vasilakis2011precision,Bro10}. The dark green shaded area represents astrophysical bounds on spin-dependent ALP interactions with nucleons \cite{Oli08,chang2018supernova}. Note, however, that there are theoretical scenarios where these astrophysical bounds can be circumvented \cite{derocco2020exploring}, and thus laboratory searches are complementary to astrophysical observations. }}
\label{Fig:sensitivity-GNOME}
\end{figure}
%----------------------------------------------------------------

%----------------------------------------------------------------
\begin{figure}[t]
\center
\includegraphics[width=\columnwidth]{StochasticFluctuationsSensClock.pdf}
\caption{\small{Estimated parameter space describing UBDM fields that can be probed by an optical clock network such as those described in Refs.\,\cite{collaboration2021frequency,lisdat2016clock} (dotted line, light purple shaded region) in $\approx 100$~days of searching for correlated stochastic fluctuations using $N_c = 10$ clocks, not accounting for (anti)screening from back-action \cite{hees2018violation,stadnik2020new}, which can play a significant role near Earth's surface above the long-dashed blue line as indicated by the blue arrow. Clocks are sensitive to the interactions described by Eq.\,\eqref{eq:scalar-Lagrangian}; $\Lambda_\gamma$ parameterizes the strength of the coupling of the ultralight bosons to photons. The vertical dashed red line marks the Compton frequency and mass for which the ultralight boson's coherence length equals the Earth's diameter. The dark green shaded area represents astrophysical bounds on such quadratic scalar interactions between ultralight bosons and photons from stellar cooling and observations of supernova 1987a \cite{Oli08,chang2018supernova}; the light green shaded region represents bounds from Big Bang nucleosynthesis (BBN) \cite{stadnik2015can}. Note that there may be nonstandard scenarios where the astrophysical and cosmological bounds could be circumvented \cite{derocco2020exploring,bernal2021alp}, so laboratory experiments are useful complementary probes.}}
\label{Fig:sensitivity-clocks}
\end{figure}
%----------------------------------------------------------------

Atomic magnetometers can search for ALP fields by detecting Zeeman shifts caused by the interaction described in Eq.\,\eqref{eq:quadratic-Hamiltonian}. In analogy with the Zeeman Hamiltonian, the gradient of the square of the ALP field acts as a ``pseudo-magnetic field'' $\bs{\mc{B}}_q$ given by
\begin{align}
    \bs{\mc{B}}_q \approx \mp\frac{2 \hbar^2 c^2}{g_F\mu_B f_q^2} \bs{\nabla} \varphi^2(\bs{r},t)~,
    \label{eq:pseudo-magnetic-field}
\end{align}
where $g_F$ is the Land\'e factor, $\mu_B$ is the Bohr magneton (or, for nuclear-spin-based magnetometers, the nuclear magneton). The projection of the near-dc component of $\bs{\mc{B}}_q$ along the sensitive axis of a magnetometer defined by the unit vector $\hat{\bs{m}}$ can be estimated in a manner similar to that discussed in, for example, Ref.\,\cite{gramolin2021spectral}, by evaluating the sum in Eq.\,\eqref{eq:gradient-field-sqr}, yielding characteristic magnitude (with an average value of zero) of %\DK{I think that we should include a factor of $1/\sqrt{3}$ below for the average over the random direction of the gradient. This is derived in Appendix~\ref{app:AngleDep}, see Eq.~\eqref{eq:angledep}. Then that cancels a factor of 2 that used to appear in the numerator. So I got rid of the 2. I don't think we need to explain it, do we?}
\begin{align}
    \hat{\bs{m}} \cdot \bs{\mc{B}}_q \sim \frac{\hbar^3 \rho\ts{dm} v_0}{g_F \mu_B m_\varphi f_q^2}~.
    \label{eq:ALP-intensity-gradient}
\end{align}
In the derivation of the above equation we assumed that the average spread of values of $\hat{\bs{m}}\cdot\bs{k}_{nm}$ is $\approx m_\varphi v_0/\hbar$. This estimate implicitly assumes that $\omega_{nm}$ and $\bs{k}_{nm}$ are uncorrelated, and thus the accuracy of this approximation varies with $\bs{v}\ts{lab}$ as discussed in Appendix~\ref{app:similarity}. Nonetheless, Eq.\,\eqref{eq:ALP-intensity-gradient} is suitable for a rough estimate of the sensitivity of a magnetometer network to such UBDM, given that $|\bs{v}\ts{lab}| \approx v_0$.

%\HMR{I think this paragraph does not add much information for our case}
%\HMRDel{In order to optimize the sensitivity of an experimental search for a correlated signal like that described by Eq.~\eqref{eq:ALP-intensity-gradient}, $1/f$ noise will have to be properly characterized, and data should be taken above the $1/f$ corner frequency and over many coherence times. We note that there are a variety of techniques that could be used to suppress $1/f$ noise (e.g.~comagnetometry, as shown in~Refs.\,\cite{Kor02,Kor05,Vas09,kimball2017constraints,hao2021herriott}).}


In order to estimate the sensitivity of a magnetometer network, for simplicity we assume $N_m$ identical sensors having the same directional sensitivity and dominated by Gaussian noise with the same variance (of course, this is not the typical case for real networks, these feature different directional sensitivities (see Appendix~\ref{app:AngleDep}), and are affected by $1/f$ noise).

In the cases of interest, the coherence length of the UBDM is much larger than the spacing between the sensors, so the UBDM signal will be identical in all sensors. 
To understand the scaling of the sensitivity with $N_m$, $\tau_\varphi$, and total acquisition time $T$, suppose that we divide the network into two distinct groups each with $N_m/2$ sensors and average the data in each group. 
%To search for a signal, the sensors can, for example, be divided into two groups of $N_m/2$ sensors and the data of each group can be averaged. 
Furthermore, suppose that the time-series data are binned in $\tau_\varphi$-long segments and time-averaged in each bin. 
Based on this approach, in the absence of a correlated UBDM signal, each group of sensors will exhibit a bin-to-bin variance in the measured magnetic field of approximately $\delta B / \sqrt{\tau_\varphi N_m/2} \sim \delta B / \sqrt{\tau_\varphi N_m}$, where $\delta B$ is the sensitivity of a single magnetometer in units of magnetic field strength times the square root of time.
%The numerator in $g^{(1)}(\tau)$ consists on the cross-correlation of the two averaged time-series over a measurement time $T$. While the denominator is a just a scaling factor.
For a total acquisition time $T$, there will be $N_b = T/\tau_\varphi$ bins. 
The expected residual from noise in the cross-correlation between the two groups provides an estimate of the network resolution, which in turn gives the minimum detectable pseudo-magnetic field squared 
%\NLF{ what happens to the sqrt(2)'s? are they contained in the "$\approx$" ?} 
%\DK{Yup. I put that explicitly up above where we state the smallest detectable signal so that the approximation is more obvious.}:
\begin{align}
    \abrk{ \mc{B}_q({\rm{min}})^2 }_t \approx \frac{\delta B^2}{N_m \tau_\varphi}\frac{1}{\sqrt{N_b}} \approx \frac{\delta B^2}{N_m \sqrt{\tau_\varphi T}}~.
    \label{eq:min-field}
\end{align}
An in-depth discussion of the $T$ and $N_m$ scaling for a similar case can be found in Ref.~\cite{derevianko2018detecting}.

Combining Eqs.~\eqref{eq:ALP-intensity-gradient} and \eqref{eq:min-field}, a bound on the UBDM coupling constant to which a magnetometer network would be sensitive is given by
\begin{align}
    f_q^2 \lesssim \frac{\hbar^3 \rho\ts{dm} v_0 }{g_F\mu_B m_\varphi \delta B} \prn{\tau_\varphi T}^{1/4} \sqrt{N_m}~.
    \label{eq:f_q-sens-mags}
\end{align}

%Further discussion of the sensitivity scaling with time and number of sensors is presented in Appendices~\ref{app:search} and\ref{app:SNscalingNate}.
%For a network consisting of $N_m$ magnetometers there are $N_m(N_m-1)/2 \sim N_m^2/2$ pairs to cross-correlate.  is sensitive to quadratic coupling constants
%where $v\ts{rel}$ is the relative velocity between the magnetometer and the rest frame of the UBDM field. %\draftNote{Derek: There are at least three different velocities like this throughout the text: the virial velocity $v\ts{vir}$, the velocity of dispersion $v_0$, and now this relative velocity $v\ts{rel}$. We should be careful that they're all needed and all properly used and defined. Maybe we are OK, but we should be careful. UPDATE: I eliminated $v\ts{vir}$ from the beginning of the paper. HMR: I think your $v\ts{rel}$ is the same as $v\ts{lab}$ with this it should be fine.}

Figure~\ref{Fig:sensitivity-GNOME} shows sensitivity estimates for the Global Network of Optical Magnetometers for Exotic physics searches (GNOME) based on alkali vapor magnetometers with $\delta B \approx 100~{\rm fT/\sqrt{Hz}}$ and the Advanced GNOME network based on noble gas comagnetometers with $\delta B \approx 1~{\rm fT/\sqrt{Hz}}$, assuming $T=100$~days and $N_m = 10$. Note that for $\tau_c \gg 24$\,hours, the signal amplitude is partially modulated at the frequency of Earth's rotation since the signals are $\propto \bs{\hat{m}}\cdot\bs{\mc{B}}_q$ and $\hat{\bs{m}}$ rotates with the Earth while $\bs{\mc{B}}_q$ does not, which can in principle enable the detection of UBDM with coherence times much longer than a day. Notable is the extent to which GNOME and Advanced GNOME can probe UBDM with Compton frequencies far beyond the nominal sensor bandwidths.

Optical atomic clocks are an example of a sensor that can search for scalar fields through the apparent variation of fundamental constants as described in Eqs.\,\eqref{eq:scalar-mass-variation} and \eqref{eq:scalar-alpha-variation}, due to, for example, the variation of the fine-structure constant $\alpha$ and relativistic effects (see Ref.\,\cite{safronova2018search} and references therein). For example, the fractional frequency variation in an atomic clock due to variation of the fine-structure constant $\alpha$ is given by
\begin{align}
    \frac{\delta \nu(t)}{\nu} = \kappa_\alpha \frac{\delta \alpha(t)}{\alpha}~,
    \label{eq:frac-freq-variation-alpha-1}
\end{align}
where $\nu$ is the clock frequency and $\kappa_\alpha$ is a sensitivity coefficient that depends on the type of clock: $\kappa_\alpha \approx 2$ for most current optical atomic clocks, but note that there are exceptions, such as the proposed clock with $\kappa_\alpha \approx -15$ described in Ref.~\cite{Safronova2018Apr}, and the possibility of future clocks based on highly charged ions \cite{kozlov2018highly} or a Th nuclear transition \cite{peik2021nuclear} that could have orders of magnitude larger values of $\kappa_\alpha$. 

%\DK{We can move most of the back-action discussion to the appendix. I think this trims about 150 words.}

It is important to note that the sensitivity of intensity interferometry can be significantly impacted by back-action of the surrounding matter density on the scalar field as pointed out in Refs.\,\cite{stadnik2020new,hees2018violation} and also discussed in Refs.\,\cite{Oli08,hinterbichler2010screening,jaffe2017testing}. The accessible range of parameter space for current optical clocks near the surface of the Earth is well within the regime where such back-action effects are significant (above the long-dashed blue line in Fig.\,\ref{Fig:sensitivity-clocks}, see Appendix~\ref{app:back-action}). However, for the range of boson masses and coupling constants considered in the present work, it turns out for a space-based network of sensors \cite{Schkolnik2022Apr} the screening effects can be largely neglected \cite{stadnik2020new}, and so for simplicity we consider such a space-based network in our sensitivity estimates.

%\DKDel{Before estimating the sensitivity of intensity interferometry to scalar dark matter fields, it is important to note that for the quadratic scalar interaction there can be non-negligible back-action of the surrounding matter density on the scalar field as pointed out in Refs.\,\cite{stadnik2020new,hees2018violation} and also discussed in Refs.\,\cite{Oli08,hinterbichler2010screening,jaffe2017testing}. 
%This back-action arises due to the fact that the bare potential for the scalar field, namely $m_\varphi^2 c^2 \varphi^2/(2 \hbar^2)$, is modified by the presence of the Lagrangian in Eq.\,\eqref{eq:scalar-Lagrangian}. 
%The quadratic terms in the interaction Lagrangian endow the scalar field with an effective mass $m\ts{eff}$ in the presence of matter; this effect is analogous to the screening of magnetic fields caused by the Meissner effect~(where the photon gains an effective mass inside a superconductor). 
%Depending on the sign of the interaction, back-action can lead to either screening or antiscreening \cite{hees2018violation}. 
%Since the accessible range of parameter space for current optical clocks near the surface of the Earth is well within the regime where such back-action effects are significant (above the long-dashed blue line in Fig.\,\ref{Fig:sensitivity-clocks}), such a sensor network would be predominantly sensitive to quadratic scalar interactions that are antiscreened and thus enhanced (see Appendix~\ref{app:back-action}). 
%Understanding details of how antiscreening affects the stochastic temporal characteristics of UBDM fields near the Earth's surface requires further analysis. 
%However, for the range of boson masses and coupling constants considered in the present work, it turns out for a space-based network of sensors \cite{Schkolnik2022Apr} the screening effects can be largely neglected \cite{stadnik2020new}, and so for simplicity we consider such a space-based network in our sensitivity estimates.}

Assuming the effect described by Eq.\,\eqref{eq:scalar-alpha-variation} and a scalar field that makes up the entirety of the dark matter density, the amplitude of the fractional frequency variation is given by
\begin{align}
    \frac{\delta \nu}{\nu} \approx \kappa_\alpha \frac{2 \hbar^3 \rho\ts{dm}}{\Lambda_\gamma^2 m_\varphi^2 c}~.
    \label{eq:frac-freq-variation-alpha-2}
\end{align}
Optical clock networks, with $N_c$ independent clocks, can achieve a fractional frequency uncertainty~\cite{collaboration2021frequency,lisdat2016clock}
\begin{align}
    \frac{\delta \nu}{\nu} \approx \frac{3 \times 10^{-16}}{(\tau_\varphi T)^{1/4}\sqrt{N_c}}~,
    \label{eq:frac-freq-variation-clock-sens}
\end{align}
which translates to the sensitivity to the quadratic scalar coupling constant shown in Fig.\,\ref{Fig:sensitivity-clocks}. Appendix~\ref{app:SensiticityDifference} offers an heuristic argument for the great nominal sensitivity difference between atomic clock and magnetometer networks to the coupling parameters $\Lambda_\gamma$ and $f_q$.

%\DK{I guess we can cut the following paragraph: the start of the paragraph can just be wholesale only discussed in the Supplemental Material, and the second sentence can be obviously inferred from the plots. This saves about 90 words.} 

%\DKDel{As seen by comparing Figs.\,\ref{Fig:sensitivity-GNOME} and \ref{Fig:sensitivity-clocks}, the nominal sensitivity of an optical clock network to the coupling parameter $\Lambda_\gamma$ far exceeds that of magnetometer networks to the equivalent coupling parameter $f_q$. An heuristic argument for this difference is given in Appendix~\ref{app:SensiticityDifference}. Note that for boson masses $m_\varphi c^2 \gtrsim 3 \times 10^{-11}~{\rm eV}$ (the region to the right of the dashed red line in both Figs.\,\ref{Fig:sensitivity-GNOME} and \ref{Fig:sensitivity-clocks}) the sensor network must be smaller than Earth-scale for the UBDM signals from all sensors to be spatially coherent.}

Ultimately, the sensitivity of sensor networks used to search for correlated signals from UBDM may be limited by systematic effects due to prosaic natural phenomena. 
Known natural phenomena that could generate noise with long-range correlations include, for example, time-dependent electromagnetic fields associated with cavity resonances of the conducting Earth-ionosphere cavity \cite{fedderke2021earth} (such as the Schumann resonances \cite{schumann1952strahlungslosen}) and vibrational noise due to free oscillations of the Earth excited by large earthquakes \cite{hu2020network} (such as the ``breathing'' mode of the Earth at $\approx 800~{\rm \mu Hz}$ \cite{dziewonski1981preliminary,rosat2007geographical}). 
In the event of a non-null result, auxiliary measurements with other instruments may be able to rule out such systematic effects. 
For example, GNOME uses unshielded magnetometers to monitor the magnetic environment near the shielded dark matter sensors to veto signals from anomalously large local magnetic field excursions \cite{afach2018characterization}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Conclusion}

\medskip

\noindent\emph{Conclusion.~---~}In summary, we propose a new method to search for UBDM by using intensity interferometry with sensor networks. We show that when the sensors measure signals quadratic in the UBDM field, there is a near-dc component of the signal that enables finite-bandwidth sensors to search for UBDM with Compton frequencies many orders of magnitude larger than possible if a traditional search for signals oscillating at the Compton frequency is carried out. Here we have focused on quadratic UBDM interactions and sensors with a linear response; however, the results are also valid for linear interactions and sensors that respond quadratically to the field (square-law detectors). The method of intensity interferometry is intrinsically broadband, with the potential to search for UBDM with particle masses ranging over many orders of magnitude without having to probe individual narrow frequency bands. UBDM searches with intensity interferometry using existing sensor networks can probe unexplored parameter space.

%The technique presented relays on all sensors located in the same coherence patch. For this reason the sensitivity region is upper-bounded at $\approx10^{-10}$\,eV. GNOME would face challenges sensing fluctuations with a coherence time shorter than half a day corresponding to masses greater than $10^{-13}$\,eV due to the directional propierties of the. Due to the non-directional coupling to the atomic clocks   }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\section*{Acknowledgements}
\vspace{12pt}
The authors are sincerely grateful to Jason Stalnaker, Ibrahim Sulai, Maxim Pospelov, Arran Phipps, Ben Buchler, Ron Folman, and Menachem Givon for enlightening discussions. The authors also thank Tatum Wilson, Rayshaun Preston, Christopher Verga, and Mario Duenas for early work on simulations. This work was supported by the U.S. National Science Foundation under grant PHYS-2110388, by the Cluster of Excellence ``Precision Physics, Fundamental Interactions, and Structure of Matter'' (PRISMA+ EXC 2118/1) funded by the German Research Foundation (DFG) within the German Excellence Strategy (Project ID 39083149), by the German Federal Ministry of Education and Research (BMBF) within the Quantumtechnologien program (Grant No. 13N15064), by the European Research Council (ERC) under the European Union Horizon 2020 research and innovation program (project Dark-OST, grant agreement No 695405), and by the DFG Project ID 423116110.
The authors at Boston University acknowledge support from the Simons Foundation Grant No. 641332, the National Science Foundation CAREER Award No. PHY-2145162, the John Templeton Foundation Grant No. 60049570, and the U.S. Department of Energy, Office of High Energy Physics program under the QuantISED program, FWP 100495. The work of YVS was supported by the Australian Research Council under the Discovery Early Career Researcher Award DE210101593. The work of SP was supported by the National Science Centre of Poland within the grant No. 2020/39/B/ST2/01524.



==> VersionControl/pre900maintext.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Introduce the dark matter problem
A wide variety of evidence suggests the existence of dark matter, an invisible substance that constitutes a large fraction of the matter in the Universe \cite{Fen10,spergel2015dark,graham2015experimental}. Despite decades of research, its microscopic nature remains unknown. A promising hypothesis is that dark matter predominantly consists of ultralight bosons, particles with masses $m_\varphi \ll 1~{\textrm{eV}}/c^2$, such as axions~\cite{Pre83,Abb83,Din83}, axion-like particles (ALPs)~\cite{Gra15,co2020predictions}, or hidden photons~\cite{holdom1986two,cvetivc1996implications,Okun1982}. Ultralight bosons can couple to Standard Model (SM) particles through a variety of ``portals'' \cite{graham2016dark,safronova2018search}, which have been used to search for ultralight bosonic dark matter (UBDM) --- see, for example, Refs.\,\cite{Asz01,Asz10,budker2014proposal,Sik14,chaudhuri2015radio,geraci2016sensitivity,abel2017search,wu2019search,garcon2019constraints,phipps2020exclusion,manley2020searching,crescini2020axion,braine2020extended,backes2021quantum,antypas2021probing,roussy2021experimental,Ayb21CASPErE,gramolin2021search}.

% Advantage of intensity measurement
Numerous experiments looking for UBDM are based on resonant systems, which require an accurate tuning to the unknown Compton frequency, $\omega_c = m_\varphi c^2 / \hbar$, in order to be sensitive to UBDM. Therefore, a time-consuming scan of tunable parameters must be performed to search a wide range of masses. However, if a search is based on the measurement of the \emph{intensity} of the UBDM, part of the signal is down-converted to near-zero frequency~\cite{stadnik2015can,hees2018violation}, regardless of the particular Compton frequency of the UBDM. Furthermore, assuming the standard halo model~\cite{Zyla:2020zbs,evans2019refinement,drukier1986detecting}, there are stochastic fluctuations of this near-dc component~\cite{Centers2019,derevianko2018detecting,foster2018,hui2021wave,schive2014cosmic,turner1990periodic,o2017axion,lisanti2021stochastic,gramolin2021spectral}. The linewidth of this spectral near-dc feature is comparable to the spectral linewidth of the UBDM field, $\approx \! \! 10^6$~times smaller than $\omega_c$. Looking for this near-dc feature allows sensors with a limited bandwidth to probe UBDM with masses $\approx \! \! 10^6$~times larger than searching for direct field oscillations at $\omega_c$.%(as in existing and planned experiments reviewed in, for example, Refs.\,\cite{safronova2018search,graham2015experimental,irastorza2018new}).%\footnote{Note that although Refs.\,\cite{derevianko2018detecting,foster2021dark} consider UBDM interferometry using sensor networks, they do not consider the intensity interferometry as we do here.}

%This method is limited by the fact that large Compton frequencies produce a broad dc feature, which eventually causes an attenuation of the signal due to the finite bandwidth of the detectors.

% quadratic Lagrangian for clocks
The frequency down-conversion discussed above occurs naturally when considering quadratic portals where the interaction with SM particles is proportional to the square of the UBDM field\,\cite{stadnik2015can,hees2018violation,Pos13,Der14,Oli08,Sta15,dailey2021quantum}. A spin-0 field $\varphi(\bs{r},t)$ can interact with SM fermions and electromagnetic fields according to the phenomenological quadratic scalar Lagrangian
\begin{align}
    \mc{L}_s = \hbar c \prn{\pm \frac{m_f c^2}{\Lambda_f^2} \bar{\psi}_f\psi_f \pm \frac{1}{4 \Lambda_\gamma^2} F_{\mu\nu}^2} \varphi^2(\bs{r},t)~,
    \label{eq:scalar-Lagrangian}
\end{align}
where $\Lambda_f$ and $\Lambda_\gamma$ parametrize the couplings to fermions and photons, respectively, where the $\pm$ indicates the sign of the coupling, $m_f$ is the fermion mass, $\psi_f$ is the fermion field, and $F_{\mu\nu}$ is the Faraday tensor.

% Effect of the interaction for clocks
The effects of the interactions described by Eq.\,\eqref{eq:scalar-Lagrangian} can be understood in terms of redefinitions of the effective fermion masses and the fine-structure constant $\alpha$\,\cite{stadnik2015can,Der14}:
\begin{align}
    m_f^{({\rm{eff}})} (\bs{r},t) & = m_f \prn{ 1 \mp \frac{\hbar c}{\Lambda_f^2} \varphi^2(\bs{r},t) }~, \label{eq:scalar-mass-variation} \\
    \alpha^{({\rm{eff}})} (\bs{r},t) & = \alpha \prn{ 1 \pm \frac{\hbar c}{\Lambda_\gamma^2} \varphi^2(\bs{r},t) }~. \label{eq:scalar-alpha-variation}
\end{align}
Variations of $m_f^{({\rm{eff}})}$ and $\alpha^{({\rm{eff}})}$ can be measured with atomic clocks or interferometers~\cite{Der14,wcislo2016experimental,roberts2017search,roberts2020search,dailey2021quantum,nagano2019axion,aiello2021constraints,badurina2020aion,Stadnik2016,Grote2019,Vermeulen2021,Sta15}, or generally by direct comparison of systems with different dependence on these fundamental constants~\cite{Antypas2019Oct,Antypas2020Apr,antypas2021probing,Oswald2021Nov,Tretiak2022Jan}.

% Quadratic interaction with magnetometers
Additionally, a UBDM field with pseudoscalar interactions (such as an axion or ALP field) can interact with SM fermions via the phenomenological interaction Lagrangian~\cite{dailey2021quantum}
\begin{align}
    \mc{L}_\varphi = \pm\frac{1}{f_q^2} \underbrace{\bar{\psi}_f \gamma^\mu\gamma_\ts{5} \psi_f}_{{\substack{\text{fermion axial} \\ \text{vector current}}}} \partial_\mu \varphi^2(\bs{r},t)~,
    \label{eq:pseudoscalar-Lagrangian}
\end{align}
where $f_q$ parameterizes the coupling to fermion spins,  $\gamma^\mu$ and $\gamma_\ts{5}$ are the Dirac matrices. %(note that $\bar{\psi}_f \gamma^\mu\gamma_\ts{5} \psi_f$ is the fermion axial vector current).
In the nonrelativistic limit, Eq.\,\eqref{eq:pseudoscalar-Lagrangian} yields the interaction Hamiltonian
\begin{align}
    \mc{H}_\varphi = \mp\frac{2\hbar^2c^2}{f_q^2} \bs{S} \cdot \bs{\nabla} \varphi^2(\bs{r},t)~,
    \label{eq:quadratic-Hamiltonian}
\end{align}
which shows that the gradient of the square of the pseudoscalar field couples to a fermion spin $\bs{S}$ similarly to a magnetic field. Here $\bs{\nabla} \varphi^2(\bs{r},t)$ plays the role of a pseudo-magnetic field. Thus, such pseudoscalar fields can be searched for in the spin dynamics of electrons or nuclei. While a variety of sensors could be used, here we focus on atomic (nuclear) magnetometers since these are intrinsically sensitive to Zeeman shifts~\cite{Pos13,Pus13,afach2018characterization,kimball2018searching,masia-roig_analysis_2020,afach2021search,Jiang2021Dec}.

% Networks to detect the stochastic fluctuations
The effects described by Eqs.\,\eqref{eq:scalar-mass-variation},~\eqref{eq:scalar-alpha-variation},~and~\eqref{eq:quadratic-Hamiltonian} are proportional to the UBDM intensity and exhibit \mbox{near-dc} stochastic amplitude fluctuations. Although measuring low-frequency signals is technically challenging due to multiple sources of low-frequency noise, an array of independent, geographically distributed sensors will tend to have uncorrelated noise. In contrast, the slowly-changing UBDM intensity will lead to a common-mode fluctuating signal present in all detectors within a coherence length of one another, which will appear in correlations between the sensors. We advocate for the use of networks of sensors to search for these stochastic fluctuations. There are existing and proposed dark matter searches sensitive to these interactions using networks consisting of a variety of sensor types such as atomic clocks~\cite{Der14,wcislo2016experimental,roberts2017search,roberts2020search,dailey2021quantum,collaboration2021frequency}, atomic magnetometers~\cite{Pos13,Pus13,afach2018characterization,kimball2018searching,masia-roig_analysis_2020,afach2021search,fedderke2021earth,fedderke2021search,arza2021earth}, gravimeters~\cite{hu2020network,mcnally2020constraining,horowitz2020gravimeter}, laser interferometers~\cite{hall2018laser,nagano2019axion,aiello2021constraints,Stadnik2016,Grote2019,Vermeulen2021,Sta15}, and atom interferometers \cite{badurina2020aion}. The methodology described below is analogous to Hanbury Brown and Twiss intensity interferometry\,\cite{brown1956question}, and can be used to dramatically expand the range of UBDM Compton frequencies that particular sensors can probe~\cite{InterferometryNote}\nocite{derevianko2018detecting,foster2021dark}.

% Suggest the use of moving trucks
%If there are UBDM-related cross-correlations discovered, further analysis can narrow the range of possible boson masses. (For example, by measuring the coherence time and length, for which portable sensors could be employed as in Refs.\,\cite{grotti2018geodesy,takamoto2020test}.)


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section*{Stochastic properties of the ultralight bosonic dark matter field}
\label{sec:field-properties}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Introduce our treatment of the UBDM field

\medskip

\noindent \emph{Stochastic properties of the UBDM field.~---~}The properties of the UBDM field can be derived using the framework described in Refs.\,\cite{Centers2019,derevianko2018detecting,foster2018,hui2021wave,schive2014cosmic,turner1990periodic,o2017axion,lisanti2021stochastic,gramolin2021spectral}. In brief, assuming that UBDM does not interact with itself, each individual particle can be treated as an independent wave. In this scenario, the UBDM field is well described by a superposition of these individual waves.

% Field produced by one boson
If the local dark-matter energy density $\rho\ts{dm}$ results from $N$ ultralight bosons of mass $m_\varphi$, the field contribution of an individual boson $n$ is
\begin{align}
    \varphi_n(\bs{r},t) \approx \frac{\varphi_0}{\sqrt{N}} \cos\prn{ \omega_n t - \bs{k}_n \cdot \bs{r} + \theta_n }~,
    \label{eq:single-boson-field}
\end{align}
where the boson field amplitude is given by~\cite{Gra13}
\begin{align}
    \varphi_0 = \frac{\hbar}{m_\varphi c} \sqrt{ 2 \rho\ts{dm} },
    \label{eq:single-ALP-field-amp}
\end{align}
such that the average energy density in the UBDM field comprises the totality of the local dark matter. Here, $\bs{k}_n = m_\varphi \bs{v}_n /  \hbar$ is the wave vector corresponding to $\bs{v}_n$, the velocity of the $n^\text{th}$ boson in the laboratory frame, while $\theta_n$ is a phase associated with each boson, that is distributed between $0$ and $2\pi$. The oscillation frequency of the individual UBDM particles, $\omega_{n}$, is determined mostly by their Compton frequency, $\omega_{c}$. However, the second-order Doppler effect introduces small deviations from $\omega_{c}$, so that
\begin{align}
    \omega_n = \omega_c \prn{ 1 + \frac{\bs{v}_n^2}{2c^2} }.
\end{align}
Therefore, the distribution of $\omega_n$ (and $\bs{k}_n$) is determined by the velocity distribution of the particles as observed in the laboratory frame, which, according to the standard halo model, follows a displaced Maxwell-Boltzmann distribution given by
\begin{equation}
f_{\text{lab}}(\bs{v}) \approx \frac{1}{\pi^{3/2} v_0^3} \exp{\left(-\frac{(\bs{v-\bs{v}_{\text{lab}}})^2}{v_0^2}\right)}, \label{eq:f_lab_velocity}
\end{equation}
where the velocity of the lab frame is~$\bs{v}_{\text{lab}} = |\bs{v}_{\text{lab}}| \bs{\hat{z}}$, and we have ignored the escape velocity cut-off. In our simulations, we take the isotropic velocity dispersion of the local UBDM to be determined by the characteristic virial velocity $v_0\approx 220~\text{km}/\text{s}$, and $\bs{v}_{\text{lab}}$ to be dominated by the motion of the Sun in the galactic frame, $|\bs{v}_{\text{lab}}| \approx 233~\text{km}/\text{s}$.

% Total UBDM field (removed as suggested by Dima and Sasha G. in order to space space. Replaced by a sentence in next paragraph)
%The total UBDM field is given by the superposition %of the $N$ individual bosons,
%\begin{align}
%    \varphi(\bs{r},t) = \frac{a_0}{\sqrt{N}} \sum_{n=1}^N  \cos\prn{ \omega_n t - \bs{k}_n \cdot \bs{r} +\phi_n }.
%    \label{eq:ALPsum}
%\end{align}


% Motivate the interest on |\varphi|^2 and \bs{\nabla} |\varphi|^2
The total UBDM field $\varphi(\bs{r},t)$ is given by the superposition of the wavefunctions of $N$ individual bosons as described by Eq.\,\eqref{eq:single-boson-field}. Here, our interest lies in quadratic interactions with the field, proportional to $\varphi^2(\bs{r},t)$ or $\bs{\nabla} \varphi^2(\bs{r},t)$. These quantities have two terms: one near-dc component and one fast oscillating component at $\approx 2\omega_c$. We consider sensors with a limited bandwidth $\Delta \omega \ll \omega_c$, such that the fast oscillating terms can be ignored. Using this approximation the near-dc component (denoted by the subscript~$s$) of $\varphi^2$ and $\bs{\nabla} \varphi^2$ can be written as
\begin{align}
    \varphi_s^2(\bs{r},t) &= \frac{\varphi_0^2}{2N} \sum_{n,m=1}^N \cos \prn{\omega_{nm} t -\bs{k}_{nm} \cdot \bs{r}  +\theta_{nm}},\label{eq:field-squared}\\
    \bs{\nabla} \varphi_s^2(\bs{r},t) &=  \frac{\varphi_0^2}{2N} \sum_{n,m=1}^N   \bs{k}_{nm} \sin \prn{\omega_{nm} t -\bs{k}_{nm} \cdot \bs{r} +\theta_{nm}}, \label{eq:gradient-field-sqr} 
\end{align}
where $\omega_{nm}= \omega_{n} - \omega_{m}$, $\bs{k}_{nm} = \bs{k}_{n} - \bs{k}_{m}$, and $\theta_{nm}=\theta_{n} - \theta_{m}$. 
Since the sensors are assumed to be within the same coherence patch (such that $\Delta\bs{k} \cdot \Delta\bs{r} \approx 0$, where $\Delta \bs{k}$ is the characteristic spread of values in $\bs{k}_{nm}$ and $\Delta \bs{r}$ is the difference of the position vectors for both sensors), the $\bs{r}$ dependence can be neglected and we can evaluate the expressions at $\bs{r}=0$ in the following calculations~\cite{TruckNote}\nocite{grotti2018geodesy,takamoto2020test}.%\footnote{Note that the spatial dependence for coherence lengths smaller than the Earth's diameter could also be exploited to look for UBDM, for which portable sensors could be employed as in Refs.\,\cite{grotti2018geodesy,takamoto2020test}.}

% Introduce the degree of first-order coherence and coherence time

The signal measured with each sensor would have a small UBDM-related component $\kappa\, \xi(t)$, where $\kappa$ accounts for the coupling of the sensor to the UBDM field, and $\xi(t)$ is either $\varphi^2_s$ (scalar interaction) or $\hat{\bs{m}} \cdot \bs{\nabla} \varphi^2_s$ (pseudoscalar gradient interaction, where $\hat{\bs{m}}$ represents the sensitive direction of the sensor). The correlations between measurable signals produced in different sensors by a UBDM field can be quantified using the degree of first-order coherence $g^{(1)}(\tau)$ for different delay times $\tau$,
\begin{equation}
    g^{(1)}(\tau) = \frac{\langle \xi(t) \xi(t+\tau) \rangle_t}{\langle \xi^2 \rangle_t}~,
    \label{eq:first-order-coherence-definition}
\end{equation}
 where $\abrk{\cdots}_t$ denotes the time average. The value of $g^{(1)}(\tau)$ is a measure of the degree of correlation between $\xi(t)$ and $\xi(t+\tau)$. Additionally, we will define the coherence time as the power-equivalent width of $g^{(1)}(\tau)$~\cite{loudon2000the,saleh2019fundamentals},

\begin{equation}
    \tau_c = \int_{-\infty}^{+\infty} |g^{(1)}(\tau)|^2 d\tau,
    \label{eq:coherence_time_def}
\end{equation}
which gives a characteristic time scale for the decay of $g^{(1)}(\tau)$. The full width at half maximum of the~$\varphi$ lineshape is $\approx \omega_c v_0^2/c^2$, giving a useful estimation of the coherence time of the field~(the result is exact for a Lorentzian lineshape~\cite{gramolin2021spectral}),

\begin{equation}
    \tau_\varphi \approx \frac{2 \hbar}{ m_\varphi v_0^2},
    \label{eq:coherence_time}
\end{equation}
which will be used as a benchmark timescale throughout the text. Note that there is an ambiguity, up to a factor of $2\pi$, in the definitions of $\tau_c$ used in the literature~\cite{Centers2019}. Because the actual lineshape describing $\varphi$ is expected to be non-Lorentzian \cite{gramolin2021spectral}, $\tau_\varphi$ slightly differs from the coherence time of the field $\varphi$ derived from the simulations. For the considered $\bs{v}_\ts{lab}$, simulations show a coherence time $\approx 1.12(1) \tau_\varphi$.

To illustrate the stochastic properties of $\bs{\nabla} \varphi^2(0,t)$ and $\varphi^2(0,t)$, their time evolution was simulated (details in Appendix~\ref{app:calculation}). Plots of $g^{(1)}(\tau)$ for $\varphi^2(t)$ and for projections of $\bs{\nabla} \varphi^2(t)$ onto parallel and perpendicular directions with respect to $\bs{v}\ts{lab}$ can be seen in Fig.\,\ref{fig:g1}. Note that these quantities experience stochastic fluctuations occurring at similar time scales.
\begin{figure}[ht]
\center
\includegraphics[width=\columnwidth,trim={0 5mm 0 3mm},clip]{Coherence.pdf}
\caption{\small{ Degree of first-order coherence as a function of delay time $\tau$ for $\varphi_s^2$ and different projections of the gradient $\bs{\nabla} \varphi_s^2$ relative to $\bs{v}_\ts{lab}$. Each curve is the result of 100~averages simulating $10^3$ particles, where the mean was subtracted (details in Appendix~\ref{app:calculation}). The approximate values of the coherence times are given in colors matching their respective plot traces.}}
\label{fig:g1}
\end{figure}

% Coherence time of $\varphi^2_s(0,t)$ and gradient
The coherence time for $\varphi^2_s$ is approximately half of that for the field $\varphi$. This is a result of the field $\varphi^2_s$ being a sum over terms depending on the difference of frequencies $\omega_{nm}$, as opposed to $\varphi$, which only contains terms depending on $\omega_n$. The probability distribution of $\omega_{nm}$ can be calculated as the convolution of the distribution of $\omega_n$ with itself. This results in a distribution for $\omega_{nm}$ that is broader. Consequently, the coherence time is shorter since $g^{(1)}(\tau)$ is given by the Fourier transform of the power spectral density of $\varphi^2_s$ (proportional to the $\omega_{nm}$ distribution), according to the Wiener–Khinchin theorem. The gradient coupling features even shorter coherence times due to the $\bs{k}_{nm}$ factor weighting the contribution of the oscillating terms. Larger $\omega_{nm}$ tends to correspond to larger $\bs{k}_{nm}$: this effectively broadens the power spectral density of $\bs{\nabla} \varphi^2_s$, leading to a shorter coherence time. This is also the reason why parallel and perpendicular components of the gradient have different coherence times~(see~Appendix~\ref{app:similarity}).

A formal derivation of $g^{(1)}(\tau)$ for $\varphi^2_s$ and $\bs{\nabla} \varphi^2_s$ in the simplified case where $|\bs{v}_{\text{lab}|} \gg v_0$ can be found in Appendix~\ref{app:analytic}.

% Relate coherence time of the fields to mass
The coherence time is also related to the mass of the UBDM particle as can be seen in Eq.\,\eqref{eq:coherence_time}. The relationship between the UBDM mass and the coherence time exhibited by $\varphi^2_s$ and $\bs{\nabla} \varphi^2_s$ is shown in Fig.\,\ref{Fig:massdep}. The coherence times for $\varphi^2_s$ and $\bs{\nabla} \varphi^2_s$ are proportional to the coherence time of $\varphi$, $\tau_\varphi$ as defined in Eq.\,\eqref{eq:coherence_time}. In the case of detection, this could be used to estimate the mass of the UBDM particles. Further discussion on the scaling of the coherence times can be found in Appendix~\ref{app:similarity}.
\begin{figure}[ht]
\center
\includegraphics[width=\columnwidth,trim={0 5mm 0 3mm},clip]{MassVStc.pdf}
\caption{\small{Mass dependence of the characteristic delay time at which $g^{(1)}(\tau)=0.5$ for $\varphi_s^2$ and projections of $\bs{\nabla} \varphi_s^2$. Each point is the result of 100~averages simulating $10^3$ particles (details in Appendix~\ref{app:calculation}).}}
\label{Fig:massdep}
\end{figure}


%Propose the search method
A possible method to look for UBDM by exploiting these stochastic properties is to use intensity interferometry with multiple sensors to measure the cross-correlation between the time-series data from different sensors.
When using pairs of independent and geographically distributed sensors, a correlated global background field will produce a nonzero cross-correlation $g^{(1)}_{AB}(\tau)$ between sensors $A$ and $B$ proportional to $g^{(1)}(\tau)$, as discussed in Appendix~\ref{app:search}. Note that uncorrelated noise in the sensors will reduce the expected value of $g^{(1)}_{AB}(0)$ in the presence of a UBDM signal, making it smaller than the maximum value of one (see Appendix~\ref{app:search}). 
Additionally, in the case of the gradient coupling, a relative misalignment of the sensors' sensitive axes also leads to a reduction in the value of $g^{(1)}_{AB}(0)$ (see Appendix~\ref{app:AngleDep}). 
In order to distinguish a signal from noise,  $g^{(1)}_{AB}(0)$ can be compared with $g^{(1)}_{AB}(\tau \gg \tau_\varphi)$. 
Additionally, the uncertainty in the measurement can be reduced by averaging over many coherence times. Therefore this approach to analysis requires measurement times $T \gg \tau_\varphi$, in practice setting a lower limit on the accessible mass range. 
However, for low frequencies, the UBDM signal can be directly detected without the need of the frequency down-conversion used here. 
Furthermore, for a network of many sensors, pairwise measurements can be used to check for consistency.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\section{Accessible ultralight bosonic dark matter parameter space}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%In this section, we show that existing networks of clocks and magnetometers have sufficient sensitivity to probe unexplored parameter space describing UBDM by searching for correlated stochastic fluctuations as described above.

\medskip

\noindent \emph{Accessible UBDM parameter space.~---~}Existing sensor networks have sufficient sensitivity to probe experimentally unexplored parameter space describing UBDM by searching for correlated stochastic fluctuations using intensity interferometry.

%----------------------------------------------------------------
\begin{figure}[t]
\center
\includegraphics[width=\columnwidth]{IntensityInterferometrySensGNOME.pdf}
\caption{\small{Estimated parameter space describing ALP dark matter that can be probed by GNOME (dashed line, purple shaded region) and Advanced GNOME (dotted line, light blue shaded region) in $\approx 100$~days of searching for correlated stochastic fluctuations using $N_m = 10$ magnetometers. GNOME and Advanced GNOME are sensitive to the interaction of the ALP field with proton spins described by Eq.\,\eqref{eq:quadratic-Hamiltonian}; $f_q$ parameterizes the ALP-fermion coupling strength. The vertical dashed red line marks the Compton frequency and mass for which the ALP coherence length equals the Earth's diameter, $\lambda\ts{coh} \approx 2R_E$, corresponding to a characteristic coherence time scale for fluctuations of $\bs{\nabla} \varphi^2_s$ of $\tau_c \approx 30~{\rm s}$. The vertical dashed blue line marks the Compton frequency and mass for which $\tau_c \approx 24~{\rm hours}$; for $m_\varphi$ much smaller than this value, the pseudo-magnetic field is quasi-static in the galactic rest frame and thus the signals are frequency upconverted in the sensor network due to Earth's rotation. The dark red shaded region shows constraints from the Noble and Alkali Spin Detectors for Ultra-light Coherent darK matter (NASDUCK) experiment \cite{bloch2022new}. Note that there are also experimental constraints for lower $m_\varphi$ and $f_q$ from the Cosmic Axion Spin Precession Experiment (CASPEr) \cite{wu2019search,garcon2019constraints} as well as constraints competitive with the projected GNOME sensitivity obtained from reinterpretation \cite{bloch2020axion} of comagnetometer data used for other tests of fundamental physics \cite{kornack2005test,vasilakis2011precision,Bro10}. The dark green shaded area represents astrophysical bounds on spin-dependent ALP interactions with nucleons \cite{Oli08,chang2018supernova}. Note, however, that there are theoretical scenarios where these astrophysical bounds can be circumvented \cite{derocco2020exploring}, and thus laboratory searches are complementary to astrophysical observations. }}
\label{Fig:sensitivity-GNOME}
\end{figure}
%----------------------------------------------------------------

%----------------------------------------------------------------
\begin{figure}[t]
\center
\includegraphics[width=\columnwidth]{StochasticFluctuationsSensClock.pdf}
\caption{\small{Estimated parameter space describing UBDM fields that can be probed by an optical clock network such as those described in Refs.\,\cite{collaboration2021frequency,lisdat2016clock} (dotted line, light purple shaded region) in $\approx 100$~days of searching for correlated stochastic fluctuations using $N_c = 10$ clocks, not accounting for (anti)screening from back-action \cite{hees2018violation,stadnik2020new}, which can play a significant role near Earth's surface above the long-dashed blue line as indicated by the blue arrow. Clocks are sensitive to the interactions described by Eq.\,\eqref{eq:scalar-Lagrangian}; $\Lambda_\gamma$ parameterizes the strength of the coupling of the ultralight bosons to photons. The vertical dashed red line marks the Compton frequency and mass for which the ultralight boson's coherence length equals the Earth's diameter. The dark green shaded area represents astrophysical bounds on such quadratic scalar interactions between ultralight bosons and photons from stellar cooling and observations of supernova 1987a \cite{Oli08,chang2018supernova}; the light green shaded region represents bounds from Big Bang nucleosynthesis (BBN) \cite{stadnik2015can}. Note that there may be nonstandard scenarios where the astrophysical and cosmological bounds could be circumvented \cite{derocco2020exploring,bernal2021alp}, so laboratory experiments are useful complementary probes.}}
\label{Fig:sensitivity-clocks}
\end{figure}
%----------------------------------------------------------------

Atomic magnetometers can search for ALP fields by detecting Zeeman shifts caused by the interaction described in Eq.\,\eqref{eq:quadratic-Hamiltonian}. In analogy with the Zeeman Hamiltonian, the gradient of the square of the ALP field acts as a ``pseudo-magnetic field'' $\bs{\mc{B}}_q$ given by
\begin{align}
    \bs{\mc{B}}_q \approx \mp\frac{2 \hbar^2 c^2}{g_F\mu_B f_q^2} \bs{\nabla} \varphi^2(\bs{r},t)~,
    \label{eq:pseudo-magnetic-field}
\end{align}
where $g_F$ is the Land\'e factor, $\mu_B$ is the Bohr magneton (or, for nuclear-spin-based magnetometers, the nuclear magneton). The projection of the near-dc component of $\bs{\mc{B}}_q$ along the sensitive axis of a magnetometer defined by the unit vector $\hat{\bs{m}}$ can be estimated in a manner similar to that discussed in, for example, Ref.\,\cite{gramolin2021spectral}, by evaluating the sum in Eq.\,\eqref{eq:gradient-field-sqr}, yielding characteristic magnitude (with an average value of zero) of %\DK{I think that we should include a factor of $1/\sqrt{3}$ below for the average over the random direction of the gradient. This is derived in Appendix~\ref{app:AngleDep}, see Eq.~\eqref{eq:angledep}. Then that cancels a factor of 2 that used to appear in the numerator. So I got rid of the 2. I don't think we need to explain it, do we?}
\begin{align}
    \hat{\bs{m}} \cdot \bs{\mc{B}}_q \sim \frac{\hbar^3 \rho\ts{dm} v_0}{g_F \mu_B m_\varphi f_q^2}~.
    \label{eq:ALP-intensity-gradient}
\end{align}
In the derivation of the above equation we assumed that the average spread of values of $\hat{\bs{m}}\cdot\bs{k}_{nm}$ is $\approx m_\varphi v_0/\hbar$. This estimate implicitly assumes that $\omega_{nm}$ and $\bs{k}_{nm}$ are uncorrelated, and thus the accuracy of this approximation varies with $\bs{v}\ts{lab}$ as discussed in Appendix~\ref{app:similarity}. Nonetheless, Eq.\,\eqref{eq:ALP-intensity-gradient} is suitable for a rough estimate of the sensitivity of a magnetometer network to such UBDM, given that $|\bs{v}\ts{lab}| \approx v_0$.

In order to optimize the sensitivity of an experimental search for a correlated signal like that described by Eq.~\eqref{eq:ALP-intensity-gradient}, $1/f$ noise will have to be properly characterized, and data should be taken above the $1/f$ corner frequency and over many coherence times. 
We note that there are a variety of techniques that could be used to suppress $1/f$ noise (e.g.~comagnetometry, as shown in~Refs.\,\cite{Kor02,Kor05,Vas09,kimball2017constraints,hao2021herriott}).

In order to estimate the sensitivity of a magnetometer network, for simplicity we assume $N_m$ identical sensors having the same directional sensitivity and dominated by Gaussian noise with the same variance (of course, this is not the typical case for real networks, in particular see the discussion of directional sensitivity in Appendix~\ref{app:AngleDep}). 
In the cases of interest, the coherence length of the UBDM is much larger than the spacing between the sensors, so the UBDM signal will be identical in all sensors. 
To understand the scaling of the sensitivity with $N_m$, $\tau_\varphi$, and total acquisition time $T$, suppose that we divide the network into two distinct groups each with $N_m/2$ sensors and average the data in each group. 
%To search for a signal, the sensors can, for example, be divided into two groups of $N_m/2$ sensors and the data of each group can be averaged. 
Furthermore, suppose that the time-series data are binned in $\tau_\varphi$-long segments and time-averaged in each bin. 
Based on this approach, in the absence of a correlated UBDM signal, each group of sensors will exhibit a bin-to-bin variance in the measured magnetic field of approximately $\delta B / \sqrt{\tau_\varphi N_m/2} \sim \delta B / \sqrt{\tau_\varphi N_m}$, where $\delta B$ is the sensitivity of a single magnetometer in units of magnetic field strength times the square root of time.
%The numerator in $g^{(1)}(\tau)$ consists on the cross-correlation of the two averaged time-series over a measurement time $T$. While the denominator is a just a scaling factor.
For a total acquisition time $T$, there will be $N_b = T/\tau_\varphi$ bins. 
The expected residual from noise in the cross-correlation between the two groups provides an estimate of the network resolution, which in turn gives the minimum detectable pseudo-magnetic field squared 
%\NLF{ what happens to the sqrt(2)'s? are they contained in the "$\approx$" ?} 
%\DK{Yup. I put that explicitly up above where we state the smallest detectable signal so that the approximation is more obvious.}:
\begin{align}
    \abrk{ \mc{B}_q({\rm{min}})^2 }_t \approx \frac{\delta B^2}{N_m \tau_\varphi}\frac{1}{\sqrt{N_b}} \approx \frac{\delta B^2}{N_m \sqrt{\tau_\varphi T}}~.
    \label{eq:min-field}
\end{align}
An in-depth discussion of the $T$ and $N_m$ scaling for a similar case can be found in Ref.~\cite{derevianko2018detecting}.

Combining Eqs.~\eqref{eq:ALP-intensity-gradient} and \eqref{eq:min-field}, a bound on the UBDM coupling constant to which a magnetometer network would be sensitive is given by
\begin{align}
    f_q^2 \lesssim \frac{\hbar^3 \rho\ts{dm} v_0 }{g_F\mu_B m_\varphi \delta B} \prn{\tau_\varphi T}^{1/4} \sqrt{N_m}~.
    \label{eq:f_q-sens-mags}
\end{align}

%Further discussion of the sensitivity scaling with time and number of sensors is presented in Appendices~\ref{app:search} and\ref{app:SNscalingNate}.
%For a network consisting of $N_m$ magnetometers there are $N_m(N_m-1)/2 \sim N_m^2/2$ pairs to cross-correlate.  is sensitive to quadratic coupling constants
%where $v\ts{rel}$ is the relative velocity between the magnetometer and the rest frame of the UBDM field. %\draftNote{Derek: There are at least three different velocities like this throughout the text: the virial velocity $v\ts{vir}$, the velocity of dispersion $v_0$, and now this relative velocity $v\ts{rel}$. We should be careful that they're all needed and all properly used and defined. Maybe we are OK, but we should be careful. UPDATE: I eliminated $v\ts{vir}$ from the beginning of the paper. HMR: I think your $v\ts{rel}$ is the same as $v\ts{lab}$ with this it should be fine.}

Figure~\ref{Fig:sensitivity-GNOME} shows sensitivity estimates for the Global Network of Optical Magnetometers for Exotic physics searches (GNOME) based on alkali vapor magnetometers with $\delta B \approx 100~{\rm fT/\sqrt{Hz}}$ and the Advanced GNOME network based on noble gas comagnetometers with $\delta B \approx 1~{\rm fT/\sqrt{Hz}}$, assuming $T=100$~days and $N_m = 10$. Note that for $\tau_c \gg 24$\,hours, the signal amplitude is partially modulated at the frequency of Earth's rotation since the signals are $\propto \bs{\hat{m}}\cdot\bs{\mc{B}}_q$ and $\hat{\bs{m}}$ rotates with the Earth while $\bs{\mc{B}}_q$ does not, which can in principle enable the detection of UBDM with coherence times much longer than a day. Notable is the extent to which GNOME and Advanced GNOME can probe UBDM with Compton frequencies far beyond the nominal sensor bandwidths.

Optical atomic clocks are an example of a sensor that can search for scalar fields through the apparent variation of fundamental constants as described in Eqs.\,\eqref{eq:scalar-mass-variation} and \eqref{eq:scalar-alpha-variation}, due to, for example, the variation of the fine-structure constant $\alpha$ and relativistic effects (see Ref.\,\cite{safronova2018search} and references therein). For example, the fractional frequency variation in an atomic clock due to variation of the fine-structure constant $\alpha$ is given by
\begin{align}
    \frac{\delta \nu(t)}{\nu} = \kappa_\alpha \frac{\delta \alpha(t)}{\alpha}~,
    \label{eq:frac-freq-variation-alpha-1}
\end{align}
where $\nu$ is the clock frequency and $\kappa_\alpha$ is a sensitivity coefficient that depends on the type of clock: $\kappa_\alpha \approx 2$ for most current optical atomic clocks, but note that there are exceptions, such as the proposed clock with $\kappa_\alpha \approx -15$ described in Ref.~\cite{Safronova2018Apr}, and the possibility of future clocks based on highly charged ions \cite{kozlov2018highly} or a Th nuclear transition \cite{peik2021nuclear} that could have orders of magnitude larger values of $\kappa_\alpha$. 

Before estimating the sensitivity of intensity interferometry to scalar dark matter fields, it is important to note that for the quadratic scalar interaction there can be non-negligible back-action of the surrounding matter density on the scalar field as pointed out in Refs.\,\cite{stadnik2020new,hees2018violation} and also discussed in Refs.\,\cite{Oli08,hinterbichler2010screening,jaffe2017testing}. 
This back-action arises due to the fact that the bare potential for the scalar field, namely $m_\varphi^2 c^2 \varphi^2/(2 \hbar^2)$, is modified by the presence of the Lagrangian in Eq.\,\eqref{eq:scalar-Lagrangian}. 
The quadratic terms in the interaction Lagrangian endow the scalar field with an effective mass $m\ts{eff}$ in the presence of matter; this effect is analogous to the screening of magnetic fields caused by the Meissner effect~(where the photon gains an effective mass inside a superconductor). 
Depending on the sign of the interaction, back-action can lead to either screening or antiscreening \cite{hees2018violation}. 
Since the accessible range of parameter space for current optical clocks near the surface of the Earth is well within the regime where such back-action effects are significant (above the long-dashed blue line in Fig.\,\ref{Fig:sensitivity-clocks}), such a sensor network would be predominantly sensitive to quadratic scalar interactions that are antiscreened and thus enhanced (see Appendix~\ref{app:back-action}). 
Understanding details of how antiscreening affects the stochastic temporal characteristics of UBDM fields near the Earth's surface requires further analysis. 
However, for the range of boson masses and coupling constants considered in the present work, it turns out for a space-based network of sensors \cite{Schkolnik2022Apr} the screening effects can be largely neglected \cite{stadnik2020new}, and so for simplicity we consider such a space-based network in our sensitivity estimates.

Assuming the effect described by Eq.\,\eqref{eq:scalar-alpha-variation} and a scalar field that makes up the entirety of the dark matter density, the amplitude of the fractional frequency variation is given by
\begin{align}
    \frac{\delta \nu}{\nu} \approx \kappa_\alpha \frac{2 \hbar^3 \rho\ts{dm}}{\Lambda_\gamma^2 m_\varphi^2 c}~.
    \label{eq:frac-freq-variation-alpha-2}
\end{align}
Optical clock networks, with $N_c$ independent clocks, can achieve a fractional frequency uncertainty~\cite{collaboration2021frequency,lisdat2016clock}
\begin{align}
    \frac{\delta \nu}{\nu} \approx \frac{3 \times 10^{-16}}{(\tau_\varphi T)^{1/4}\sqrt{N_c}}~,
    \label{eq:frac-freq-variation-clock-sens}
\end{align}
which translates to the sensitivity to the quadratic scalar coupling constant shown in Fig.\,\ref{Fig:sensitivity-clocks}.

As seen by comparing Figs.\,\ref{Fig:sensitivity-GNOME} and \ref{Fig:sensitivity-clocks}, the nominal sensitivity of an optical clock network to the coupling parameter $\Lambda_\gamma$ far exceeds that of magnetometer networks to the equivalent coupling parameter $f_q$. An heuristic argument for this difference is given in Appendix~\ref{app:SensiticityDifference}. Note that for boson masses $m_\varphi c^2 \gtrsim 3 \times 10^{-11}~{\rm eV}$ (the region to the right of the dashed red line in both Figs.\,\ref{Fig:sensitivity-GNOME} and \ref{Fig:sensitivity-clocks}) the sensor network must be smaller than Earth-scale for the UBDM signals from all sensors to be spatially coherent.

Ultimately, the sensitivity of sensor networks used to search for correlated signals from UBDM may be limited by systematic effects due to prosaic natural phenomena. 
Known natural phenomena that could generate noise with long-range correlations include, for example, time-dependent electromagnetic fields associated with cavity resonances of the conducting Earth-ionosphere cavity \cite{fedderke2021earth} (such as the Schumann resonances \cite{schumann1952strahlungslosen}) and vibrational noise due to free oscillations of the Earth excited by large earthquakes \cite{hu2020network} (such as the ``breathing'' mode of the Earth at $\approx 800~{\rm \mu Hz}$ \cite{dziewonski1981preliminary,rosat2007geographical}). 
In the event of a non-null result, auxiliary measurements with other instruments may be able to rule out such systematic effects. 
For example, GNOME uses unshielded magnetometers to monitor the magnetic environment near the shielded dark matter sensors to veto signals from anomalously large local magnetic field excursions \cite{afach2018characterization}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Conclusion}

\medskip

\noindent\emph{Conclusion.~---~}In summary, we propose a new method to search for UBDM by using intensity interferometry with sensor networks. We show that when the sensors measure signals quadratic in the UBDM field, there is a near-dc component of the signal that enables finite-bandwidth sensors to search for UBDM with Compton frequencies many orders of magnitude larger than possible if a traditional search for signals oscillating at the Compton frequency is carried out. Here we have focused on quadratic UBDM interactions and sensors with a linear response; however, the results are also valid for linear interactions and sensors that respond quadratically to the field (square-law detectors). The method of intensity interferometry is intrinsically broadband, with the potential to search for UBDM with particle masses ranging over many orders of magnitude without having to probe individual narrow frequency bands. UBDM searches with intensity interferometry using existing sensor networks can probe unexplored parameter space.

%The technique presented relays on all sensors located in the same coherence patch. For this reason the sensitivity region is upper-bounded at $\approx10^{-10}$\,eV. GNOME would face challenges sensing fluctuations with a coherence time shorter than half a day corresponding to masses greater than $10^{-13}$\,eV due to the directional propierties of the. Due to the non-directional coupling to the atomic clocks   }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\section*{Acknowledgements}
\vspace{12pt}
The authors are sincerely grateful to Jason Stalnaker, Ibrahim Sulai, Maxim Pospelov, Arran Phipps, Ben Buchler, Ron Folman, and Menachem Givon for enlightening discussions. The authors also thank Tatum Wilson, Rayshaun Preston, Christopher Verga, and Mario Duenas for early work on simulations. This work was supported by the U.S. National Science Foundation under grant PHYS-2110388, by the Cluster of Excellence ``Precision Physics, Fundamental Interactions, and Structure of Matter'' (PRISMA+ EXC 2118/1) funded by the German Research Foundation (DFG) within the German Excellence Strategy (Project ID 39083149), by the German Federal Ministry of Education and Research (BMBF) within the Quantumtechnologien program (Grant No. 13N15064), by the European Research Council (ERC) under the European Union Horizon 2020 research and innovation program (project Dark-OST, grant agreement No 695405), and by the DFG Project ID 423116110.
The authors at Boston University acknowledge support from the Simons Foundation Grant No. 641332, the National Science Foundation CAREER Award No. PHY-2145162, the John Templeton Foundation Grant No. 60049570, and the U.S. Department of Energy, Office of High Energy Physics program under the QuantISED program, FWP 100495. The work of YVS was supported by the Australian Research Council under the Discovery Early Career Researcher Award DE210101593. The work of SP was supported by the National Science Centre of Poland within the grant No. 2020/39/B/ST2/01524



==> VersionControl/suppmat_20230407.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical simulation}\label{app:calculation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%This section describes the methods and parameters used in the simulations presented in the main text. %Figures~\ref{fig:g1} and~\ref{Fig:massdep} are generated by simulating the UBDM fields $\varphi_s^2$ and $\bs{\nabla} \varphi_s^2$. %These are defined in Eqs.\,\eqref{eq:field-squared} and~\eqref{eq:gradient-field-sqr}.
The detection scheme presented in the main text relies on the near-dc component of $\varphi^2$ and $\bs{\nabla} \varphi^2$ (denoted by the
subscript s). These are written as
\begin{align}
    \varphi_s^2(\bs{r},t) &= \frac{\varphi_0^2}{2N} \sum_{n,m=1}^N \cos \prn{\omega_{nm} t -\bs{k}_{nm} \cdot \bs{r}  +\theta_{nm}},\label{eq:field-squared}\\
    \bs{\nabla} \varphi_s^2(\bs{r},t) &=  \frac{\varphi_0^2}{2N} \sum_{n,m=1}^N   \bs{k}_{nm} \sin \prn{\omega_{nm} t -\bs{k}_{nm} \cdot \bs{r} +\theta_{nm}}, \label{eq:gradient-field-sqr} 
\end{align}
where $\omega_{nm}= \omega_{n} - \omega_{m}$, $\bs{k}_{nm} = \bs{k}_{n} - \bs{k}_{m}$, and $\theta_{nm}=\theta_{n} - \theta_{m}$. 
Since the sensors are assumed to be within the same coherence patch (such that $\Delta\bs{k} \cdot \Delta\bs{r} \approx 0$, where $\Delta \bs{k}$ is the characteristic spread of values in $\bs{k}_{nm}$ and $\Delta \bs{r}$ is the difference in the position vectors for the pair of sensors at $\boldsymbol{r}_n$ and $\boldsymbol{r}_m$), the $\bs{r}$ dependence can be neglected and we can evaluate the expressions at $\bs{r}=0$ in the following calculations~\cite{TruckNote}\nocite{grotti2018geodesy,takamoto2020test}.

To illustrate the stochastic properties of $\bs{\nabla} \varphi_s^2(0,t)$ and $\varphi_s^2(0,t)$, their time evolution was simulated. Plots of $g^{(1)}(\tau)$ for $\varphi_s^2(t)$ and for projections of $\bs{\nabla} \varphi_s^2(t)$ onto parallel and perpendicular directions with respect to $\bs{v}\ts{lab}$ can be seen in Fig.\,\ref{fig:g1}. Additionally, for the simplified case where $|\bs{v}_{\text{lab}}| \gg v_0$, an analytical expression for $g^{(1)}(\tau)$ can be found in Appendix~\ref{app:analytic}. Note that, as seen in Fig.\,\ref{fig:g1} and discussed in detail in Appendix~\ref{app:similarity}, the coherence time $\tau_c$ of $\bs{\nabla} \varphi_s^2(0,t)$ and $\varphi_s^2(0,t)$ is approximately half of that for the field $\varphi_s$. 

The characteristic coherence time of the field $\varphi$ is~\cite{derevianko2018detecting} 
\begin{equation}
    \tau_\varphi \approx \frac{2 \hbar}{ m_\varphi v_0^2},
    \label{eq:coherence_time}
\end{equation}
which is used as a benchmark timescale throughout the text.

\begin{figure}[ht]
\center
\includegraphics[width=\columnwidth,trim={0 5mm 0 3mm},clip]{Coherence.pdf}
\caption{\small{ Degree of first-order coherence as a function of delay time $\tau$ for $\varphi_s^2$ and different projections of the gradient $\bs{\nabla} \varphi_s^2$ relative to $\bs{v}_\ts{lab}$. Each curve is the result of 100~averages simulating $10^3$ particles, where the mean was subtracted (details in Appendix~\ref{app:calculation}). The approximate values of the coherence times are given in colors matching their respective plot traces.}}
\label{fig:g1}
\end{figure}

To perform the numerical calculations, we express the field in complex notation, 
\begin{equation}
	\varphi_c(0,t) =  \frac{\varphi_0}{\sqrt{N}} \sum_{n=1}^N \exp{[i (\omega_n t + \theta_n)]} .
	\label{eq:complex-field-sum}
\end{equation}
Then the near-dc component of the field squared is calculated
\begin{equation}
	\varphi_s^2 = \frac{1}{2} \varphi_c \varphi_c^* .
	\label{eq:complex-scalar-field-squared}
\end{equation}
This is a real number describing the average of $\varphi^2$ over a cycle of the oscillation. 

Similarly, $\bs{\nabla} \varphi_s^2$ is numerically evaluated by applying the chain rule
\begin{equation}
	\begin{split}
		\bs{\nabla} \varphi_s^2(\bs{r},t)\Bigr\rvert_{\bs{r} = 0} = & \frac{i}{2} \varphi_c \frac{\varphi_0}{\sqrt{N}} \sum_{n=1}^N \bs{k}_{n} \exp{[-i (\omega_n t + \theta_n)]} \\
		& - \frac{i}{2}\varphi_c^* \frac{\varphi_0}{\sqrt{N}} \sum_{n=1}^N \bs{k}_{n} \exp{[i (\omega_n t + \theta_n)]} . \label{eq:gradient-sum-two-terms}
	\end{split}
\end{equation}

Note that by first evaluating Eq.~\eqref{eq:complex-field-sum} to obtain $\varphi_c(0,t)$ and then evaluating Eqs.~\eqref{eq:complex-scalar-field-squared} and \eqref{eq:gradient-sum-two-terms} to find $\varphi_s^2$ and $\bs{\nabla} \varphi_s^2$, we need only calculate a few sums with $\mathcal{O}(N)$ terms for $N$ bosons. This is in contrast to the equivalent expressions presented in Eqs.\,\eqref{eq:field-squared}~and~\eqref{eq:gradient-field-sqr}, which have double sums with $\mathcal{O}(N^2)$ terms. This makes numerical calculations using Eqs.~\eqref{eq:complex-scalar-field-squared} and \eqref{eq:gradient-sum-two-terms} considerably more efficient for large $N$.

The individual wave vectors $\bs{k}_{n}$ and frequencies $\omega_{n}$ are calculated from the velocities $\bs{v}_{n}$. These are drawn from the displaced Maxwell-Boltzmann distribution
\begin{equation}
f_{\text{lab}}(\bs{v}) \approx \frac{1}{\pi^{3/2} v_0^3} \exp{\left(-\frac{(\bs{v-\bs{v}_{\text{lab}}})^2}{v_0^2}\right)}, \label{eq:f_lab_velocity}
\end{equation}
where the velocity of the lab frame is~$\bs{v}_{\text{lab}} = |\bs{v}_{\text{lab}}| \bs{\hat{z}}$, and we have ignored the escape velocity cut-off. In our simulations, we take the isotropic velocity dispersion of the local UBDM to be determined by the characteristic virial velocity $v_0\approx 220~\text{km}/\text{s}$, and $\bs{v}_{\text{lab}}$ to be dominated by the motion of the Sun in the galactic frame, $|\bs{v}_{\text{lab}}| \approx 233~\text{km}/\text{s}$. The phases $\theta_n$ are drawn from a uniform distribution spanning from $0$~to~$2\pi$.

The simulations consider $N=10^3$ bosons evolving during $20\,\tau_\varphi$ with a time resolution of $0.05\,\tau_\varphi$, where $\tau_\varphi$ is calculated using Eq.\,\eqref{eq:coherence_time}. Let us estimate the number density of particles in the UBDM field. For example, a UBDM mass of $10^{-11}$\,eV/$c^2$ (and a local energy density of $\rho\ts{dm} = 0.3$~GeV/cm$^3$) yields a number density of particles of $\sim \! 10^{19}$\,cm$^{-3}$. Also, consider that the de~Broglie wavelength, if the particles move with a velocity of $v_0$, is $\sim \! 10^{10}$\,cm. Therefore, a sensor will be interacting with a number of particles that cannot be simulated with the methods presented here within a reasonable time. Instead we chose $N=10^3$ as the number of particles that can be simulated with our available hardware. By repeating the simulation hundreds of times, we can observe that the results converge. Additional checks were made to ensure that the spectral properties of the simulations matched theoretical predictions. An analytical solution for $g^{(1)}(\tau)$ in the limit $|\bs{v}_{\text{lab}}| \gg v_0$ can be found in Appendix~\ref{app:analytic} which is shown to agree with our simulations. The temporal resolution and the duration of the simulated field evolution were chosen considering plausible values for an experimental search. 

After generating $\varphi_s^2$ and $\bs{\nabla} \varphi_s^2$, $g^{(1)}(\tau)$ is calculated using Eq.\,\eqref{eq:first-order-coherence-definition}. Note that the mean value of the field is subtracted so that $g^{(1)}(\tau) \rightarrow 0$ for $ \tau \gg \tau_\varphi$ (see Appendix~\ref{app:search}). The coherence time [as defined in Eq.\,\eqref{eq:coherence_time_def}] for these fields can be obtained by integrating numerically. The integration is realized considering the data over the time interval $[0,5\tau_\varphi]$, and multiplying by two in order to account for the negative segment of the range.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Coherence time}
\label{app:similarity}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We define the coherence time as the power-equivalent width of $g^{(1)}(\tau)$~\cite{loudon2000the,saleh2019fundamentals},
\begin{equation}
    \tau_c = \int_{-\infty}^{+\infty} |g^{(1)}(\tau)|^2 d\tau,
    \label{eq:coherence_time_def}
\end{equation}
which describes a characteristic temporal width of $g^{(1)}(\tau)$. The full width at half maximum of the~$\varphi$ lineshape is $\approx \omega_c v_0^2/c^2$, giving a useful estimate of the benchmark coherence time $\tau_\varphi$ of the field~(the result is exact for a Lorentzian lineshape~\cite{gramolin2021spectral}), see Eq.~\eqref{eq:coherence_time} in the main text. Note that there is an ambiguity, up to a factor of $2\pi$, in the definitions of $\tau_c$ used in the literature~\cite{Centers2019}. Because the actual lineshape describing $\varphi$ is expected to be non-Lorentzian \cite{gramolin2021spectral}, $\tau_\varphi$ slightly differs from the coherence time of the field $\varphi$ derived from the simulations. For the considered $\bs{v}_\ts{lab}$, simulations show a coherence time $\approx 1.12(1) \tau_\varphi$.

% Coherence time of $\varphi^2_s(0,t)$ and gradient
The coherence time for $\varphi^2_s$ is approximately half of that for the field $\varphi$. This is a result of the field $\varphi^2_s$ being a sum over terms depending on the difference of frequencies $\omega_{nm}$, as opposed to $\varphi$, which only contains terms depending on $\omega_n$. The probability distribution of $\omega_{nm}$ can be calculated as the convolution of the distribution of $\omega_n$ with itself. This results in a distribution for $\omega_{nm}$ that is broader. Consequently, the coherence time is shorter since $g^{(1)}(\tau)$ is given by the Fourier transform of the power spectral density of $\varphi^2_s$ (proportional to the $\omega_{nm}$ distribution), according to the Wiener–Khinchin theorem. The gradient coupling features even shorter coherence times due to the $\bs{k}_{nm}$ factor weighting the contribution of the oscillating terms. Larger $\omega_{nm}$ tends to correspond to larger $\bs{k}_{nm}$: this effectively broadens the power spectral density of $\bs{\nabla} \varphi^2_s$, leading to a shorter coherence time. This is also the reason why parallel and perpendicular components of the gradient have different coherence times, as discussed below.

% Refer to appendix with analytical expresions
A formal derivation of $g^{(1)}(\tau)$ for $\varphi^2_s$ and $\bs{\nabla} \varphi^2_s$ in the simplified case where $|\bs{v}_{\text{lab}}| \gg v_0$ can be found in Appendix~\ref{app:analytic}.

% Relate coherence time of the fields to mass
The coherence time is also related to the mass of the UBDM particle as can be seen in Eq.\,\eqref{eq:coherence_time}. The relationship between the UBDM mass and the coherence time exhibited by $\varphi^2_s$ and $\bs{\nabla} \varphi^2_s$ is shown in Fig.\,\ref{Fig:massdep}. The coherence times for $\varphi^2_s$ and $\bs{\nabla} \varphi^2_s$ are proportional to the coherence time of $\varphi$, $\tau_\varphi$ as defined in Eq.\,\eqref{eq:coherence_time}. In the case of detection, this could be used to estimate the mass of the UBDM particles.
\begin{figure}[ht]
\center
\includegraphics[width=\columnwidth,trim={0 5mm 0 3mm},clip]{MassVStc.pdf}
\caption{\small{Mass dependence of the characteristic delay time at which $g^{(1)}(\tau)=0.5$ for $\varphi_s^2$ and projections of $\bs{\nabla} \varphi_s^2$. Each point is the result of 100~averages simulating $10^3$ particles (details in Appendix~\ref{app:calculation}).}}
\label{Fig:massdep}
\end{figure}

The velocity offset due to the movement of the laboratory frame, here equivalent to the galactic velocity of Earth $\bs{v}_\ts{lab} = v_\ts{lab} \bs{\hat{z}}$, breaks the isotropy of the field. However, this anisotropy is not directly observed when measuring the average intensity because the quadratic interactions depend on the difference of wave-vectors and frequencies as can be seen in Eqs.\,\eqref{eq:field-squared}~and~\eqref{eq:gradient-field-sqr}. Yet, the coherence time of the field is different for directions parallel and perpendicular to $\bs{v}_\ts{lab}$ and depends on its magnitude.

\begin{figure}[ht]
	\center
	\includegraphics[width=\columnwidth]{tcVSvlab.pdf}
	\caption{\small{ Coherence time, as defined in Eq.\,\eqref{eq:coherence_time_def}, as a function of $\bs{v}_\ts{lab}$ for the different cases of the UBDM field $\varphi$ studied.}}
	\label{Fig:tcVSvab}
\end{figure}

To understand the influence of $\bs{v}_\ts{lab}$ on the coherence time it is instructive to consider the limiting cases: $\bs{v}_\ts{lab}=0$ and $| \bs{v}_\ts{lab} | \gg v_0$ . Decomposing $\bs{k}$ into parallel and perpendicular components to $\bs{v}_\ts{lab}$ yields the following relationships:
\begin{equation}
	\bs{k}^\parallel_{nm} = \frac{ m_\varphi \bs{v}^\parallel_{nm} }{\hbar},~\text{and}~\bs{k}^\perp_{nm} = \frac{ m_\varphi \bs{v}^\perp_{nm} }{\hbar}.
	\label{eq:k_nm}
\end{equation}
The velocity difference  $\bs{v}_{nm} = \bs{v}_{n}-\bs{v}_{m}$ and the superscripts $\parallel$ and $\perp$ indicate whether the component is parallel or perpendicular to $\bs{v}_\ts{lab}$. One can also write the difference of frequencies in terms of the galactic-rest-frame velocity components as
\begin{equation}
	\begin{split}
		\frac{2c^2\omega_{nm}}{\omega_c} =~&(\bs{v}^\parallel_{n} + \bs{v}^\parallel_{m})\cdot \bs{v}^\parallel_{nm} + (\bs{v}^\perp_{n} + \bs{v}^\perp_{m})\cdot\bs{v}^\perp_{nm} \\
		&+ 2\bs{v}_\ts{lab}\cdot\bs{v}^\parallel_{nm}.
		\label{eq:omega_nm}
	\end{split}
\end{equation}

For $\bs{v}_\ts{lab}\ll \bs{v}_\ts{0}$ there is almost no anisotropy and therefore parallel and perpendicular components of $\nabla\varphi^2(\bs{r},t)$ have the same coherence time. However, as can be seen in Eqs.\,\eqref{eq:k_nm} and \eqref{eq:omega_nm}, $\omega_{nm}$ and $\bs{k}_{nm}$ have different dependence on $\bs{v}_{nm}$. For $\bs{k}_\ts{nm}$ the relationship is linear, while for $\omega_\ts{nm}$ it is non-linear and depends on the product of the sum and the difference of velocities. This implies a nonlinear correlation between $\omega_{nm}$ and $\bs{k}_{nm}$ as can be seen in Fig.\,\ref{Fig:tcVSvab}. Larger $\bs{v}_{nm}$ correlates with larger $\omega_{nm}$ and $\bs{k}_{nm}$. Since the gradient coupling is weighted by $\bs{k}_{nm}$ [see Eq.\,\eqref{eq:gradient-field-sqr}], the larger $\omega_{nm}$ have more weight in the sum. This broadens the frequency spectrum and shortens the coherence time of the gradient with respect to the field squared as can be seen in Fig.\,\ref{Fig:tcVSvab}. 

For large $v_\ts{lab}$ the behavior of $\nabla_\perp\varphi^2$ resembles that of $\varphi^2$ (see Fig.\,\ref{Fig:tcVSvab}) because the perpendicular terms of the velocity $\bs{v}^\perp_{nm} $ contribute little to $\omega_{nm}$. Therefore, $\bs{k}^\perp_{nm}$ and $\omega_{nm}$ are effectively independent and Eq.\,\eqref{eq:gradient-field-sqr} resembles Eq.\,\eqref{eq:field-squared} if multiplied by an appropriate scaling factor. 

In contrast, the coherence time of $\nabla_\parallel\varphi^2$ reduces faster than that of $\varphi^2$ as can be seen in Fig.\,\ref{fig:correlation}. The reason for this is that for large $v_\ts{lab}$, $\omega_{nm}$ becomes approximately $\propto \bs{k}^\parallel_{nm}$ and this proportionality scales with $v_\ts{lab}$. This increases the weight in the sum of terms with large $\omega_{nm}$ [in Eq.\,\eqref{eq:gradient-field-sqr}], leading to a broader power spectrum and consequently, a shorter coherence time. 

In the derivation of Eq.~\eqref{eq:ALP-intensity-gradient} in the main text we assumed that the average spread of values of $\hat{\bs{m}}\cdot\bs{k}_{nm}$ is $\approx m_\varphi v_0/\hbar$. This estimate implicitly assumes that $\omega_{nm}$ and $\bs{k}_{nm}$ are uncorrelated, and thus the accuracy of this approximation varies with $\bs{v}\ts{lab}$. Nonetheless, Eq.\,\eqref{eq:ALP-intensity-gradient} is suitable for a rough estimate of the sensitivity of a magnetometer network to such UBDM, given that $|\bs{v}\ts{lab}| \approx v_0$.

\begin{figure}[ht]
	\center
	\includegraphics[width=\columnwidth]{Correlation.pdf}
	\caption{\small{ Visualization of the dependence of $\omega_{nm}$ on $\bs{v}_{nm}^\perp$ and $\bs{v}_{nm}^\parallel$. The Monte Carlo simulation was performed drawing $10^5$ velocities from the distribution in Eq.~\eqref{eq:f_lab_velocity}. The number of instances in which $\bs{v}^\perp_{nm} $ or $\bs{v}^\parallel_{nm}$ results in a $\omega_{nm}$ within a 20 km/s $\times 4.6 \times 10^{-7}$ s$^{-1}$ bin is represented in color. The black contour-lines indicate when the number of counts is $10^1$, $10^2$ or $10^3$ and serve as a guide to illustrate the shape of the distributions. }}
	\label{fig:correlation}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Search with correlated sensor networks}\label{app:search}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Introduce use of stochastic properties
The stochastic properties of $\varphi^2_s$ and $\bs{\nabla}\varphi^2_s$ can be used to search for UBDM. However, magnetometers and optical clocks are subjected to systematic noise sources in the laboratory, which feature some degree of temporal self-coherence similar to the UBDM field. For this reason, we focus our search on the cross-correlation of independent sensors, as their noise can be assumed to be mostly uncorrelated. 

Prosaic natural phenomena may also limit the sensitivity of a sensor network. Known natural phenomena that could generate noise with long-range correlations include, for example, time-dependent electromagnetic fields associated with cavity resonances of the conducting Earth-ionosphere cavity \cite{fedderke2021earth} (such as the Schumann resonances \cite{schumann1952strahlungslosen}) and vibrational noise due to free oscillations of the Earth excited by large earthquakes \cite{hu2020network} (such as the ``breathing'' mode of the Earth at $\approx 800~{\rm \mu Hz}$ \cite{dziewonski1981preliminary,rosat2007geographical}). Auxiliary measurements with other instruments may be able to rule out such systematic effects. For example, GNOME uses unshielded magnetometers to monitor the magnetic environment near the shielded dark matter sensors to veto signals from anomalously large local magnetic field excursions \cite{afach2018characterization}. The possibility of the data containing non-dark-matter long-range correlated signals is not considered in this analysis.

%Definitions
In order to illustrate a possible method that could be used to search for UBDM fields using intensity interferometry, let us consider a measured time-series $\tilde{\mc{S}}_{A,B}(t)$ lasting several $\tau_{\varphi}$ from two different sensors, $A$~and~$B$. These time-series have their mean subtracted, such that $\mc{S}_{A,B} = \tilde{\mc{S}}_{A,B} - \langle \tilde{\mc{S}}_{A,B} \rangle_t$. The measurement in each sensor would have a small UBDM-related component $\kappa s(t)$, and a noise term $\mc{N}(t)$, $\mc{S}_{A,B} = \kappa_{A,B} s_{A,B}(t) + \mc{N}_{A,B}(t)$. The factor $\kappa_{A,B}$ accounts for coupling of the sensor to the UBDM field, and $s_{A,B}(t)$ is either $\varphi^2_s$ (scalar interaction) or $\hat{\bs{m}} \cdot \bs{\nabla} \varphi^2_s$ (pseudoscalar gradient interaction).

%Derive the auto-correlation (equivalent to cross-correlation) signal for clocks and magnetometers.
For a particular time series the degree of first-order coherence of these signals can be calculated as
\begin{equation}
	g^{(1)}_{AB}(\tau) = \frac{\langle \mc{S}_A(t) \mc{S}_B(t+\tau) \rangle_t}{\sqrt{\langle \mc{S}_A^2 \rangle_t \langle \mc{S}_B^2 \rangle_t}}.
	\label{eq:g1appc}
\end{equation}
%Uncorrelated noise terms to 0
While the signals $s_A(t)$ and $s_B(t)$ are correlated, the corresponding noise contributions, $\mc{N}_A(t)$ and $\mc{N}_B(t)$, are not. As a consequence, one can suppress the cross-terms $\langle \mc{N}_A \mc{N}_B \rangle_t$, $\langle \mc{N}_A s_B \rangle_t$, and $\langle \mc{N}_B s_A \rangle_t$ with sufficient amount of averaging (determined by the signal-to-noise ratios of sensors $A$ and $B$). Then, Eq.\,\eqref{eq:g1appc} reduces to
\begin{equation}
	g^{(1)}_{AB}(\tau) = \kappa_A \kappa_B \frac{ \langle  s_A(t) s_B(t+\tau) \rangle_t}{\sqrt{\langle \mc{S}_A^2 \rangle_t \langle \mc{S}_B^2 \rangle_t}}.
\end{equation}

%Mention sensors should be within de Broglie wavelength to meaure correlated signal (could scan distance).}
Strictly speaking, there will be a difference between $s_A(t)$ and $s_B(t)$ because of the spatial dependence of $\varphi^2$  (or $\bs{\nabla} \varphi^2$) that arises from the $\bs{k}\cdot \bs{r}$ term in Eq.\,\eqref{eq:single-boson-field}. However, for the considered UBDM mass range, the coherence length is much larger than the distance between the sensors. Therefore, $\varphi^2_s$ (or $\bs{\nabla} \varphi^2_s$) will approximately be the same for both sensors, $s_{A,B}(t) \approx s(t)$; and so $g^{(1)}(\tau)$ is proportional to the autocorrelation of the slow-varying component of the UBDM field squared~(or its gradient):
\begin{equation}
	\label{eq:g_tau_simple}
	g^{(1)}_{AB}(\tau) \approx \frac{\kappa_A \kappa_B}{\sqrt{\langle \mc{S}_A^2 \rangle_t \langle \mc{S}_B^2 \rangle_t}}\langle s(t) s(t+\tau) \rangle_t.
\end{equation}

As an example, evaluating Eq.\,\eqref{eq:g_tau_simple} at $\tau=0$ yields
\begin{equation}
	g^{(1)}_{AB}(0) \approx \frac{\kappa_A \kappa_B}{\sqrt{\langle \mc{S}_A^2 \rangle_t \langle \mc{S}_B^2 \rangle_t}}\langle s^2 \rangle_t .
	\label{eq:g1ofzero}
\end{equation}
The quantity $g^{(1)}(0)$ can be used as an estimator for the slow-varying component (of the gradient) of the field squared; it can be used to determine whether or not a UBDM signal is present in the data. For the scalar interaction, $\langle s^2 \rangle_t = \langle \varphi^2_s \varphi^2_s  \rangle_t$ and it can be shown  that for the gradient interaction $\langle s^2 \rangle_t = \prn{\cos \vartheta_{AB}/3} \langle \bs{\nabla}\varphi^2_s \cdot \bs{\nabla}\varphi^2_s  \rangle_t$, where $\vartheta_{AB}$ is the angle between the sensitive axes of the two sensors, $\bs{\hat{m}}_A$ and $\bs{\hat{m}}_B$ (see Appendix~\ref{app:AngleDep}). Assuming Gaussian noise with standard deviation $\sigma$, $\mc{N}\sim \mc{G}(0,\sigma^2)$, that dominates over the UBDM-signal component, $ \kappa s \ll \sigma$, Eq.\,\eqref{eq:g1ofzero} can be simplified to:
\begin{equation}
	g^{(1)}_{AB}(0) \approx \frac{\kappa_A \kappa_B}{\sigma_A \sigma_B}\langle s^2 \rangle_t.
	\label{eq:g0approx}
\end{equation}
%In order to improve the accuracy to $g^{(1)}(0)$, one can average this value over measurements with different independent pairs of sensors since noise in the sensor leads to $|g^{(1)}(0)|<1$. If this value is significantly greater than zero, one can conclude that a common correlated signal is present in the data, as could arise from UBDM. This method is inherently broadband, as a large range of UBDM masses could lead to $|g^{(1)}(0)|>0$.
The presence of a common correlated UBDM signal between two sensors will lead to a nonzero $g^{(1)}(0)$. This method is inherently broadband, as a large range of UBDM masses could lead to $|g^{(1)}(0)|>0$. 

In order to estimate the sensitivity to a nonzero $g^{(1)}(0)$, we assume $N_m$ identical sensors having the same directional sensitivity and dominated by Gaussian noise with the same variance (of course, this is not the typical case for real networks, these feature different directional sensitivities -- see Appendix~\ref{app:AngleDep} -- and are affected by $1/f$ noise).
In the cases of interest, the coherence length of the UBDM is much larger than the spacing between the sensors, so the UBDM signal will be identical in all sensors. 
To understand the scaling of the sensitivity with $N_m$, $\tau_\varphi$, and total acquisition time $T$, suppose that we divide the network into two distinct groups each with $N_m/2$ sensors and average the data in each group. 
Furthermore, suppose that the time-series data are binned in $\tau_\varphi$-long segments and time-averaged in each bin. 
Based on this approach, in the absence of a correlated UBDM signal, each group of sensors will exhibit a bin-to-bin variance in the measured magnetic field of approximately $\delta B / \sqrt{\tau_\varphi N_m/2} \sim \delta B / \sqrt{\tau_\varphi N_m}$, where $\delta B$ is the sensitivity of a single magnetometer in units of magnetic field strength times the square root of time. For a total acquisition time $T$, there will be $N_b = T/\tau_\varphi$ bins.
The expected residual from noise in the cross-correlation between the two groups provides an estimate of the network resolution, which in turn gives the minimum detectable pseudo-magnetic field squared 
\begin{align}
    \abrk{ \mc{B}_q({\rm{min}})^2 }_t \approx \frac{\delta B^2}{N_m \tau_\varphi}\frac{1}{\sqrt{N_b}} \approx \frac{\delta B^2}{N_m \sqrt{\tau_\varphi T}}~.
    \label{eq:min-field}
\end{align}
An in-depth discussion of the $T$ and $N_m$ scaling for a similar case can be found in Ref.~\cite{derevianko2018detecting}.


This scheme does not rely on the boson having a Compton wave resonant with the experimental set-up. Such resonant searches require the interrogation of numerous narrow frequency bands which is a time-consuming process \cite{Asz01,Asz10,budker2014proposal,Sik14,chaudhuri2015radio,phipps2020exclusion,manley2020searching,crescini2020axion,braine2020extended,backes2021quantum,Ayb21CASPErE}.
In the case of detection in a search for correlated stochastic fluctuations, the mass range of the UBDM particle could be narrowed by analyzing the coherence time, as illustrated in Fig.~\ref{Fig:massdep} in Appendix~B.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Angle dependence of the correlation between magnetometers}\label{app:AngleDep}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Introduce problem
We are interested in understanding the coherence between two signals, $s_A$ and $s_B$, that are the result of the gradient coupling. In particular, for $j\in\{A,B\}$, let $\boldsymbol{\hat{m}_j}$ be the sensitive axis of magnetometer $j$, so $s_j = \boldsymbol{\hat{m}_j} \cdot \boldsymbol{\nabla} \varphi^2_s$. The calculation of the coherence requires one to understand $\left< s_A s_B \right>_t$, but each $s_A$ and $s_B$ depends on the relative angle between the respective sensitive axis and the field gradient. These angles are not known and change over time as the field evolves.

% Define assumptions
Note that $\boldsymbol{\nabla} \varphi^2_s$ is a sum of terms $\propto \bs{v}_{nm}$. The angle dependence between the field gradient and the sensitive axes can be accounted for under some basic assumptions. In particular, assume that $\boldsymbol{v}_{nm}$ is ergodic in direction --- that is, over time, $\boldsymbol{\hat{v}}_{nm}$ will take all values over the sphere $S^2$.
Ergodicity implies that $\left< s_A s_B\right>_t = \left< s_A s_B\right>_{S^2}$.
As another simplifying assumption, let $v^2$ be independent of $\boldsymbol{\hat{m}_j}\cdot \boldsymbol{\hat{v}}_{nm}$ so 
\[
\left< (\boldsymbol{\hat{m}_A}\cdot \boldsymbol{v}_{nm})(\boldsymbol{\hat{m}_B}\cdot \boldsymbol{v}_{nm}) \right>_t = \bar{v}^2 \left< (\boldsymbol{\hat{m}_A}\cdot \boldsymbol{\hat{v}}_{nm})(\boldsymbol{\hat{m}_B}\cdot \boldsymbol{\hat{v}}_{nm}) \right>_t\ ,
\]
for $\bar{v}^2 = \left< \lVert \boldsymbol{v}_{nm} \rVert^2 \right>_t$.

% Calculate the dependence
The correlation between magnetometers can be calculated explicitly with the above assumptions. This will still depend on the relative angle $\vartheta_{AB}$ between the sensitive axes $\boldsymbol{\hat{m}_A}$ and $\boldsymbol{\hat{m}_B}$. Let us define the axes such that $\boldsymbol{\hat{m}_B}$ points along the $z$-axis and $\boldsymbol{\hat{m}_A}$ lies in the $xz$-plane in the $+x$-direction. The gradient direction $\boldsymbol{\hat{v}}$ can be arbitrary, described by the azimuthal angle $\phi$ and polar angle $\theta$ in this coordinate system. Thus
\begin{align*}
	\boldsymbol{\hat{m}_A} &= \left( \sin\vartheta_{AB}, 0, \cos\vartheta_{AB} \right)\ , \\
	\boldsymbol{\hat{m}_B} &= (0, 0, 1)\ , \\
	\boldsymbol{\hat{v}}_{nm} &= \left( \cos\phi \sin\theta, \sin\phi \sin\theta, \cos\theta \right)\ .
\end{align*}
The following calculation can be made explicitly:
\begin{align}
	\left<s_As_B\right>_t &\approx \left<s_As_B\right>_{S^2} \nonumber \\
	&= \frac{\bar{v}^2}{4\pi}\int_0^{2\pi}d\phi \int_0^\pi d\theta ( \sin\vartheta_{AB} \cos\phi\sin\theta \nonumber \\
	& \qquad +\cos\vartheta_{AB} \cos\theta )\cos\theta\sin\theta \nonumber \\
	&= \frac{\bar{v}^2}{3} \cos\vartheta_{AB}\ ,
	\label{eq:angledep}
\end{align}
where the $\sin\vartheta_{AB}$ term averages out over the sphere over both the azimuthal and polar directions. 

\begin{figure}
	\center
	\includegraphics[width=\columnwidth]{AngleDependance.pdf}
	\caption{\small{$g^{(1)}(0)$ of $\hat{\bs{m}}_A \cdot \bs{\nabla} \varphi_s^2$ and $\hat{\bs{m}}_B \cdot \bs{\nabla} \varphi_s^2$ as a function of the relative angle between $\hat{\bs{m}}_A$ and $\hat{\bs{m}}_B$, $\vartheta_{AB}$. No noise was added to the generated fields. The blue dots are the results of independent simulations where the sensitive axes are randomly generated on the sphere. The red curve shows the $\cos(\vartheta_{AB}$) as predicted in Eq.\,\eqref{eq:angledep}.}}
	\label{Fig:angledep}
\end{figure}

The results of simulations shown in Fig.\,\ref{Fig:angledep} illustrate this dependence. An interesting feature is that the dispersion in $g^{(1)}(0)$ also depends on the relative angle between the magnetometers. This dispersion in $g^{(1)}(0)$ is not due to noise, as noise was not added to the simulated magnetometer data, but rather results from the UBDM fields themselves. If the sensitive axes of the sensors are not parallel,  dispersion in $g^{(1)}(0)$ is introduced by the uncorrelated components of the UBDM field measured; because the orthogonal components of $\bs{\nabla} \varphi_s^2$ (e.g., along $\hat{x},\hat{y},\hat{z}$) are uncorrelated, measuring different orientations produces a spread in $g^{(1)}(0)$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analytic solution for \texorpdfstring{$g^{(1)}(\tau)$}{g1(t)}}
\label{app:analytic}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this Appendix, an analytic expression for the degree of coherence is derived. Let us consider a signal given by the sum of sinusoidal functions,
\begin{equation}\label{eq:sinSumSig}
	S(t) = \sum_n a_n \cos\left( \omega_n t + \phi_n \right)\,.
\end{equation}
For simplicity, we consider the case in which the average signal is zero, $\omega_n\neq0$, and the frequencies are all different, $\omega_n\neq\omega_m$ for $m\neq n$. Considering the two-point correlation function defined as,
\begin{equation}
	C_2(\tau) = \left< S(t)S(t+\tau) \right>_t\,,
\end{equation}
then $g^{(1)}(\tau) = C_2(\tau)/C_2(0)$. 

% two-pt corr funct exact
When averaging over the product of the two signal functions, the oscillating components average out. As a result, the only components that contribute to the coherence are from products of the same sinusoidal terms. The resulting two-point correlation function is then
\begin{equation}\label{eq:sinSum2ptCorr}
	C_2(\tau) = \frac{1}{2} \sum_n a_n^2 \cos\left( \omega_n\tau \right)\,.
\end{equation}

% distribution of frequencies
For this study, we consider the case in which there are $N\gg 1$ sinusoidal components in the signal. The frequencies $\omega_n$ and amplitudes $a_n$ are sampled from some probability distribution. Here, this distribution is derived from a distribution of particle velocities $P_v(\boldsymbol{v})d^3\boldsymbol{v}$ given by Eq.\,\eqref{eq:f_lab_velocity}. 

We approximate the sum in Eq.\,\eqref{eq:sinSum2ptCorr} as an integral in which $a_n^2$ is replaced with the differential $a^2(\boldsymbol{x})P(\boldsymbol{x}) d\boldsymbol{x}$,
\begin{equation}\label{eq:sinInt2ptCorr}
	C_2(\tau) = \frac{1}{2} \int d\boldsymbol{x}\,a^2(\boldsymbol{x})P(\boldsymbol{x}) \cos\left[\omega(\boldsymbol{x}) \tau \right]\,.
\end{equation}

% case for both couplings
Here, for both the $\varphi^2$- and $\bs{\nabla}\varphi^2$-coupling, the probability distribution function is parameterized by $\boldsymbol{x}=\{ \boldsymbol{k_1}, \boldsymbol{k_2} \}$, for $\boldsymbol{k_i}=(m_\varphi / \hbar)\boldsymbol{v_i}$ described by a Gaussian distribution of velocities offset by the laboratory reference frame. It is useful to consider the average $\boldsymbol{\bar{k}}=(\boldsymbol{k_1}+\boldsymbol{k_2})/{2}$ and difference $\boldsymbol{\Delta} = \boldsymbol{k_1} - \boldsymbol{k_2}$. In these variables, $d^3\boldsymbol{k_1}d^3\boldsymbol{k_2}=d^3\boldsymbol{\bar{k}}d^3\boldsymbol{\Delta}$ and the difference in frequencies $\omega_{12} = (\hbar/m_\varphi) \boldsymbol{\bar{k}}\cdot\boldsymbol{\Delta}$. For either coupling, the contribution from $\mathcal{O}(2\omega_c)$ frequency components and the constant offset will be neglected. Also, let $\sigma_k=(m_\varphi / \hbar)\sigma_v$ ($v_0^2=2\sigma_v^2$) describe the width of the $\boldsymbol{k}$-vector distribution and $\boldsymbol{k_\text{lab}} = ({m_\varphi}/{\hbar}) \boldsymbol{v_\text{lab}}$ describe the offset of the distribution due to the laboratory reference frame. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{coherence_analytic}
    \caption{\small{Coherence of different signal types from numeric simulations (solid) compared to their analytic approximations (dashed, given by Eqs.\,\eqref{eq:g1_analytic_phi2}\,,\,\eqref{eq:g1_analytic_grad_phi2}). To better reflect the approximation conditions, the lab velocity is tripled, $v_\text{lab}=699$\,km/s (while $v_0$ is kept at $220$\,km/s). The analytic approximation for $\varphi_s^2$ is the same as for the gradient coupling for a $\boldsymbol{\hat{m}}$ perpendicular to the lab velocity $\nabla_\perp\varphi_s^2$.}}
    \label{fig:coherence_analytic}
\end{figure}

% \phi^2 coupling
For a signal given by $\varphi_s^2$, the amplitude of a sinusoidal component is constant while the frequency is given by the difference $\omega(\boldsymbol{k}_1) - \omega(\boldsymbol{k}_2)$. The integral in Eq.\,\eqref{eq:sinInt2ptCorr} can be approximated for $k_\text{lab} \gg \sigma_k$. Under this approximation, $\boldsymbol{\bar{k}}\approx\boldsymbol{k_\text{lab}}$ (i.e., one can neglect the uncertainty in the average $\boldsymbol{\bar{k}}$), which reduces the six-dimensional integral to a three-dimensional integral over $\boldsymbol{\Delta}$. The result is the degree of first-order coherence (see Fig.\,\ref{fig:coherence_analytic})
\begin{equation}
	g^{(1)}(\tau) \approx \exp\left[ -\left( \frac{m_\varphi v_\text{lab} \sigma_v}{\hbar} \right)^2 \tau^2 \right]\,.
	\label{eq:g1_analytic_phi2}
\end{equation}
Note that we consider a lab-frame for which $v_\ts{lab}\approx v_k$, so this is only a rough approximation. Heuristically, one would expect that the coherence is overestimated, because this approximation neglects a component of the frequency dispersion. 

% grad(\phi^2)
A signal given by coupling to the gradient $\nabla \varphi_s^2$ will have amplitudes of different sinusoidal components $\sim \boldsymbol{\hat{m}}\cdot\boldsymbol{\Delta}$. Here, we denote the angle between $\boldsymbol{\hat{m}}$ and $\boldsymbol{v_\text{lab}}$ with $\theta$. Using the approximation $k_\text{lab} \gg \sigma_k$ as before, the coherence is (see Fig.\,\ref{fig:coherence_analytic})
\begin{align}
	g^{(1)}(\tau) &\approx \frac{\sin^2(\theta) + 2\pi\left[ 1-2\left( \frac{m_\varphi}{\hbar} v_\text{lab} \sigma_v \tau \right)^2 \right]\cos^2(\theta) }{\sin^2(\theta) + 2\pi\cos^2(\theta) } \nonumber \\
	&\qquad\times\exp\left[ -\left( \frac{m_\varphi v_\text{lab} \sigma_v}{\hbar} \right)^2 \tau^2 \right]\,.
	\label{eq:g1_analytic_grad_phi2}
\end{align}
Observe that the coherence becomes negative for $\theta\neq \pi/2$ when
\begin{equation}
    \tau>\frac{\hbar}{m_\varphi v_\text{lab} \sigma_v}\sqrt{\frac{1}{2}+\frac{\tan^2(\theta)}{2\pi}}.
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Back-action effects}
\label{app:back-action}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As noted in the main text, a consideration particular to searches for ultralight scalar fields with quadratic couplings to SM particles and fields is the possible back-action of mass density on the scalar field, which can either reduce or enhance the field amplitude \cite{stadnik2020new,Oli08,hinterbichler2010screening,jaffe2017testing,hees2018violation}. This back-action arises due to the fact that the bare potential for the scalar field, namely $m_\varphi^2 c^2 \varphi^2/(2 \hbar^2)$, is modified by the presence of the Lagrangian in Eq.\,\eqref{eq:scalar-Lagrangian}. 

The quadratic terms in the interaction Lagrangian endow the scalar field with an effective mass $m\ts{eff}$ in the presence of matter; this effect is analogous to the screening of magnetic fields caused by the Meissner effect~(where the photon gains an effective mass inside a superconductor). Depending on the sign of the interaction, back-action can lead to either screening or antiscreening \cite{hees2018violation}.

For the interaction between $\varphi$ and the electromagnetic field leading to variation of $\alpha$ considered in Eq.~\eqref{eq:scalar-Lagrangian}, in the presence of matter the scalar field acquires an effective mass given by
\begin{align}
m^2_\ts{eff} \approx m_\varphi^2 \pm \frac{2 \hbar^3}{c} \frac{\rho_\gamma}{\Lambda_\gamma^2}~,
    \label{eq:effective-scalar-mass}
\end{align}
where $\rho_\gamma \approx -F_{\mu\nu}^2/4$ is the Coulomb energy density of a nonrelativistic nucleus averaged over the characteristic volume outside of which the UBDM field changes appreciably, which in our considered case is orders of magnitude larger than the size of a nucleus and thus depends on the average local matter density. Based on the numerical estimates of Ref.\,\cite{stadnik2020new}, for the Earth's interior $\rho_\gamma \approx 6 \times 10^{21}~{\rm GeV/cm^3}$ and for Earth's atmosphere $\rho_\gamma \approx 6 \times 10^{17}~{\rm GeV/cm^3}$. The (anti)screening effect due to back-action can be important if
\begin{align}
    m_\varphi^2 \Lambda_\gamma^2  \lesssim \frac{2 \hbar^3}{c} \rho_\gamma~.
    \label{eq:screening-limit}
\end{align}

Based on Eq.~\eqref{eq:screening-limit}, for values of $m_\varphi\Lambda_\gamma$ above the long-dashed blue line in Fig.~\ref{Fig:sensitivity-clocks} (anti)screening effects can be important and cover the entire range of parameter space accessible with a network of current optical atomic clocks. Here $\rho_\gamma$ for Earth's interior is used since this is the relevant value for the long-wavelength interactions considered. Thus sensitivity to positive-signed quadratic scalar interactions [as in Eq.~\eqref{eq:effective-scalar-mass}] is significantly diminished near Earth's surface. On the other hand, a space-based clock \cite{schiller2007optical,Schkolnik2022Apr} (or atom interferometer \cite{arvanitaki2018search}) network could largely avoid such screening effects due to the significantly lower average mass density in the interplanetary medium. In the case of negative-signed quadratic scalar interactions [as in Eq.~\eqref{eq:effective-scalar-mass}], there is antiscreening and the field amplitude can be significantly enhanced \cite{hees2018violation}. However, further analysis is required to calculate the form of the signal from stochastically fluctuating UBDM in this scenario. Finally, we note that constraints on coupling constants based on screening and antiscreening of scalar fields can be derived from experiments testing the equivalence principle \cite{hees2018violation}.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Heuristic argument for the difference in sensitivity between magnetometers and clocks }
\label{app:SensiticityDifference}

As can be seen in Figs.\,\ref{Fig:sensitivity-GNOME} and \ref{Fig:sensitivity-clocks}, the sensitivity of an optical clock network to the coupling parameter $1/\Lambda_\gamma$ far exceeds that of magnetometer networks to the equivalent coupling parameter $1/f_q$. 
Here we offer a heuristic explanation for this difference between the two cases. 
In the case of the scalar interaction [described by Eq.\,\eqref{eq:scalar-Lagrangian}] probed by clocks, the UBDM field modulates the electromagnetic binding energy of the atom [$\sim e^2/(2a_B) \approx \alpha^2 m_e c^2/2$, where $e$ is the electron charge magnitude, $a_B$ is the Bohr radius, and $m_e$ is the electron mass]. 
This effect leads to an energy shift approximately given by
\begin{align}
    \Delta E\ts{clock} \sim \prn{\frac{\hbar c \varphi_s^2}{\Lambda_\gamma^2}} \times \prn{\frac{1}{2} \alpha^2 m_e c^2}~,
    \label{eq:clock-energy-shift-order-of-mag}
\end{align}
where the first factor in parentheses describes the effective coupling constant associated with the UBDM field (proportional to the UBDM-induced fractional energy shift) and the second factor in the parentheses describes the scale of the electromagnetic binding energy of the atom. 
This manifestation of the scalar coupling is seen from the fact that it results in an effective modulation of the fine-structure constant $\alpha$ and/or electron mass $m_e$ as described by Eqs.\,\eqref{eq:scalar-mass-variation} and \eqref{eq:scalar-alpha-variation}. 
In the case of the pseudoscalar interaction Eq.~\eqref{eq:quadratic-Hamiltonian} probed by magnetometers, it is the energy associated with the field gradient ($\sim m_\varphi c v_0$) that is modulated, leading to an energy shift approximately given by %\draftNote{Revise dependence with $v\ts{lab}$} \DK{I think we can use $v_0$.}
\begin{align}
    \Delta E\ts{mag} \sim \prn{\frac{\hbar c \varphi_s^2}{f_q^2}} \times \prn{m_\varphi c^2 \frac{v_0}{c}}~.
    \label{eq:mag-energy-shift-order-of-mag}
\end{align}
By comparing Eqs.\,\eqref{eq:clock-energy-shift-order-of-mag} and \eqref{eq:mag-energy-shift-order-of-mag}, it is evident that the scale of the fractional energy modulation given by the first numerator in parentheses is similar in the two cases. 
Taking the ratio between the two energy shifts yields
\begin{align}
\frac{\Delta E\ts{clock}}{\Delta E\ts{mag}} \sim \frac{f_q^2}{\Lambda_\gamma^2} \frac{\alpha^2}{2}  \frac{c}{v_0} \frac{m_e}{m_\varphi}~,
\end{align}
and thus the ratio of the squares of the coupling constants determined by given energy shift measurements is
\begin{align}
\frac{\Lambda_\gamma^2}{f_q^2} \sim \frac{\Delta E\ts{mag}}{\Delta E\ts{clock}} \frac{\alpha^2}{2}  \frac{c}{v_0} \frac{m_e}{m_\varphi} \sim 0.1 \frac{\Delta E\ts{mag}}{\Delta E\ts{clock}} \frac{m_e}{m_\varphi}~.
\end{align}\\
For $m_\varphi c^2 \sim 10^{-14}~{\rm eV}$, $\Delta E\ts{mag} \sim 10^{-19}~{\rm eV}$ (corresponding to a magnetic field measurement at the level of a few pT for a nuclear spin), $\Delta E\ts{clock} \sim 10^{-16}~{\rm eV}$ (corresponding to a fractional uncertainty in a measurement of an optical transition at the $10^{-16}$ level) and $c/v_0 \sim 10^3$, we see that $\Lambda_\gamma^2/f_q^2 \sim 10^{15}$. This estimate demonstrates that the source of the enhanced sensitivity of clocks is from the large $m_e/m_\varphi$~mass ratio, expected for UBDM ($m_\varphi \ll 1$~eV/$c^2$).\\


==> VersionControl/suppmat_long.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical simulation}\label{app:calculation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\DK{This section needs a little introductory sentence to explain what all this is about and what the purpose is, just to orient the reader and ease them into the technical discussion.} 

This section describes the methods and parameters used in the simulations presented in the main text. Figures~\ref{fig:g1} and~\ref{Fig:massdep} are generated by simulating the UBDM fields $\varphi^2$ and $\bs{\nabla} \varphi_s^2$. These are defined in Eqs.\,\eqref{eq:field-squared} and~\eqref{eq:gradient-field-sqr}. 

To perform the numerical calculations, we express the field in complex notation, 
\begin{equation}
	\varphi_c(0,t) =  \frac{\varphi_0}{\sqrt{N}} \sum_{n=1}^N \exp{[i (\omega_n t + \theta_n)]} .
	\label{eq:complex-field-sum}
\end{equation}
Then the near-dc component of the field squared is calculated
\begin{equation}
	\varphi_s^2 = \frac{1}{2} \varphi_c \varphi_c^* .
	\label{eq:complex-scalar-field-squared}
\end{equation}
This is a real number describing the average of $\varphi^2$ over a cycle of the oscillation. 

Similarly, $\bs{\nabla} \varphi_s^2$ is numerically evaluated by applying the chain rule
%\DK{OK, now I think I understand it. I have made some edits below, see if they make sense!}
\begin{equation}
	\begin{split}
		\bs{\nabla} \varphi_s^2(\bs{r},t)\Bigr\rvert_{\bs{r} = 0} = & \frac{i}{2} \varphi_c \frac{\varphi_0}{\sqrt{N}} \sum_{n=1}^N \bs{k}_{n} \exp{[i (\omega_n t + \theta_n)]} \\
		& - \frac{i}{2}\varphi_c^* \frac{\varphi_0}{\sqrt{N}} \sum_{n=1}^N \bs{k}_{n} \exp{[-i (\omega_n t + \theta_n)]} . \label{eq:gradient-sum-two-terms}
	\end{split}
\end{equation}

%\begin{equation}
%	\begin{split}
%		\bs{\nabla} \varphi_s^2(\bs{r},t)= %\frac{1}{2} \bs{\nabla}  \varphi_c %\varphi_c^* = \frac{1}{2} (\varphi_c^* %\bs{\nabla}  \varphi_c + \varphi_c %\bs{\nabla}  \varphi_c^*)
%	\end{split}
%\end{equation}

%\begin{equation}
%	\begin{split}
%		\bs{\nabla}  \varphi_c = \frac{a_0^2}{2 N} %\sum_{n=1}^N i \bs{k_n} \exp{[i (\omega_n t %+ \phi_n)]}
%	\end{split}
%\end{equation}

Note that by first evaluating Eq.~\eqref{eq:complex-field-sum} to obtain $\varphi_c(0,t)$ and then evaluating Eqs.~\eqref{eq:complex-scalar-field-squared} and \eqref{eq:gradient-sum-two-terms} to find $\varphi_s^2$ and $\bs{\nabla} \varphi_s^2$, we need only calculate a few sums with $\mathcal{O}(N)$ terms for $N$ bosons. This is in contrast to the equivalent expressions presented in the main text, Eqs.\,\eqref{eq:field-squared}~and~\eqref{eq:gradient-field-sqr}, which have double sums with $\mathcal{O}(N^2)$ terms. This makes numerical calculations using Eqs.~\eqref{eq:complex-scalar-field-squared} and \eqref{eq:gradient-sum-two-terms} considerably more efficient for large $N$.
%these expressions is preferable to those presented in the main text, Eqs.\,\eqref{eq:field-squared}~and~\eqref{eq:gradient-field-sqr}; the latter are calculated by using a double sum for which the number of terms increases rapidly, $\mathcal{O}(N^2)$, with the number of bosons considered. In contrast, the expressions presented here in Eqs.\,\eqref{eq:complex-scalar-field-squared}~and~\eqref{eq:gradient-sum-two-terms} scale as $\mathcal{O}(N)$, making them more accessible for numerical calculations involving large $N$. 
The individual wave vectors $\bs{k}_{n}$ and frequencies $\omega_{n}$ are calculated from the velocities $\bs{v}_{n}$. These are drawn from the displaced Maxwell-Boltzmann distribution described by Eq.\,\eqref{eq:f_lab_velocity}. The phases $\theta_n$ are drawn from a uniform distribution spanning from $0$~to~$2\pi$.

The simulations consider $N=10^3$ bosons evolving during $20\,\tau_\varphi$ with a time resolution of $0.05\,\tau_\varphi$, where $\tau_\varphi$ is calculated using Eq.\,\eqref{eq:coherence_time}. Let us estimate the number density of particles in the UBDM field. For example, a UBDM mass of $10^{-11}$\,eV/$c^2$ (and a local energy density of $\rho\ts{dm} = 0.3$~GeV/cm$^3$) yields a number density of particles of $\sim \! 10^{19}$\,cm$^{-3}$. Also, consider that the de~Broglie wavelength if they move with a velocity of $v_0$ is $\sim \! 10^{10}$\,cm. Therefore, a sensor will be interacting with a number of particles that cannot be simulated with the methods presented here within a reasonable time. Instead we chose $N=10^3$ as the number of particles that can be simulated with our available hardware. By repeating the simulation hundreds of times, we can observe that the results converge. Additional checks were made to ensure that the spectral properties of the simulations matched theoretical predictions. The temporal resolution and the duration of the simulated field evolution were chosen considering plausible values for an experimental search. 

After generating $\varphi^2$ and $\bs{\nabla} \varphi_s^2$, $g^{(1)}(\tau)$ is calculated using Eq.\,\eqref{eq:first-order-coherence-definition}. Note that the mean value of the field is subtracted so that $g^{(1)}(\tau) \rightarrow 0$ for $ \tau \gg \tau_\varphi$ (see Appendix~\ref{app:search}). The coherence time [as defined in Eq.\,\eqref{eq:coherence_time_def}] for these fields can be obtained by integrating numerically. The integration is realized considering the data over the time interval $[0,5\tau_\varphi]$, and multiplying by two in order to account for the negative segment of the range.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Coherence time}
\label{app:similarity}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We define the coherence time as the power-equivalent width of $g^{(1)}(\tau)$~\cite{loudon2000the,saleh2019fundamentals},
\begin{equation}
    \tau_c = \int_{-\infty}^{+\infty} |g^{(1)}(\tau)|^2 d\tau,
    \label{eq:coherence_time_def}
\end{equation}
which describes a characteristic temporal width of $g^{(1)}(\tau)$. The full width at half maximum of the~$\varphi$ lineshape is $\approx \omega_c v_0^2/c^2$, giving a useful estimate of the benchmark coherence time $\tau_\varphi$ of the field~(the result is exact for a Lorentzian lineshape~\cite{gramolin2021spectral}), see Eq.~\eqref{eq:coherence_time} in the main text. Note that there is an ambiguity, up to a factor of $2\pi$, in the definitions of $\tau_c$ used in the literature~\cite{Centers2019}. Because the actual lineshape describing $\varphi$ is expected to be non-Lorentzian \cite{gramolin2021spectral}, $\tau_\varphi$ slightly differs from the coherence time of the field $\varphi$ derived from the simulations. For the considered $\bs{v}_\ts{lab}$, simulations show a coherence time $\approx 1.12(1) \tau_\varphi$.

% Coherence time of $\varphi^2_s(0,t)$ and gradient
The coherence time for $\varphi^2_s$ is approximately half of that for the field $\varphi$. This is a result of the field $\varphi^2_s$ being a sum over terms depending on the difference of frequencies $\omega_{nm}$, as opposed to $\varphi$, which only contains terms depending on $\omega_n$. The probability distribution of $\omega_{nm}$ can be calculated as the convolution of the distribution of $\omega_n$ with itself. This results in a distribution for $\omega_{nm}$ that is broader. Consequently, the coherence time is shorter since $g^{(1)}(\tau)$ is given by the Fourier transform of the power spectral density of $\varphi^2_s$ (proportional to the $\omega_{nm}$ distribution), according to the Wiener–Khinchin theorem. The gradient coupling features even shorter coherence times due to the $\bs{k}_{nm}$ factor weighting the contribution of the oscillating terms. Larger $\omega_{nm}$ tends to correspond to larger $\bs{k}_{nm}$: this effectively broadens the power spectral density of $\bs{\nabla} \varphi^2_s$, leading to a shorter coherence time. This is also the reason why parallel and perpendicular components of the gradient have different coherence times, as discussed below.

A formal derivation of $g^{(1)}(\tau)$ for $\varphi^2_s$ and $\bs{\nabla} \varphi^2_s$ in the simplified case where $|\bs{v}_{\text{lab}|} \gg v_0$ can be found in Appendix~\ref{app:analytic}.

% Relate coherence time of the fields to mass
The coherence time is also related to the mass of the UBDM particle as can be seen in Eq.\,\eqref{eq:coherence_time}. The relationship between the UBDM mass and the coherence time exhibited by $\varphi^2_s$ and $\bs{\nabla} \varphi^2_s$ is shown in Fig.\,\ref{Fig:massdep}. The coherence times for $\varphi^2_s$ and $\bs{\nabla} \varphi^2_s$ are proportional to the coherence time of $\varphi$, $\tau_\varphi$ as defined in Eq.\,\eqref{eq:coherence_time}. In the case of detection, this could be used to estimate the mass of the UBDM particles.
\begin{figure}[ht]
\center
\includegraphics[width=\columnwidth,trim={0 5mm 0 3mm},clip]{MassVStc.pdf}
\caption{\small{Mass dependence of the characteristic delay time at which $g^{(1)}(\tau)=0.5$ for $\varphi_s^2$ and projections of $\bs{\nabla} \varphi_s^2$. Each point is the result of 100~averages simulating $10^3$ particles (details in Appendix~\ref{app:calculation}).}}
\label{Fig:massdep}
\end{figure}

The velocity offset due to the movement of the laboratory frame, here equivalent to the galactic velocity of Earth $\bs{v}_\ts{lab} = v_\ts{lab} \bs{\hat{z}}$, breaks the isotropy of the field. However, this anisotropy is not directly observed when measuring the average intensity because the quadratic interactions depend on the difference of wave-vectors and frequencies as can be seen in Eqs.\,\eqref{eq:field-squared}~and~\eqref{eq:gradient-field-sqr}. Yet, the coherence time of the field is different for directions parallel and perpendicular to $\bs{v}_\ts{lab}$ and depends on its magnitude.

\begin{figure}[ht]
	\center
	\includegraphics[width=\columnwidth]{tcVSvlab.pdf}
	\caption{\small{ Coherence time, as defined in Eq.\,\eqref{eq:coherence_time_def}, as a function of $\bs{v}_\ts{lab}$ for the different cases of the UBDM field $\varphi$ studied.}}
	\label{Fig:tcVSvab}
\end{figure}

To understand the influence of $\bs{v}_\ts{lab}$ on the coherence time it is instructive to consider the limiting cases: $\bs{v}_\ts{lab}=0$ and $| \bs{v}_\ts{lab} | \gg v_0$ . Decomposing $\bs{k}$ into parallel and perpendicular components to $\bs{v}_\ts{lab}$ yields the following relationships:
\begin{equation}
	\bs{k}^\parallel_{nm} = \frac{ m_\varphi \bs{v}^\parallel_{nm} }{\hbar},~\text{and}~\bs{k}^\perp_{nm} = \frac{ m_\varphi \bs{v}^\perp_{nm} }{\hbar}.
	\label{eq:k_nm}
\end{equation}
The velocity difference  $\bs{v}_{nm} = \bs{v}_{n}-\bs{v}_{m}$ and the superscripts $\parallel$ and $\perp$ indicate whether the component is parallel or perpendicular to $\bs{v}_\ts{lab}$. One can also write the difference of frequencies in terms of the galactic-rest-frame velocity components as
\begin{equation}
	\begin{split}
		\frac{2c^2\omega_{nm}}{\omega_c} =~&(\bs{v}^\parallel_{n} + \bs{v}^\parallel_{m})\cdot \bs{v}^\parallel_{nm} + (\bs{v}^\perp_{n} + \bs{v}^\perp_{m})\cdot\bs{v}^\perp_{nm} \\
		&+ 2\bs{v}_\ts{lab}\cdot\bs{v}^\parallel_{nm}.
		\label{eq:omega_nm}
	\end{split}
\end{equation}

For $\bs{v}_\ts{lab}\ll \bs{v}_\ts{0}$ there is almost no anisotropy and therefore parallel and perpendicular components of $\nabla\varphi^2(\bs{r},t)$ have the same coherence time. However, as can be seen in Eqs.\,\eqref{eq:k_nm} and \eqref{eq:omega_nm}, $\omega_{nm}$ and $\bs{k}_{nm}$ have different dependence on $\bs{v}_{nm}$. For $\bs{k}_\ts{nm}$ the relationship is linear, while for $\omega_\ts{nm}$ it is non-linear and depends on the product of the sum and the difference of velocities. This implies a nonlinear correlation between $\omega_{nm}$ and $\bs{k}_{nm}$ as can be seen in Fig.\,\ref{Fig:tcVSvab}. Larger $\bs{v}_{nm}$ correlates with larger $\omega_{nm}$ and $\bs{k}_{nm}$. Since the gradient coupling is weighted by $\bs{k}_{nm}$ [see Eq.\,\eqref{eq:gradient-field-sqr}], the larger $\omega_{nm}$ have more weight in the sum. This broadens the frequency spectrum and shortens the coherence time of the gradient with respect to the field squared as can be seen in Fig.\,\ref{Fig:tcVSvab}. 

For large $v_\ts{lab}$ the behavior of $\nabla_\perp\varphi^2$ resembles that of $\varphi^2$ (see Fig.\,\ref{Fig:tcVSvab}) because the perpendicular terms of the velocity $\bs{v}^\perp_{nm} $ contribute little to $\omega_{nm}$. Therefore, $\bs{k}^\perp_{nm}$ and $\omega_{nm}$ are effectively independent and Eq.\,\eqref{eq:gradient-field-sqr} resembles Eq.\,\eqref{eq:field-squared} if multiplied by an appropriate scaling factor. 

In contrast, the coherence time of $\nabla_\parallel\varphi^2$ reduces faster than that of $\varphi^2$ as can be seen in Fig.\,\ref{fig:correlation}. The reason for this is that for large $v_\ts{lab}$, $\omega_{nm}$ becomes approximately $\propto \bs{k}^\parallel_{nm}$ and this proportionality scales with $v_\ts{lab}$. This increases the weight in the sum of terms with large $\omega_{nm}$ [in Eq.\,\eqref{eq:gradient-field-sqr}], leading to a broader power spectrum and consequently, a shorter coherence time. 

\begin{figure}[ht]
	\center
	\includegraphics[width=\columnwidth]{Correlation.pdf}
	\caption{\small{ Visualization of the dependence of $\omega_{nm}$ on $\bs{v}_{nm}^\perp$ and $\bs{v}_{nm}^\parallel$. The Monte Carlo simulation was performed drawing $10^5$ velocities from the distribution in Eq.~\eqref{eq:f_lab_velocity}. The number of instances in which $\bs{v}^\perp_{nm} $ or $\bs{v}^\parallel_{nm}$ results in a $\omega_{nm}$ within a 20 km/s $\times 4.6 \times 10^{-7}$ s$^{-1}$ bin is represented in color. The black contour-lines indicate when the number of counts is $10^1$, $10^2$ or $10^3$ and serve as a guide to illustrate the shape of the distributions. }}
	\label{fig:correlation}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Search with correlated sensor networks}\label{app:search}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Introduce use of stochastic propierties
The stochastic properties of $\varphi^2_s$ and $\bs{\nabla}\varphi^2_s$ can be used to search for UBDM. However, magnetometers and optical clocks are subjected to systematic noise sources in the laboratory, which feature some degree of temporal self-coherence similar to the UBDM field. For this reason, we focus our search on the cross-correlation of independent sensors, as their noise can be assumed to be mostly uncorrelated. %Therefore, if some degree of coherence between sensors is found it cannot be attributed to local sources.


%Definitions
In order to illustrate a possible method that could be used to search for UBDM fields using intensity interferometry, let us consider a measured time-series $\tilde{\mc{S}}_{A,B}(t)$ lasting several $\tau_{\varphi}$ from two different sensors, $A$~and~$B$. These time-series have their mean subtracted, such that $\mc{S}_{A,B} = \tilde{\mc{S}}_{A,B} - \langle \tilde{\mc{S}}_{A,B} \rangle_t$. The measurement in each sensor would have a small UBDM-related component $\kappa s(t)$, and a noise term $\mc{N}(t)$, $\mc{S}_{A,B} = \kappa_{A,B} s_{A,B}(t) + \mc{N}_{A,B}(t)$. The factor $\kappa_{A,B}$ accounts for coupling of the sensor to the UBDM field, and $s_{A,B}(t)$ is either $\varphi^2_s$ (scalar interaction) or $\hat{\bs{m}} \cdot \bs{\nabla} \varphi^2_s$ (pseudoscalar gradient interaction).

%Derive the auto-correlation (equivalent to cross-correlation) signal for clocks and magnetometers.
For a particular time series the degree of first-order coherence of these signals can be calculated as
\begin{equation}
	g^{(1)}_{AB}(\tau) = \frac{\langle \mc{S}_A(t) \mc{S}_B(t+\tau) \rangle_t}{\sqrt{\langle \mc{S}_A^2 \rangle_t \langle \mc{S}_B^2 \rangle_t}}.
	\label{eq:g1appc}
\end{equation}
%Uncorrelated noise terms to 0
While the signals $s_A(t)$ and $s_B(t)$ are correlated, the corresponding noise contributions, $\mc{N}_A(t)$ and $\mc{N}_B(t)$, are not. As a consequence, one can suppress the cross-terms $\langle \mc{N}_A \mc{N}_B \rangle_t$, $\langle \mc{N}_A s_B \rangle_t$, and $\langle \mc{N}_B s_A \rangle_t$ with sufficient amount of averaging (determined by the signal-to-noise ratios of sensors $A$ and $B$). Then, Eq.\,\eqref{eq:g1appc} reduces to

%Since the noise terms are uncorrelated with each other and the UBDM signals, we will assume that  $\langle \mc{N}_A \mc{N}_B  \rangle_t = 0$, $\langle \mc{N}_{A} s_{B} \rangle_t = \langle \mc{N}_{B} s_{A} \rangle_t =0$. In reality--for finite data segments--these quantities will not be zero, which will lead to experimental errors in the measurement of $g^{(1)}(\tau)$. Therefore, we stress that for an experiment one would have to measure $g^{(1)}(\tau)$ enough times in order to properly characterize its value and uncertainty (and compare it to that of $g^{(1)}(\tau\gg \tau_\ts{c})$). However, this assumption is instructive to understand the effect of the UBDM signal in the expected value of $g^{(1)}(\tau)$, and using it we can express~Eq.\,\ref{eq:g1appc} as
\begin{equation}
	g^{(1)}_{AB}(\tau) = \kappa_A \kappa_B \frac{ \langle  s_A(t) s_B(t+\tau) \rangle_t}{\sqrt{\langle \mc{S}_A^2 \rangle_t \langle \mc{S}_B^2 \rangle_t}}.
\end{equation}

%Mention sensors should be within de Broglie wavelength to meaure correlated signal (could scan distance).}
Strictly speaking, there will be a difference between $s_A(t)$ and $s_B(t)$ because of the spatial dependence of $\varphi^2$  (or $\bs{\nabla} \varphi^2$) that arises from the $\bs{k}\cdot \bs{r}$ term in Eq.\,\eqref{eq:single-boson-field}. However, for the considered UBDM mass range, the coherence length is much larger than the distance between the sensors. Therefore, $\varphi^2_s$ (or $\bs{\nabla} \varphi^2_s$) will approximately be the same for both sensors, $s_{A,B}(t) \approx s(t)$; and so $g^{(1)}(\tau)$ is proportional to the autocorrelation of the slow-varying component of the UBDM field squared~(or its gradient):
\begin{equation}
	\label{eq:g_tau_simple}
	g^{(1)}_{AB}(\tau) \approx \frac{\kappa_A \kappa_B}{\sqrt{\langle \mc{S}_A^2 \rangle_t \langle \mc{S}_B^2 \rangle_t}}\langle s(t) s(t+\tau) \rangle_t.
\end{equation}

As an example, evaluating Eq.\,\eqref{eq:g_tau_simple} at $\tau=0$ yields
\begin{equation}
	g^{(1)}_{AB}(0) \approx \frac{\kappa_A \kappa_B}{\sqrt{\langle \mc{S}_A^2 \rangle_t \langle \mc{S}_B^2 \rangle_t}}\langle s^2 \rangle_t .
	\label{eq:g1ofzero}
\end{equation}
The quantity $g^{(1)}(0)$ can be used as an estimator for the slow-varying component of the field (gradient) squared; it can be used to determine whether or not a UBDM signal is present in the data. For the scalar interaction, $\langle s^2 \rangle_t = \langle \varphi^2_s \varphi^2_s  \rangle_t$ and it can be shown  that for the gradient interaction $\langle s^2 \rangle_t = \prn{\cos \vartheta_{AB}/3} \langle \bs{\nabla}\varphi^2_s \cdot \bs{\nabla}\varphi^2_s  \rangle_t$, where $\vartheta_{AB}$ is the angle between the sensitive axes of the two sensors, $\bs{\hat{m}}_A$ and $\bs{\hat{m}}_B$ (see Appendix~\ref{app:AngleDep}). Assuming Gaussian noise with standard deviation $\sigma$, $\mc{N}\sim \mc{G}(0,\sigma^2)$, that dominates over the UBDM-signal component, $ \kappa s \ll \sigma$, Eq.\,\eqref{eq:g1ofzero} can be simplified to:
\begin{equation}
	g^{(1)}_{AB}(0) \approx \frac{\kappa_A \kappa_B}{\sigma_A \sigma_B}\langle s^2 \rangle_t.
	\label{eq:g0approx}
\end{equation}

The presence of a common correlated UBDM signal between two sensors will lead to a nonzero $g^{(1)}(0)$. In order to improve the accuracy to $g^{(1)}(0)$, one can average this value over measurements with different independent pairs of sensors since noise in the sensor leads to $g^{(1)}(0)<1$. If this value is significantly greater than zero, one can conclude that a common correlated signal is present in the data, as could arise from UBDM. This method is inherently broadband, as a large range of UBDM masses could lead to $g^{(1)}(0)>0$.

This scheme does not rely on the ALP having a Compton wave resonant with the experimental set-up. Such resonant searches require the interrogation of numerous narrow frequency bands which is a time-consuming process \cite{Asz01,Asz10,budker2014proposal,Sik14,chaudhuri2015radio,phipps2020exclusion,manley2020searching,crescini2020axion,braine2020extended,backes2021quantum,Ayb21CASPErE}.
In the case of detection in a search for correlated stochastic fluctuations, the mass range of the UBDM particle could be narrowed by analyzing the decay of the degree of coherence with the delay between the time-series, as illustrated in Figs.\,\ref{fig:g1}~and~\ref{Fig:massdep} of the main text.


%\section{Attenuation of $g^{(1)}(0)$ depending on the noise in each sensor} \label{app:attenuation}

%In the absence of noise in the sensors, $g^{(1)}(0)=1$. However, if noise is present, this value decreases. In the regime where the standard deviation of the noise is much greater than the signal, the behavior is described in Eq.\,\eqref{eq:g0approx}. We carried out simulations to confirm the scaling of $g^{(1)}(0)$ for $ \kappa s \ll \sigma$. 

%The evolution of $\varphi^2$ in time is simulated for $m_\varphi=10^{-11}$\,eV with $N=10^3$ particles. The duration of the segments used is $T=2 \times 10^3\,\tau_\varphi$ with a period of $\delta T=\tau_\varphi/20$. Two time-series, $A$ and $B$, are generated containing the simulation of $\varphi^2$ and Gaussian noise characterized by $\sigma_{A,B}= n_{A,B} \sqrt{\langle \varphi^2 \rangle_T}$, where $n_{A,B}$ characterizes the strength of the noise of $A$ and $B$. $5 \times 10^3$ simulations were performed then the results were binned to produce Fig.\,\ref{Fig:g0vsStN}
%\begin{figure}[ht]
%	\center
%	\includegraphics[width=\columnwidth]{g0vsStoN.pdf}
%	\caption{\small{$g^{(1)}(0)$ of $\mc{S_A}=\varphi_s^2 + \mc{N}_A$ and $\mc{S_B}=\varphi_s^2 + \mc{N}_B$. Where $\mc{N}_{A,B}$ indicates an added Gaussian noise component with centered at 0 with width $\sigma_{A,B}$. The red line show the expected value from the approximation given in Eq.\,\eqref{eq:g0approx}. \DK{This caption is quite unclear! Explain blue dots and red line. Explain simulation parameters.}\HMRIns{Is it better now?}} }
%	\label{Fig:g0vsStN}
%\end{figure}

%For high signal-to-noise ratios, $g^{(1)}(0)$ is found to be approximately one as expected. However, for low signal-to-noise ratios, the value of $g^{(1)}(0)$ decreases proportionally to the product of the respective signal-to-noises . Note that sampling longer times or averaging more measurements of $g^{(1)}(0)$ will increase the accuracy. \DK{Unfortunately the figure and caption are pretty unclear as to what is going on. How about this: can you show noise only and have that on the plot, too? (I guess it would be a line roughly at $g^{(1)} \approx 5 \times 10^{-4}$?) Then what you show is for a given noise level how large should the signal be to be distinguishable. This has to depend on the details of the simulation (like how many coherence times do you simulate = 2000), which should all be described in the figure caption. } \HMRIns{You are right it is quite unclear. I tried to explain it better now. However, I think this appendix is not important. It just justifying Eq.\,\eqref{eq:g0approx} which is theoretically clear. Moreover as you say this attenuation depends strongly on the parameters of the simulation. I don't think it is worth it to play more with the simulations here.}\draftNote{HMR: I suggest to remove this appendix} \DK{OK, that sounds good, I think you are right that this is not really necessary given Eq.\,\eqref{eq:g0approx} which seems to explain everything this is trying to say :).}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Signal to noise scaling with time}\label{app:SNscaling}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\NLF{THIS APPENDIX IS UNDER CONSTRUCTION.}\\
%\HMRDel{One could think that the signal-to-noise ratio scales at $T^{1/4}$ for these methods, as this can be the case when averaging power spectra of incoherent signals. This $T^{1/4}$ scaling can appear in UBDM searches when the data acquisition time is $\gg \tau_\varphi$, as presented in Ref.~\cite{budker2014proposal} for example. In such a case, the signal is being compared to a local oscillator where the phase between the local oscillator and the UBDM signal would effectively be random at any given time.}

%In the main text, we use that the signal-to-noise ratio of a UBDM-search that uses intensity interferometry will improve as $T^{1/2}$ in order to obtain Eqs.~\eqref{eq:min-field} and \eqref{eq:frac-freq-variation-clock-sens}, where $T$ is the measurement time.

%This seems to contradict Ref.~\cite{budker2014proposal}: which proposes that if a signal has a finite coherence time, the signal-to-noise will improve as $T^{1/4}$ for long times ($T \gg \tau_\varphi$). In this section, we clarify the differences between these two methods and demonstrate the $T^{1/2}$ scaling for the intensity interferometry method presented in this paper.

%The method presented in Reference~\cite{budker2014proposal} is based on the power spectral density. The peak amplitude in frequency-space of a coherent sinusoidal signal in time space increases linearly with $T$ since its lineshape corresponds Dirac delta. In contrast, when dealing with a sinusoidal signal with finite coherence time, the amplitude of the power spectral density peak remains constant when $T \gg \tau_\varphi$. This gives rise to the $T^{1/4}$ scaling of the signal-to-noise ratio.

%In order to determine the carrier frequency of a sinusoidal signal with finite coherence time, the signal is compared with a local oscillator that is coherent through the whole time $T$. Then the local oscillator frequency is scanned. So can the realization of the power spectral density be understood. Since the phase between the local oscillator and the signal is effectively random, part of the signal is lost.

%In contrast, the intensity interferometry method proposed in this work does not intend to determine the carrier frequency. Our interest lies on resolving the temporal correlation of the signal. For this, two independent measurements of the UBDM signal can be compared at different delay times $\tau$. Even though the phase of the signal incoherently changes in time, the effective phase between the two measurements is determined by $\tau$. For $\tau=0$ the two measurements are in phase which yields the maximum $g^{(1)}$. Since the two measurements are effectively coherent, the signal-to-noise ratio for the determination of $g^{(1)}$ increases as $T^{1/2}$.

%\HMRDel{However, for the intensity interferometry proposed in this work, the stochastic signal in a sensor network will effectively be the same (after properly accounting for the different sensitivities) in all sensors for a given time; so although the signal is stochastic in nature, all its harmonic components are in phase in the different sensors, so one may expect a signal-to-noise ratio scaling of $T^{1/2}$.}

%\HMREdit{Here we look at a ``bare-bones" analysis procedure in order to illustrate the signal-to-noise scaling properties}{The signal-to-noise scaling on the measuring time $T$ of the method presented can be determined by studying the statistical properties of $g^(1)(0)$.} \HMREdit{Let us c}{C}onsider two sensors (denoted by $A,B$) that measure signals \HMREdit{like the ones introduced}{as defined} in Appendix~\ref{app:search}, $\mc{S}_{A,B}(t) = \kappa_{A,B} s(t) + \mc{N}_{A,B}(t)$. For simplicity, we assume the sensitivity factors to be $\kappa_{A,B} = 1$.

%The signal-to-noise scaling on the measuring time $T$ of the method presented can be determined by studying the statistical properties of $g^{(1)}(0)$. Consider two sensors (denoted by $A,B$) that measure signals as defined in Appendix~\ref{app:search}, $\mc{S}_{A,B}(t) = \kappa_{A,B} s(t) + \mc{N}_{A,B}(t)$. For simplicity, we assume the sensitivity factors to be $\kappa_{A,B} = 1$.

%\HMREdit{Let us consider two discrete time-series with $M$ points each: $x_A$ and $x_B$. }{The sensors $A,B$ measure for some time $T$ with a sampling rate $SR$ producing two time-series with $M=T/SR$ points denoted by $x_A(t_m),x_B(t_m)$. The sensors sample $\mc{S}_{A,B}$ at the same time.} \HMRDel{These time series $x_A$ and $x_B$ are taken from sensors $A$ and $B$ respectively and correspond to $\mc{S}_{A,B}$ sampled at the same time.} \HMREdit{It is useful to note that, multiplying $x_A$ and $x_B$ will lead to:}{ The element-wise multiplication of the two time-series can be written as, }
%The sensors $A,B$ measure for some time $T$ with a sampling rate $SR$ producing two time-series with $M=T/SR$ points denoted by $x_A(t_m),x_B(t_m)$. The sensors sample $\mc{S}_{A,B}$ at the same time. The element-wise multiplication of the two time-series can be written as,
%\begin{align}
%    x_A x_B &= (s + \mc{N}_A)( s + \mc{N}_B) \\&= \mc{N}_A \mc{N}_B + (\mc{N}_A + \mc{N}_B)s + s^2,
%\end{align}
%for each of the elements. Where the time dependence of the terms is omitted to simplify the notation. The noise in the sensors is assumed to be Gaussian centered at zero with variance $\sigma^2$, $\mc{N} \sim \mc{G}(0,\sigma^2)$, while the expectation value of the UBDM component, $s$, is zero. Then it follows that the expectation values for the elements in the time-series $x_A x_B$ are,
%\begin{align}
%    \EE[x_A x_B] &= \EE[s^2].
%\end{align}
%Second order terms with the noise and cross terms noise-signal have an expectation value of zero. 

%The variance $\VV[x_A x_B]$ of these individual elements are approximated by
%\begin{align}
%    \zeta^2 \equiv \VV[x_A x_B] \approx  \EE[\mc{N}_A^2 \mc{N}_B^2].
%\end{align}
%Since $s$, $\mc{N}_A$, and $\mc{N}_B$ are independent, the expectation value of terms proportional to odd powers of these terms is 0. Additionally since we focus on small signals (${\EE[\mc{N}^2] \gg \EE[s^2]}$), the variance in the product is dominated by square of the noise terms.

%Following the calculation of $g^{(1)}(0)$, consider the average of the $M$ points after the element-wise multiplication of the time-series,
%\begin{align}
%    \Gamma &\equiv \frac{1}{M} \sum^M_{m=0} x_A(t_m) x_B(t_m).
%\end{align}
%Given a large enough $M$, we can use the central limit theorem, which states that $\Gamma$ will be approximately distributed by a Gaussian with a mean and variance well-defined by those of their individual elements,
%\begin{align}
%    \Gamma &\sim \mathcal{G}(\EE[s^2], \zeta^2/M ) \label{eq:GaussianDMSensitive}
%\end{align}

%By measuring $N$ segments of $M$ points, one could obtain a measurement of $\Gamma$ with a determined uncertainty, ie. $\Gamma = \overline{\Gamma} \pm \delta \Gamma$. Where the overline denotes the mean. Since we are interested in seeing how the signal-to-noise ratio of $s$ (and not $s^2$) scales, we can relate the measured $\Gamma = \overline{\Gamma} \pm \delta \Gamma$ to $s= \overline{s} \pm \delta s$ using linear error propagation:
%\begin{align}
%    \overline{s} &= \sqrt{\overline{\Gamma}}\\
%    \delta s &= \frac{\delta\Gamma}{2 \sqrt{\overline{\Gamma}}}.
%\end{align}
%One may object that linear propagation is not suitable because the uncertainties are expected to be large. However, $M$ is arbitrary, so for a large enough $M$, linear propagation will be valid.  Also, this is just an example to show this scaling can be obtained, in reality... things are more complicated... XXXX. \NLF{Help me Derek/Hector!}
%From Eq.\eqref{eq:GaussianDMSensitive} it follows that the uncertainty of $\Gamma$ is,
%\begin{align}
%    \delta \Gamma &\propto \sqrt{\frac{\zeta^2}{M}}.
%\end{align}
%Therefore, the signal-to-noise ratio, $s_0 / \delta s_0$ (ie. how many standard deviations is the mean away from zero), scales as:
%\begin{align}
%    \frac{\overline{s}}{\delta s} = \frac{2 \overline{\Gamma}}{\delta \Gamma} \propto (M N)^{1/2}.
%\end{align}
%Each element in the product of time-series contributes to reduce the uncertainty in $\Gamma$. Naturally, the number of points $N M \propto T$. 

%Consider an additional pairs of equivalent sensors $C,D$ measure simulatinously for the same time $T$. By grouping the data in the same way $N$ measurements of $\Gamma$ using $M$ points each, we can double the statistics for the determination of $\Gamma$. Then for $N_p$ additional pairs we find that,
%\begin{align}
%    \frac{\overline{s}}{\delta s} \propto (N_p M N)^{1/2} \propto (N_p T)^{1/2} .
%\end{align}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Angle dependence of the correlation between magnetometers}\label{app:AngleDep}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Introduce problem
We are interested in understanding the coherence between two signals, $s_A$ and $s_B$, that are the result of the gradient coupling. In particular, for $j\in\{A,B\}$, let $\boldsymbol{\hat{m}_j}$ be the sensitive axis of magnetometer $j$, so $s_j = \boldsymbol{\hat{m}_j} \cdot \boldsymbol{\nabla} \varphi^2_s$. The calculation of the coherence requires one to understand $\left< s_A s_B \right>_t$, but each $s_A$ and $s_B$ depends on the relative angle between the respective sensitive axis and the field gradient. These angles are not known and change over time as the field evolves.

% Define assumptions
Note that $\boldsymbol{\nabla} \varphi^2_s$ is a sum of terms $\propto \bs{v}_{nm}$. The angle dependence between the field gradient and the sensitive axes can be accounted for under some basic assumptions. In particular, assume that $\boldsymbol{v}_{nm}$ is ergodic in direction --- that is, over time, $\boldsymbol{\hat{v}}_{nm}$ will take all values over the sphere $S^2$.
Ergodicity implies that $\left< s_A s_B\right>_t = \left< s_A s_B\right>_{S^2}$.
As another simplifying assumption, let $v^2$ be independent of $\boldsymbol{\hat{m}_j}\cdot \boldsymbol{\hat{v}}_{nm}$ so 
\[
\left< (\boldsymbol{\hat{m}_A}\cdot \boldsymbol{v}_{nm})(\boldsymbol{\hat{m}_B}\cdot \boldsymbol{v}_{nm}) \right>_t = \bar{v}^2 \left< (\boldsymbol{\hat{m}_A}\cdot \boldsymbol{\hat{v}}_{nm})(\boldsymbol{\hat{m}_B}\cdot \boldsymbol{\hat{v}}_{nm}) \right>_t\ ,
\]
for $\bar{v}^2 = \left< \lVert \boldsymbol{v}_{nm} \rVert^2 \right>_t$.

% Calculate the dependence
The correlation between magnetometers can be calculated explicitly with the above assumptions. This will still depend on the relative angle $\vartheta_{AB}$ between the sensitive axes $\boldsymbol{\hat{m}_A}$ and $\boldsymbol{\hat{m}_B}$. Let us define the axes such that $\boldsymbol{\hat{m}_B}$ points along the $z$-axis and $\boldsymbol{\hat{m}_A}$ lies in the $xz$-plane in the $+x$-direction. The gradient direction $\boldsymbol{\hat{v}}$ can be arbitrary, described by the azimuthal angle $\phi$ and polar angle $\theta$ in this coordinate system. Thus
\begin{align*}
	\boldsymbol{\hat{m}_A} &= \left( \sin\vartheta_{AB}, 0, \cos\vartheta_{AB} \right)\ , \\
	\boldsymbol{\hat{m}_B} &= (0, 0, 1)\ , \\
	\boldsymbol{\hat{v}}_{nm} &= \left( \cos\phi \sin\theta, \sin\phi \sin\theta, \cos\theta \right)\ .
\end{align*}
The following calculation can be made explicitly:
\begin{align}
	\left<s_As_B\right>_t &\approx \left<s_As_B\right>_{S^2} \nonumber \\
	&= \frac{\bar{v}^2}{4\pi}\int_0^{2\pi}d\phi \int_0^\pi d\theta ( \sin\vartheta_{AB} \cos\phi\sin\theta \nonumber \\
	& \qquad +\cos\vartheta_{AB} \cos\theta )\cos\theta\sin\theta \nonumber \\
	&= \frac{\bar{v}^2}{3} \cos\vartheta_{AB}\ ,
	\label{eq:angledep}
\end{align}
where the $\sin\vartheta_{AB}$ term averages out over the sphere over both the azimuthal and polar directions. 

\begin{figure}
	\center
	\includegraphics[width=\columnwidth]{AngleDependance.pdf}
	\caption{\small{$g^{(1)}(0)$ of $\hat{\bs{m}}_A \cdot \bs{\nabla} \varphi_s^2$ and $\hat{\bs{m}}_B \cdot \bs{\nabla} \varphi_s^2$ as a function of the relative angle between $\hat{\bs{m}}_A$ and $\hat{\bs{m}}_B$, $\vartheta_{AB}$. No noise was added to the generated fields. The blue dots are the results of independent simulations where the sensitive axes are randomly generated on the sphere. The red curve shows the $\cos(\vartheta_{AB}$) as predicted in Eq.\,\eqref{eq:angledep}.}}
	\label{Fig:angledep}
\end{figure}

The results of simulations shown in Fig.\,\ref{Fig:angledep} illustrate this dependence. An interesting feature is that the dispersion in $g^{(1)}(0)$ also depends on the relative angle between the magnetometers. This dispersion in $g^{(1)}(0)$ is not due to noise, as noise was not added to the simulated magnetometer data, but rather results from the UBDM fields themselves. If the sensitive axes of the sensors are not parallel,  dispersion in $g^{(1)}(0)$ is introduced by the uncorrelated components of the UBDM field measured; because the orthogonal components of $\bs{\nabla} \varphi_s^2$ (e.g., along $\hat{x},\hat{y},\hat{z}$) are uncorrelated, measuring different orientations produces a spread in $g^{(1)}(0)$.
%this dispersion is geometrical in origin and arises from the random orientation of $\bs{\nabla} \varphi_s^2$ with respect to the pair of magnetometers. Since the different components of $\bs{\nabla} \varphi_s^2$ (along $\hat{x},\hat{y},\hat{z}$) are uncorrelated, a misalignment between the sensors will lead to a larger uncorrelated component in the signals, that increases the spread in $g^{(1)}(0)$.


	
%	of the pseudoscalar gradient interaction as a function of the angle between the sensitive axes of the magnetometers.}. For each \DKEdit{measurement}{simulation} a $\bs{\nabla}\varphi^2_s$ is generated and projected in two random directions. \DK{Describe the meaning of the blue dots and red curve!}. The red curve shows the cosine of the relative angle $\cos\vartheta_{AB}$ between two sensors   }

% \draftNote{JAS (Note on gradient coupling): we see $s_i\sim \boldsymbol{\hat{m}_i}\cdot \boldsymbol{v}=v\cos\theta_i$, where $\boldsymbol{v}$ is the gradient. Then, $s_A s_B = v^2\cos(\theta_A)\cos(\theta_B)$, but with $\theta_A$ and $\theta_B$ given with respect to $\boldsymbol{v}$. 
% WLOG, let $B$ point in the $z$-direction $\boldsymbol{\hat{m}_B}=(0,0,1)$, $A$ point in the $xz$-plane $\boldsymbol{\hat{m}_A}=(\sin\vartheta_{AB},0,\cos\vartheta_{AB})$, and the gradient point in a random direction over time, $\boldsymbol{\hat{v}}=(\cos\phi \sin\theta,\sin\phi \sin\theta, \cos\theta)$. Now, take the average over the sphere 
% \begin{align*}
% \left<s_As_B\right>_t &\approx \left<s_As_B\right>_{S^2} \\
% &= \frac{v^2}{4\pi}\int_0^{2\pi}d\phi \int_0^\pi d\theta ( \sin\vartheta_{AB} \cos\phi\sin\theta \\
% & \qquad +\cos\vartheta_{AB} \cos\theta )\cos\theta\sin\theta \\
% &= \frac{v^2}{3} \cos\vartheta_{AB}\ .
% \end{align*}
% Note that the term with $\cos\phi$ averages-out, and ``3'' can be replaced by the number of spatial dimensions (the proof of this is a bit long, but I can send it to anyone who wants to see it). 
% }

%OLD - To be replaced with Joey's derivation of g1(tau) fur a^2, and gradients.
%\section{Analysis with a simplified lineshape}

%The lineshape (or normalized power spectral density), for the $a(t)$ field has been derived and is given by:

%\begin{gather}
%\lambda(\nu) = \frac{2c^2}{\sqrt{\pi} v_0 v_{\text{lab}} \nu_a} \exp{\left(-\frac{\beta^2 v_0^2}{4v_{\text{lab}}^2} - \frac{v_{\text{lab}}^2}{v_0^2}\right)} \sinh{\beta}, %\label{eq:non-gradient_lineshape}
%\end{gather}
%where $v_{\text{lab}} = |\mathbf{v}_{\text{lab}}|$ and we have denoted for brevity
%\begin{equation}
%\beta =\frac{2c v_{\text{lab}}}{v_0^2} \sqrt{\frac{2(\nu - \nu_a)}{\nu_a}}.
%\end{equation}

%In different forms, the lineshape~\eqref{eq:non-gradient_lineshape} has been previously reported in Refs.\,\cite{gramolin2021spectral,turner1990periodic,o2017axion,derevianko2018detecting,foster2018}. This normalized lineshape can be interpreted as the probability density function of finding an UBDM particle with a frequency between $\nu$ and $\nu+d\nu$.

%From Eq.\,\eqref{eq:field-squared} it can be seen that each UBDM-particle pair will add a unit of power at $\omega_{nm} = \omega_n - \omega_m$. Therefore, the normalized lineshape for the slow-varying part of $a^2(t)$, $\lambda_{2,s}$, will be the probability density function of $\omega_{nm}$; which can be calculated with a convolution given that we know that $\omega_n,\omega_m$ are distributed as $\lambda(\nu)$,

%\begin{equation}
%    \lambda_{2,s}(\nu) = \int_{-\infty}^{\infty} \lambda(\nu + \tilde{\nu}) \lambda( \tilde{\nu}) d\tilde{\nu}.
%\end{equation}

%\draftNote{This section is under construction.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analytic solution for \texorpdfstring{$g^{(1)}(\tau)$}{g1(t)}}
\label{app:analytic}
%\draftNote{This section is new}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this Appendix, an analytic expression for the degree of coherence is derived. Let us consider a signal given by the sum of sinusoidal functions,
\begin{equation}\label{eq:sinSumSig}
	S(t) = \sum_n a_n \cos\left( \omega_n t + \phi_n \right)\,.
\end{equation}
For simplicity, we consider the case in which the average signal is zero, $\omega_n\neq0$, and the frequencies are all different, $\omega_n\neq\omega_m$ for $m\neq n$. Considering the two-point correlation function defined as,
\begin{equation}
	C_2(\tau) = \left< S(t)S(t+\tau) \right>_t\,,
\end{equation}
then $g^{(1)}(\tau) = C_2(\tau)/C_2(0)$. 

% two-pt corr funct exact
When averaging over the product of the two signal functions, the oscillating components average out. As a result, the only components that contribute to the coherence are from products of the same sinusoidal terms. The resulting two-point correlation function is then
\begin{equation}\label{eq:sinSum2ptCorr}
	C_2(\tau) = \frac{1}{2} \sum_n a_n^2 \cos\left( \omega_n\tau \right)\,.
\end{equation}
%If different sinusoidal components had the same frequency, additional cross-terms $a_na_m\cos(\phi_m-\phi_n)$ would appear in the sum. If there are many such terms with random phases, these cross-terms will average out. 

% distribution of frequencies
For this study, we consider the case in which there are $N\gg 1$ sinusoidal components in the signal. The frequencies $\omega_n$ and amplitudes $a_n$ are sampled from some probability distribution. Here, this distribution is derived from a distribution of particle velocities $P_v(\boldsymbol{v})d^3\boldsymbol{v}$ given by Eq.\,\eqref{eq:f_lab_velocity}. %Generically, one parameterizes the probability distribution function with $\boldsymbol{x}$, $P(\boldsymbol{x})d\boldsymbol{x}$, where $\boldsymbol{x}$ can be reparameterized with the frequency, amplitude, and other ancillary variables.
We approximate the sum in Eq.\,\eqref{eq:sinSum2ptCorr} as an integral in which $a_n^2$ is replaced with the differential $a^2(\boldsymbol{x})P(\boldsymbol{x}) d\boldsymbol{x}$,
\begin{equation}\label{eq:sinInt2ptCorr}
	C_2(\tau) = \frac{1}{2} \int d\boldsymbol{x}\,a^2(\boldsymbol{x})P(\boldsymbol{x}) \cos\left[\omega(\boldsymbol{x}) \tau \right]\,.
\end{equation}

% case for both couplings
Here, for both the $\varphi^2$- and $\bs{\nabla}\varphi^2$-coupling, the probability distribution function is parameterized by $\boldsymbol{x}=\{ \boldsymbol{k_1}, \boldsymbol{k_2} \}$, for $\boldsymbol{k_i}=(m_\varphi / \hbar)\boldsymbol{v_i}$ described by a Gaussian distribution of velocities offset by the laboratory reference frame. It is useful to consider the average $\boldsymbol{\bar{k}}=(\boldsymbol{k_1}+\boldsymbol{k_2})/{2}$ and difference $\boldsymbol{\Delta} = \boldsymbol{k_1} - \boldsymbol{k_2}$. In these variables, $d^3\boldsymbol{k_1}d^3\boldsymbol{k_2}=d^3\boldsymbol{\bar{k}}d^3\boldsymbol{\Delta}$ and the difference in frequencies $\omega_{12} = (\hbar/m_\varphi) \boldsymbol{\bar{k}}\cdot\boldsymbol{\Delta}$. For either coupling, the contribution from $\mathcal{O}(2\omega_c)$ frequency components and the constant offset will be neglected. Also, let $\sigma_k=(m_\varphi / \hbar)\sigma_v$ ($v_0^2=2\sigma_v^2$) describe the width of the $\boldsymbol{k}$-vector distribution and $\boldsymbol{k_\text{lab}} = ({m_\varphi}/{\hbar}) \boldsymbol{v_\text{lab}}$ describe the offset of the distribution due to the laboratory reference frame. 

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{coherence_analytic}
    \caption{\small{Coherence of different signal types from numeric simulations (solid) compared to their analytic approximations (dashed, given by Eqs.\,\eqref{eq:g1_analytic_phi2}\,,\,\eqref{eq:g1_analytic_grad_phi2}). To better reflect the approximation conditions, the lab velocity is tripled, $v_\text{lab}=699$\,km/s (while $v_0$ is kept at $220$\,km/s). The analytic approximation for $\varphi_s^2$ is the same as for the gradient coupling for a $\boldsymbol{\hat{m}}$ perpendicular to the lab velocity $\nabla_\perp\varphi_s^2$.}}
    \label{fig:coherence_analytic}
\end{figure}

% \phi^2 coupling
For a signal given by $\varphi_s^2$, the amplitude of a sinusoidal component is constant while the frequency is given by the difference $\omega(\boldsymbol{k}_1) - \omega(\boldsymbol{k}_2)$. The integral in Eq.\,\eqref{eq:sinInt2ptCorr} can be approximated for $k_\text{lab} \gg \sigma_k$. Under this approximation, $\boldsymbol{\bar{k}}\approx\boldsymbol{k_\text{lab}}$ (i.e., one can neglect the uncertainty in the average $\boldsymbol{\bar{k}}$), which reduces the six-dimensional integral to a three-dimensional integral over $\boldsymbol{\Delta}$. The result is the degree of first-order coherence (see Fig.\,\ref{fig:coherence_analytic})
\begin{equation}
	g^{(1)}(\tau) \approx \exp\left[ -\left( \frac{m_\varphi v_\text{lab} \sigma_v}{\hbar} \right)^2 \tau^2 \right]\,.
	\label{eq:g1_analytic_phi2}
\end{equation}
Note that we consider a lab-frame for which $v_\ts{lab}\approx v_k$, so this is only a rough approximation. Heuristically, one would expect that the coherence is overestimated, because this approximation neglects a component of the frequency dispersion. 

% grad(\phi^2)
A signal given by coupling to the gradient $\nabla \varphi_s^2$ will have amplitudes of different sinusoidal components $\sim \boldsymbol{\hat{m}}\cdot\boldsymbol{\Delta}$. Here, we denote the angle between $\boldsymbol{\hat{m}}$ and $\boldsymbol{v_\text{lab}}$ with $\theta$. Using the approximation $k_\text{lab} \gg \sigma_k$ as before, the coherence is (see Fig.\,\ref{fig:coherence_analytic})
\begin{align}
	g^{(1)}(\tau) &\approx \frac{\sin^2(\theta) + 2\pi\left( 1-2\left( \frac{m_\varphi}{\hbar} v_\text{lab} \sigma_v \tau \right)^2 \right)\cos^2(\theta) }{\sin^2(\theta) + 2\pi\cos^2(\theta) } \nonumber \\
	&\qquad\times\exp\left[ -\left( \frac{m_\varphi v_\text{lab} \sigma_v}{\hbar} \right)^2 \tau^2 \right]\,.
	\label{eq:g1_analytic_grad_phi2}
\end{align}
Observe that the coherence becomes negative for $\theta\neq \pi/2$ when
\begin{equation}
    \tau>\frac{\hbar}{m_\varphi v_\text{lab} \sigma_v}\sqrt{\frac{1}{2}+\frac{\tan^2\theta}{2\pi}}.
\end{equation}

% 1d case
%\draftNote{HMR: I would remove the discussion of the one dimensional case.} \DK{It's cool, but I agree with Hector here :).}  Finally, exact solutions to the coherence can be calculated in one-dimension without the need for any approximations. The coherence for a $\varphi_s^2$ signal is given by
%\begin{equation}
%	g^{(1)}(\tau) = \frac{\exp\left[ -\frac{\left( \frac{m_\varphi}{\hbar} v_\text{lab} \sigma_v \tau \right)^2}{1+ \left( \frac{m_\varphi}{\hbar} \sigma_v^2\tau \right)^2}\right]}{\sqrt{1+ \left( \frac{m_\varphi}{\hbar} \sigma_v^2\tau \right)^2}}\,.
%\end{equation}
%Likewise, for $\nabla\varphi_s^2$ in one-dimension,
%\begin{align}
%	g^{(1)}(\tau) &= \frac{ (\sigma_v^2-2v_\text{lab}^2)\left(\frac{m_\varphi}{\hbar}\sigma_v \tau\right)^2 + 1 }{\left( \left(\frac{m_\varphi \sigma_v^2}{\hbar}\tau\right)^2 + 1 \right)^{5/2}} \nonumber \\
%	&\qquad\times \exp\left[ -\frac{ \left( \frac{m_\varphi}{\hbar}  v_\text{lab} \sigma_v \tau \right)^2}{ \left(\frac{m_\varphi \sigma_v^2}{\hbar}\tau\right)^2 + 1 } \right]\,,
%\end{align}
%where $\boldsymbol{\hat{m}}$ is trivially parallel to $v_\text{lab}$. Of particular note, the coherence for the gradient coupling is always positive for $v_\text{lab}\leq \sigma_v/\sqrt{2} = v_0/2$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Back-action effects}
\label{app:back-action}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As noted in the main text, a consideration particular to searches for ultralight scalar fields with quadratic couplings to SM particles and fields is the possible back-action of mass density on the scalar field, which can either reduce or enhance the field amplitude \cite{stadnik2020new,Oli08,hinterbichler2010screening,jaffe2017testing,hees2018violation}. This back-action arises due to the fact that the bare potential for the scalar field, namely $m_\varphi^2 c^2 \varphi^2/(2 \hbar^2)$, is modified by the presence of the Lagrangian in Eq.\,\eqref{eq:scalar-Lagrangian}. 
The quadratic terms in the interaction Lagrangian endow the scalar field with an effective mass $m\ts{eff}$ in the presence of matter; this effect is analogous to the screening of magnetic fields caused by the Meissner effect~(where the photon gains an effective mass inside a superconductor). 
Depending on the sign of the interaction, back-action can lead to either screening or antiscreening \cite{hees2018violation}.

For the interaction between $\varphi$ and the electromagnetic field leading to variation of $\alpha$ considered in Eq.~\eqref{eq:scalar-Lagrangian}, in the presence of matter the scalar field acquires an effective mass given by
\begin{align}
m\ts{eff}^2 \approx m_\varphi^2 \pm \frac{2 \hbar^3}{c} \frac{\rho_\gamma}{\Lambda_\gamma^2}~,
    \label{eq:effective-scalar-mass}
\end{align}
where $\rho_\gamma \approx -F_{\mu\nu}^2/4$ is the Coulomb energy density of a nonrelativistic nucleus averaged over the characteristic volume outside of which the UBDM field changes appreciably, which in our considered case is orders of magnitude larger than the size of a nucleus and thus depends on the average local matter density. Based on the numerical estimates of Ref.\,\cite{stadnik2020new}, for the Earth's interior $\rho_\gamma \approx 6 \times 10^{21}~{\rm GeV/cm^3}$ and for Earth's atmosphere $\rho_\gamma \approx 6 \times 10^{17}~{\rm GeV/cm^3}$. The (anti)screening effect due to back-action can be important if
\begin{align}
    m_\varphi^2 \Lambda_\gamma^2  \lesssim \frac{2 \hbar^3}{c} \rho_\gamma~.
    \label{eq:screening-limit}
\end{align}

%\DKDel{Based on Eq.\,\eqref{eq:effective-scalar-mass}, it is evident that the (anti)screening effect due to back-action is most important for the smallest values of $\Lambda_\gamma$ and $m_\varphi$. To probe beyond astrophysical limits we are interested in $\Lambda_\gamma \gtrsim 10^4~{\rm GeV}$, and for practical purposes it is difficult to measure fluctuations corresponding to boson masses smaller than $m_\varphic^2 \approx 10^{-16}~{\rm eV}$. Using these values as lower bounds on $\Lambda_\gamma$ and $m_\varphi$, we find that even for the interior of Earth the inequality \eqref{eq:no-screening-limit} is satisfied, so the accessible parameter space for clock experiments illustrated in Fig.\,\ref{Fig:sensitivity-clocks} is unaffected by (anti)screening due to back-action.}

Based on Eq.~\eqref{eq:screening-limit}, for values of $m_\varphi\Lambda_\gamma$ above the long-dashed blue line in Fig.~\ref{Fig:sensitivity-clocks} (anti)screening effects can be important and cover the entire range of parameter space accessible with a network of current optical atomic clocks. Here $\rho_\gamma$ for Earth's interior is used since this is the relevant value for the long-wavelength interactions considered. Thus sensitivity to positive-signed quadratic scalar interactions [as in Eq.~\eqref{eq:effective-scalar-mass}] is significantly diminished near Earth's surface. On the other hand, a space-based clock \cite{schiller2007optical,Schkolnik2022Apr} (or atom interferometer \cite{arvanitaki2018search}) network could largely avoid such screening effects due to the significantly lower average mass density in the interplanetary medium. In the case of negative-signed quadratic scalar interactions [as in Eq.~\eqref{eq:effective-scalar-mass}], there is antiscreening and the field amplitude can be significantly enhanced \cite{hees2018violation}. However, further analysis is required to calculate the form of the signal from stochastically fluctuating UBDM in this scenario. Finally, we note that constraints on coupling constants based on screening and antiscreening of scalar fields can be derived from experiments testing the equivalence principle \cite{hees2018violation}.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Heuristic argument for the difference in sensitivity between magnetometers and clocks }
\label{app:SensiticityDifference}

As can be seen in Figs.\,\ref{Fig:sensitivity-GNOME} and \ref{Fig:sensitivity-clocks}, the sensitivity of an optical clock network to the coupling parameter $1/\Lambda_\gamma$ far exceeds that of magnetometer networks to the equivalent coupling parameter $1/f_q$. 
Here we offer a heuristic explanation for this difference between the two cases. 
In the case of the scalar interaction [described by Eq.\,\eqref{eq:scalar-Lagrangian}] probed by clocks, the UBDM field modulates the electromagnetic binding energy of the atom [$\sim e^2/(2a_B) \approx \alpha^2 m_e c^2/2$, where $e$ is the electron charge magnitude, $a_B$ is the Bohr radius, and $m_e$ is the electron mass]. 
This effect leads to an energy shift approximately given by
\begin{align}
    \Delta E\ts{clock} \sim \prn{\frac{\hbar c \varphi_s^2}{\Lambda_\gamma^2}} \times \prn{\frac{1}{2} \alpha^2 m_e c^2}~,
    \label{eq:clock-energy-shift-order-of-mag}
\end{align}
where the first factor in parentheses describes the effective coupling constant associated with the UBDM field (proportional to the UBDM-induced fractional energy shift) and the second factor in the parentheses describes the scale of the electromagnetic binding energy of the atom. 
This manifestation of the scalar coupling is seen from the fact that it results in an effective modulation of the fine-structure constant $\alpha$ and/or electron mass $m_e$ as described by Eqs.\,\eqref{eq:scalar-mass-variation} and \eqref{eq:scalar-alpha-variation}. 
In the case of the pseudoscalar interaction Eq.~\eqref{eq:quadratic-Hamiltonian} probed by magnetometers, it is the energy associated with the field gradient ($\sim m_\varphi c v_0$) that is modulated, leading to an energy shift approximately given by %\draftNote{Revise dependence with $v\ts{lab}$} \DK{I think we can use $v_0$.}
\begin{align}
    \Delta E\ts{mag} \sim \prn{\frac{\hbar c \varphi_s^2}{f_q^2}} \times \prn{m_\varphi c^2 \frac{v_0}{c}}~.
    \label{eq:mag-energy-shift-order-of-mag}
\end{align}
From comparing Eqs.\,\eqref{eq:clock-energy-shift-order-of-mag} and \eqref{eq:mag-energy-shift-order-of-mag}, it is evident that the scale of the fractional energy modulation given by the first factor in parentheses is similar in the two cases. 
Taking the ratio between the two energy shifts yields
\begin{align}
\frac{\Delta E\ts{clock}}{\Delta E\ts{mag}} \sim \frac{f_q^2}{\Lambda_\gamma^2} \frac{\alpha^2}{2}  \frac{c}{v_0} \frac{m_e}{m_\varphi}~,
\end{align}
and thus the ratio of the squares of the coupling constants determined by given energy shift measurements is
\begin{align}
\frac{\Lambda_\gamma^2}{f_q^2} \sim \frac{\Delta E\ts{mag}}{\Delta E\ts{clock}} \frac{\alpha^2}{2}  \frac{c}{v_0} \frac{m_e}{m_\varphi} \sim 0.1 \frac{\Delta E\ts{mag}}{\Delta E\ts{clock}} \frac{m_e}{m_\varphi}~.
\end{align}
For $m_\varphi c^2 \sim 10^{-14}~{\rm eV}$, $\Delta E\ts{mag} \sim 10^{-19}~{\rm eV}$ (corresponding to a magnetic field measurement at the level of a few pT for a nuclear spin), $\Delta E\ts{clock} \sim 10^{-16}~{\rm eV}$ (corresponding to a fractional uncertainty in a measurement of an optical transition at the $10^{-16}$ level) and $c/v_0 \sim 10^3$, we see that $\Lambda_\gamma^2/f_q^2 \sim 10^{15}$. This estimate demonstrates that the source of the enhanced sensitivity of clocks is from the large $m_e/m_\varphi$~mass ratio, expected for UBDM ($m_\varphi \ll 1$~eV/$c^2$).\\

